Optimal moments on redundancies in job cloning

We consider the problem of job assignment where a master server aims to compute some tasks and is provided a few child servers to compute under a uniform straggling pattern where each server is equally likely to straggle. We distribute tasks to the servers so that the master is able to receive most of the tasks even if a significant number of child servers fail to communicate. We first show that all \textit{balanced} assignment schemes have the same expectation on the number of distinct tasks received and then study the variance. We show constructions using a generalization of ``Balanced Incomplete Block Design''\cite{doi:10.1111/j.1469-1809.1939.tb02219.x,sprott1955} minimizes the variance, and constructions based on repetition coding schemes attain the largest variance.

==> extreme-varaince-results.tex <==
\section{Results on extreme variance based on $[\mathfrak{m}^D(m)]_{m=0}^{r}$}\label{extreme_var_section}

To explore the range of variances that balanced $(n,k,r,c)$ job assignments attain, we define a shape vector $h_D$.

%From the previous sections, that while all $(n,k,r,c)$ balanced job assignments give the same mean, they display different variances based on the values of $\mathfrak{m}^D(m)$ and explore the range of variances that balanced  $(n,k,r,c)$ job assignments.


%that arise in the respective job assignments. Here $\mathfrak{m}^D(m)$ refers to number of pairs of distinct jobs assigned together to precisely $m$ servers as defined in \eqref{m_D_defn}. We now explore the range of variances that balanced  $(n,k,r,c)$ job assignments can attain. %therefore define a vector $h_D$ that we call a shape vector that can be associated to each balanced $(n,k,r,c)$ job assignment $D$ as %follows using $\mathfrak{m}^D(m)$ (number of pairs of distinct jobs assigned to precisely $m$ servers) as defined in Equation \eqref{m_D_defn} 

\begin{definition}
Given a balanced $(n,k,r,c)$ job assignment $D$, we define a shape vector $h_D \in \mathbb{N}^{r+1}$ \footnote{In our notation, $\mathbb{N}$ is the set of all non-negative integers including 0.} associated to the assignment $D$ as
\begin{equation}{\label{vec_h_defn}}
    h_D = [\mathfrak{m}^D(0), \mathfrak{m}^D(1), \ldots \mathfrak{m}^D(r)]^T
\end{equation}
\end{definition}

%Thus the shape vector lists the number of pairs of jobs that are assigned together to $m$ servers, for $m = 0, 1, \cdots, r$ and is a vector of length $r+1$. Clearly, the entries of $h_D$ are all non-negative integers. 
Two distinct balanced $(n,k,r,c)$ job assignments $D_1, D_2$ would have the same mean and variance if and only if the corresponding shape vectors $h_{D_1}$ and $h_{D_2}$ are the same. Using equations \eqref{proporty_m_1} and \eqref{property_m_2}, we have 
\begin{equation}{\label{defn_of_A}}
    H h_D = \begin{pmatrix} {n \choose 2} \\ c{k \choose 2} \end{pmatrix} \text{where}, H = \begin{bmatrix}
        1 & 1 & 1 & \cdots & 1 \\
        0 & 1 & 2 & \cdots & r
    \end{bmatrix}
    \end{equation}  

% We first characterize all possible candidate shape vectors in $\mathbb{N}^{r+1}$. Since the entries of the shape vectors are $\mathfrak{m}^D(m)$ arising out of  balanced $(n,k,r,c)$ job assignment, they must satisfy equations \eqref{proporty_m_1} and \eqref{property_m_2}. These can be rewritten as \begin{equation}{\label{defn_of_A}}
%     \begin{bmatrix}
%         1 & 1 & 1 & \cdots & 1 \\
%         0 & 1 & 2 & \cdots & r
%     \end{bmatrix} \begin{pmatrix} \mathfrak{m}^D(0) \\ \mathfrak{m}^D(1) \\ \vdots \\ \mathfrak{m}^D(r) \end{pmatrix} = H h_D = \begin{pmatrix} {n \choose 2} \\ c{k \choose 2} \end{pmatrix}
%     \end{equation}  
% Here the matrix $H = \begin{bmatrix}
%         1 & 1 & 1 & \cdots & 1 \\
%         0 & 1 & 2 & \cdots & r
%     \end{bmatrix}$. 
    
    
    Thus, two possible shape vectors differ by a vector in the kernel of the matrix $H$. Therefore, if one has a particular balanced $(n,k,r,c)$ job assignment $D$ with the corresponding shape vector $h_D$, then all other possible shape vectors can be characterized as vectors $(h_D + v) \in \mathbb{N}^{r+1}$ where $v \in \ker H$. A basis for the kernel of the matrix $H$ is given by the $r-1$ vectors \begin{equation}{\label{basis_ker}} \left\{h_1, h_2, h_3, \cdots, h_{r-2}, h_{r-1} \right\} =  \left\{ \begin{pmatrix} 1 \\ -2 \\ 1 \\ 0 \\ \vdots \\ 0 \\ 0 \\ 0 \end{pmatrix},  \begin{pmatrix} 0 \\ 1 \\ -2 \\ 1 \\  \vdots \\ 0 \\ 0 \\ 0 \end{pmatrix}, \begin{pmatrix} 0 \\ 0 \\ 1 \\ -2 \\ \vdots \\ 0 \\ 0 \\ 0 \end{pmatrix}, \cdots , \begin{pmatrix} 0 \\ 0 \\ 0 \\ 0 \\ \vdots \\ -2 \\ 1 \\ 0 \end{pmatrix}, \begin{pmatrix} 0 \\ 0 \\ 0 \\ 0 \\ \vdots \\ 1 \\ -2 \\ 1 \end{pmatrix} \right\}\end{equation} 
    
    Note that each of these basis vectors $h_i$ have only three nonzero entries. We make use of these basis vectors in determining extremal values of variances that a balanced $(n,k,r,c)$ job assignment can attain. Based on the shape vectors, we now define certain special kinds of balanced $(n,k,r,c)$ job assignments.

\begin{definition}{\label{minimal_compact}}
 A balanced $(n,k,r,c)$ assignment $D$ is compact if the corresponding shape vector $h_D$ has at most two non-zero elements.   
\end{definition}

Under certain special conditions, there is a possibility that the shape vector $h_D$ has only one nonzero entry. Of course, in this special case, every possible pair of jobs is assigned together to $m$ servers, where $m = \frac{ck(k-1)}{n(n-1)} = r\frac{k-1}{n-1}$. Clearly, the dependence of $m$ on the values of $n,k,r$ forces such a possibility to be rare. So in general, compact balanced $(n,k,r,c)$ job assignments have two nonzero entries. 

%We further divide it into 2 categories i.e. proximally minimally compact and stretched minimally compact assignments.


\begin{definition}{\label{proximally_minimal_compact}}
    A balanced assignment $D$ is proximally compact if the shape vector $h_D$ has either exactly one nonzero entry or has exactly two consecutive nonzero entries.    
\end{definition}

\begin{namedlemma}{Lemma}{\label{lemma_on_l_proximally_minimal}}
    For proximally compact $(n,k,r,c)$ assignment $D$, we have $\ell=\Bigl\lfloor\frac{r(k-1)}{n-1}\Bigr\rfloor$ where $\ell$ denotes the index of the smallest non-zero entry in the shape vector $h_D$.
    %\Bigl\lfloor\dfrac{1}{2}\Bigr\rfloor
\end{namedlemma}

\begin{proof}


For a proximally compact $(n,k,r,c)$ assignment $D$, if the shape vector has only one nonzero entry, then $\mathfrak{m}^D(\ell) = {n \choose 2}$. As the total number of job pairs at the $c$ servers is $c{k \choose 2}$, therefore using \eqref{property_m_2}, we have $\ell = \frac{c{k \choose 2}}{{n \choose 2}} = \frac{r(k-1)}{n-1}$. 

On the other hand, if a proximally compact $(n,k,r,c)$ assignment $D$, has a shape vector with exactly two consecutive nonzero entries, then $\mathfrak{m}^D(m)$ is zero for all $m\neq \ell,\ell+1$ for some $\ell$. Using \eqref{proporty_m_1}, we have $\mathfrak{m}^D(\ell+1) = {{n \choose 2}}- \mathfrak{m}^D(\ell)$ and by \eqref{property_m_2}, we get  $\ell(\mathfrak{m}^D(\ell)) + (\ell+1)({{n \choose 2}}- \mathfrak{m}^D(\ell)) = c{{k\choose 2}}$. Thus we can conclude that  $\ell {{n \choose 2}} \leq c{{k \choose 2}}$ and $(\ell +1){{n \choose 2}} > c{{k \choose 2}}$ (as $\mathfrak{m}^D(\ell)>0$) and therefore $\ell=\Bigl\lfloor\frac{c.{{k \choose 2}}}{{{n \choose 2}}}\Bigr\rfloor = \Bigl\lfloor\frac{r(k-1)}{n-1}\Bigr\rfloor$.
\end{proof}

 %By Lemma~\ref{lemma_on_l_proximally_minimal}, it is clear that there can be only one shape vector in $\mathbb{N}^{r+1}$ that satisfies the condition of proximal compactness. One can therefore conclude that there is at most only one proximally compact balanced $(n,k,r,c)$ job assignment.   
Given $n,k,r,c$ it is not clear whether a balanced $(n,k,r,c)$ job assignment which is proximally compact exists. The special case of the shape vector having only one nonzero entry corresponds to the case of balanced incomplete block designs (BIBD) \cite{doi:10.1111/j.1469-1809.1939.tb02219.x,10.5555-1202540}. Balanced incomplete block designs is a very well studied subject. For the sake of completeness, we give the definition of BIBD below.

\begin{nameddefinition}{Defintion}
    (BIBD $(v,b,r,k,\lambda)$ scheme as in \cite{10.5555-1202540}) - A balanced incomplete block design (BIBD) is a pair $(V, B)$ where V is a $v$-set and B
is a collection of $b$ $k$-sized subsets of $V$ (blocks) such that each element of $V$ is contained
in exactly $r$ blocks and any 2-subset of V is contained in exactly $\lambda$ blocks.
\end{nameddefinition}

Note that we can associate the set $V$ to the set of jobs $\mathcal{A}$. Thus $v$ is the same as $n$ that we have employed so far. Each $k$ sized subset of $V$ (or $\mathcal{A}$) can be identified to the set of jobs assigned to a server. The number $r$ has the same interpretation as in our case. Since $B$ is a collection of $b$  $k$-sized sets, we can think of the number of servers $c$ being equal to $b$. Finally $\lambda = \frac{r(k-1)}{n-1}$. Thus $(n,k,r,c)$ in our case is the same as $(v,b,r,k,\lambda)$ quoted in the definition of BIBD above.  %{\color{red} It is known that if $\lambda$ so calculated is a positive integer, then a BIBD exists and there is substantial work about how to construct these BIBDs.  Comment SS- Don't think this statement is true.}


Even in cases where $n,k,r$ may lead to a  $\lambda$ which is a positive integer,  it is not known whether a BIBD always exists. However, multiple constructions of BIBD for various parameters have been described in \cite{doi:10.1111/j.1469-1809.1939.tb02219.x} using various techniques, like vector sub-spaces over finite fields etc. The famous Bruck-Ryser-Chowla theorem in \cite{sprott1955} gives some necessary conditions on $n,k,r$ that guarantees the existence of a BIBD.


Proximally compact assignments may be thought of as a generalization of BIBDs that do not insist on a unique number $\lambda$, that represents the number of servers to be shared by every pair of jobs. Instead proximally compact assignments allow every pair of jobs to be assigned to either $\ell$ or $\ell+1$ servers. As remarked earlier, Lemma~\ref{lemma_on_l_proximally_minimal} ensures that given $n,k,r,c$ there is a unique shape vector that can be constructed and therefore at most only one proximally compact assignment can exist.  We now provide an example of a proximally compact assignment scheme that is not a BIBD. %Example \ref{proximally_compact_Example} of a proximally minimally compact assignment scheme

\begin{example}{\label{proximally_compact_Example}} {\rm
    Consider balanced $(9,3,3,9)$ assignment schemes. In this case, $\frac{r(k-1)}{n-1} = \frac{3}{4}$ and so there is no BIBD possible. Further, $\ell = 0$ and the corresponding shape vector for a possible proximally compact assignment should be $h_D = [9, 
 27, 0, 0]^T$. We display an assignment scheme in Table \ref{proximally_minimally_compact_design} whose shape vector is indeed $h_D$. Note that in this scheme, 27 pairs of jobs are assigned together to a server once and there are 9 pairs of jobs that were never assigned together.}    % $h_D = \begin{pmatrix} 9 \\ 27 \\ 0 \\ 0 \end{pmatrix}$. 
    
 
\end{example}


\begin{table}[!h]
    \centering
{
	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c| } 
		\hline
	{{\diagbox[width = 5 em]{Jobs}{Servers}}}& $s_1$ & $s_2$ & $s_3$ & $s_4$ & $s_5$ & $s_6$ &$s_7$ & $s_8$ & $s_9$ \\
    \hline
    $a_1$ & 1 & 1 & 1 & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$ \\
    \hline
    $a_2$ & $\text{}$ & $\text{}$ & $\text{}$ & 1 & 1 & 1 & $\text{}$ & $\text{}$ & $\text{}$ \\
    \hline
     $a_3$ & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$ & 1 & 1 & 1 \\
        \hline
    $a_4$ & 1 & $\text{}$ & $\text{}$ & 1 & $\text{}$ & $\text{}$ & 1 & $\text{}$ & $\text{}$\\
    \hline
    $a_5$ & $\text{}$ & 1 & $\text{}$ & $\text{}$ & 1 & $\text{}$ & $\text{}$ & 1 & $\text{}$\\
    \hline
     $a_6$ & $\text{}$ & $\text{}$ & 1 & $\text{}$ & $\text{}$ & 1 & $\text{}$ & $\text{}$ & 1\\
    \hline
    
    $a_7$ & 1 &  $\text{}$ & $\text{}$ & $\text{}$ & 1 & $\text{}$ & $\text{}$ & $\text{}$ & 1 \\
    \hline
    $a_8$ & $\text{}$ & 1 & $\text{}$ & $\text{}$ & $\text{}$ & 1 & 1 & $\text{}$ & $\text{}$\\
    \hline
    $a_9$ & $\text{}$ & $\text{}$ & 1 & 1 & $\text{}$ & $\text{}$ & $\text{}$ & 1 & $\text{}$ \\
        \hline
     
        
	\end{tabular}
 }
	\vspace{1 em}
	\caption{Assignment of jobs to servers in a proximally minimally compact $(9,3,3,9)$ assignment scheme}
        \label{proximally_minimally_compact_design}
	
\end{table}


%The construction of BIBD's has been broadly studied and there are multiple constructions using \cite{doi:10.1111/j.1469-1809.1939.tb02219.x}. We could use vector sub-spaces or other techniques to construct some of them. The famous Bruck-Ryser-Chowla theorem in \cite{sprott1955} gives some necessary conditions on $n,k,c,r$ so that it might be possible to have a balanced symmetric design.

\begin{theorem}{\label{min_var}}
 If a proximally compact balanced $(n,k,r,c)$ job assignment exists, then it has the least variance amongst all balanced $(n,k,r,c)$ job assignments. 
\end{theorem}

A proof sketch is presented below. A detailed proof is given in Appendix \ref{sec:min_var_proof}. Recall that in our notation $\mathbb{N}$ denotes the set of all non-negative integers including 0.

\begin{proof}[Proof Sketch]
Let $h_D$ be the shape vector corresponding to the proximally compact balanced $(n,k,r,c)$ job assignment. Thus $h_D(i) = 0$ for all $i \le \ell$ and $i > \ell + 2$ for $\ell$ as calculated in Lemma~\ref{lemma_on_l_proximally_minimal}.   Any balanced $(n,k,r,c)$ job assignment $D_1$ would have a shape vector $h_D + v$ where $v \in \ker H$ with matrix $H$ as defined in \eqref{defn_of_A}. Observe from the expression of variance in \eqref{var_sim_exp} that it is only the term $\sum\limits_{m=0}^{r}\mathfrak{m}^D(m)g(m,x)$ that varies amongst the different balanced $(n,k,r,c)$ assignments. Thus it is enough to show that for every permissible $v \in \ker H$ mentioned above,  $\sum\limits_{m=0}^{r}v(m+1)g(m,x) \ge 0$, in order to conclude that the proximally compact balanced $(n,k,r,c)$ assignment has the least variance.

We therefore first characterize $v \in \ker H$ that may appear from some balanced $(n,k,r,c)$ assignment. As both the shape vectors $h_D, h_D+v \in \mathbb{N}^{r+1}$, therefore $v(i) \ge 0$ for all $i \neq \ell+1, \ell + 2$. Further, as $v \in \ker H$, therefore $\sum\limits_{i=1}^{r+1} v(i) = 0$ and so if $v$ is a nonzero vector, then at least one of $v(\ell+1), v(\ell+2)$ must be a negative integer. As $v \in \ker H$, therefore $v$ can be expressed in terms of the basis vectors $\left\{h_i\right\}$ listed in \eqref{basis_ker}. Let $v = \sum\limits_{i=1}^{r-1}\alpha_ih_i$ and we show \footnote{A detailed proof proving non-negativity of $\alpha_i$ is in Appendix \ref{sec:min_var_proof}} that all $\alpha_i \in \mathbb{N}$.

% Consider the components of $v$ for $i \le \ell$. Let $j$ be the smallest index where $v(j) > 0$ and $j \le \ell$. Then one can inductively argue that $\alpha_i = 0$ for all $i < j$ by starting with $i=1$ as $v(i) = 0$ for $i < j$. Further, $\alpha_j = v(j) > 0$. Now, $v(j+1) = \alpha_{j+1} -2\alpha_j \ge 0$ implies that $\alpha_{j+1} \ge 2\alpha_j$. Similarly, $v(j+2) = \alpha_{j+2} - 2\alpha_{j+1} + \alpha_j$, which implies $\alpha_{j+2} \ge 2\alpha_{j+1} - \alpha_{j} \ge 3\alpha_j$ as $v(j+2) \ge 0$. On the same lines, $\alpha_{j+3} \ge 2\alpha_{j+2} - \alpha_{j+1} \ge 2(2\alpha_{j+1} - \alpha_j) - \alpha_{j+1} = 3\alpha_{j+1} - 2\alpha_j \ge 4\alpha_j$. Inductively, one can show that $\alpha_{j+k} \ge (k+1)\alpha_j$ for all $k \le (\ell - j)$. Thus $\alpha_i \ge 0$ for all $1 \le i \le \ell$. This accounts for all $v(i) \ge 0$ for $i \le \ell$. 

% Similarly, one can utilize $v(i) \ge 0$ for $i > \ell+2$ to conclude that $\alpha_i \ge 0$ for $\ell + 1 \le i \le r-1$, by proceeding from the other end. Let $j$ now be the largest index where $v(j) > 0$ and $j > \ell+2$. If $j < r+1$, then $v(r+1) = 0$ forces $\alpha_{r-1} = 0$. Once again, one can inductively argue that $\alpha_i = 0$ for $j-1 \le i \le r-1$ as the corresponding $v(i+2) = 0$. Further, $\alpha_{j-2} = v(j) > 0$. Now, $v(j-1) = \alpha_{j-3} - 2\alpha_{j-2} \ge 0$ implies that $\alpha_{j-3} \ge 2\alpha_{j-2}$. Using $v(j-2) \ge 0$, one obtains $\alpha_{j-4} \ge 2\alpha_{j-3} - \alpha_{j-2} \ge 3\alpha_{j-2}$. Reflecting the argument used before, one can conclude that $\alpha_{j-2-k} \ge (k+1)\alpha_{j-2}$ for $0 \le k \le (j - \ell - 3)$ and so $\alpha_i \ge 0$ for $\ell + 1 \le i \le r-1$. Thus all $\alpha_i \in \mathbb{N}$.

% %It is easy to see that as $v(i) \ge 0$ for $i \neq \ell+1,\ell+2$, therefore $v = \sum\limits_{i=1}^{r-1}\alpha_ih_i$ where $\left\{h_i\right\}$ are the basis vectors of $\ker H$ and $\alpha_i \in \mathbb{N}$ for $i=1,2,\cdots,(r-1)$. 

As a result, we get \begin{eqnarray*}
    \sum\limits_{m=0}^{r} v(m+1)g(m,x) = \sum\limits_{i=1}^{r-1} \alpha_i \left( g(i-1,x) -2g(i,x) + g(i+1,x) \right)
\end{eqnarray*}
By Lemma~\ref{g_p_diff_lemma}, we know that $g(m+1,x) - g(m,x) = {{c-2} \choose {x-1}} - 2{{c-r-1} \choose {x-1}} + {{c-2r+m} \choose {x-1}}$ and therefore \begin{eqnarray}
    g(i-1,x) -2g(i,x) + g(i+1,x) & = & \left(g(i+1,x) - g(i,x)\right) - \left( g(i,x) - g(i-1,x) \right) \nonumber \\
    & = & {{c-2r+i} \choose {x-1}} -  {{c-2r+i-1} \choose {x-1}} \nonumber \\ & = & \frac{x-1}{c-2r+i-x+1}{{c-2r+i-1} \choose {x-1}} \ge 0
\end{eqnarray}
Thus we have \begin{eqnarray}{\label{ineq_gre}}
    \sum\limits_{m=0}^{r} v(m+1)g(m,x) & = & \sum\limits_{i=1}^{r-1} \alpha_i \left( g(i-1,x) -2g(i,x) + g(i+1,x) \right) \nonumber \\ & = & \sum\limits_{i=1}^{r-1} \frac{\alpha_i(x-1)}{c-2r+i-x+1}{{c-2r+i-1} \choose {x-1}} \ge 0
\end{eqnarray}
As the above is true for every permissible $v \in \ker H$ such that $h_D + v$ is a shape vector, therefore we conclude that proximally compact balanced $(n,k,r,c)$ assignment has the least variance amongst all balanced $(n,k,r,c)$ assignments.
\end{proof}

The above theorem guarantees that if a proximally compact balanced $(n,k,r,c)$ assignment exists, then it has the least variance. Also note from \eqref{ineq_gre} that for the case $x = 1$, the contribution due to every permissible $v \in \ker H$ is zero and so all shape vectors give the same variance, which is zero. That is consistent with what we have shown earlier. Similarly, note that for $x > c - r$, every ${{c-2r+i-1}\choose {x-1}}$ is zero and therefore from \eqref{ineq_gre} we can conclude that every balanced $(n,k,r,c)$ assignment has the same variance when one considers the cases of $x > c-r$. 

We now provide an example of  $(n,k,r,c)$ that does not have a proximally compact assignment.

\begin{example}{\rm
Consider balanced $(10,5,4,8)$ assignments. Here $\frac{r(k-1)}{n-1} = \frac{16}{9}$ and so the shape vector must have at least two nonzero entries. Moreover, $\ell = 1$ and the corresponding shape vector for a possible proximally compact assignment should be $h_D = [0, 10, 35, 0, 0]^T$. We now show that an assignment with the shape vector $h_D$ does not exist. 

%$h_D = \begin{pmatrix} 0 \\ 10 \\ 35 \\ 0 \\ 0 \end{pmatrix}$.

As every job is assigned to $r=4$ servers, every job is involved in $r(k-1) = 16$ job pairs. Consider the job $a_1$ and let $x$ be the number of other jobs with whom $a_1$ shares only one server. So $9-x$ jobs share two servers each with $a_1$. Clearly $2(9-x) + x = 16$ which implies that $x = 2$. As $a_1$ was an arbitrary choice, we can conclude that every job shares one server with two other jobs and shares two servers with the other $7$ jobs. 

Let $\mathfrak{G} = \left\{a_1, a_2, a_3, \cdots a_i, a_1 \right\}$ be a cycle of jobs such that each job shares only one server with the jobs that are its predecessor and successor in $\mathfrak{G}$. One can now argue that the only permissible lengths of these cycles can be either 5 or 10.\footnote{This follows since there cannot exist a cycle of size 3 i.e. there cannot exist jobs $a,b$ and $c$ such that pairs $(a,b)$, $(b,c)$ and $(c,a)$ share a server each.} Then some more work proves that it is not possible to have an assignment with $h_D= [0, 10, 35, 0, 0]^T$  The actual balanced $(10,5,4,8)$ assignments that have shape vectors closest to $h_D$ have shape vectors $[1, 8, 36, 0, 0]^T$ and $[0, 12, 31, 2, 0]^T$ respectively.  

%$\begin{pmatrix} 1 \\ 8 \\ 36 \\ 0 \\ 0 \end{pmatrix}$ and $\begin{pmatrix} 0 \\ 12 \\ 31 \\ 2 \\ 0 \end{pmatrix}$ respectively.
    }
    %$h_D = \begin{pmatrix} 0 \\ 10 \\ 35 \\ 0 \\ 0 \end{pmatrix}$.
\end{example}

We now define another class of compact assignments.

\begin{definition}{\label{strectched_minimal_compact}}
    A balanced assignment $D$ is stretched compact if the shape vector $h_D$ has non-zero elements only in the first and the last entries.
\end{definition}

If only the first and last entries of the shape vector $h_D$ are nonzero, then by \eqref{defn_of_A} it is clear that the last entry of the shape vector is $\frac{c}{r}{k \choose 2} = \frac{n(k-1)}{2}$ and therefore the first entry of the shape vector is $\frac{n(n-k)}{2}$. Of course, if $n$ is a odd number and $k$ is even, then these calculated quantities are not integers and therefore for such cases, there is no possibility of existence of a stretched compact $(n,k,r,c)$ assignment. Even for the other cases, there is no guarantee that a stretched compact $(n,k,r,c)$ assignment exists even though the shape vector has integer entries.  

\begin{theorem}{\label{max_var}}
 If a stretched compact balanced $(n,k,r,c)$ job assignment exists, then it has the largest variance amongst all balanced $(n,k,r,c)$ job assignments. 
\end{theorem}

This proof goes along very similar lines to that of Theorem \ref{min_var} and we prove in Appendix \ref{sec:max_var_proof}.

% \begin{proof}
%    Let $h_D$ be the shape vector corresponding to a stretched compact balanced $(n,k,r,c)$ job assignment. Then $h_D(i) = 0$ for all $i \neq 1, r+1$. Any balanced $(n,k,r,c)$ job assignment $D_1$ has a shape vector $h_D + v$ where $v \in \ker H$ with $H$ as defined in \eqref{defn_of_A}. Similar to the proof of Theorem~\ref{min_var}, we now characterize $v \in \ker H$ that can arise from some balanced $(n,k,r,c)$ assignment. Note that $v(i) \ge 0$ for all $i \neq 1,r+1$ and $\sum\limits_{i=1}^{r+1} v(i) = 0$. Hence $v(1) \le 0$ and $v(r+1) \le 0$. As $v \in \ker H$, therefore $v = \sum\limits_{i=1}^{r-1}\alpha_ih_i$ where $\left\{h_i\right\}$ is the basis for $\ker H$ as listed in \eqref{basis_ker}. Following the proof of Theorem~\ref{min_var}, it is now enough to show that all $\alpha_i \le 0$ for any permissible nonzero vector $v \in \ker H$ since the expression in \eqref{ineq_gre} would then be rendered negative, thereby signalling a decrease in the variance for all balanced $(n,k,r,c)$ assignments with shape vector $h_D + v$. 

%    Observe that as $v(1) \le 0$, therefore $\alpha_1 = v(1) \le 0$. If $r = 2$, then $\ker H$ is one dimensional and therefore $v(1) = v(3) \le 0$, while $v(2) = -2v(1) \ge 0 \ge v(1)$. If $r > 2$, then as $v(2) \ge 0$ and  $v(2) = \alpha_2 - 2\alpha_1$, therefore $\alpha_2 \ge 2\alpha_1$. Now if $r = 3$, then $\ker H$ is two dimensional and $\alpha_2 = v(4) \le 0$. Further, $v(3) \ge 0$ implies $\alpha_1 - 2\alpha_2 \ge 0$ and therefore $\alpha_1 \ge 2\alpha_2$. Thus again, for $r = 3$, both $\alpha_1, \alpha_2$ are negative and their values are mutually bound by the constraints $\frac{\alpha_1}{2} \ge \alpha_2 \ge 2\alpha_1$ and $\frac{\alpha_2}{2} \ge \alpha_1 \ge 2\alpha_2$.

%    Now, we consider the cases of $r > 3$. In this case, $v(3) \ge 0$ translates to $2\alpha_2 \le \alpha_1 + \alpha_3$. Therefore $4\alpha_2 \le 2\alpha_1 + 2\alpha_3 \le \alpha_2 + 2\alpha_3$ (by using the condition obtained from $v(2) \ge 0$) which in turn translates to $3\alpha_2 \le 2\alpha_3$. From the condition $v(4) \ge 0$, we get $2\alpha_3 \le \alpha_2 + \alpha_4$ which can now be manipulated to $6\alpha_3 \le 3\alpha_2 + 3\alpha_4 \le 2\alpha_3 + 3\alpha_4$ which gives us $4\alpha_3 \le 3\alpha_4$. Following the steps mentioned above, one can use the subsequent $v(k) \ge 0$ to show that $k\alpha_{k-1} \le (k-1)\alpha_k$ for $2 \le k \le (r-1)$. Combining all these inequalities, one gets $\alpha_1 \le \frac{\alpha_2}{2} \le \frac{\alpha_3}{3} \le \cdots \le \frac{\alpha_k}{k} \le \cdots \le \frac{\alpha_{r-1}}{r-1} \le 0$. This proves that all the $\alpha_i \le 0$. 
% \end{proof}

%Interestingly, in the proof above, one could have started from the other end and as already shown for the case $r = 3$, one can get another set of constraints $\alpha_{r-1} \le \frac{\alpha_{r-2}}{2} \le \cdots \le \frac{\alpha_{r-k}}{k} \le \cdots \le \frac{\alpha_1}{r-1} \le 0$. These interwoven constraints restrict the possible values for the $\alpha_i$ where $v = \sum\limits_{i=1}^{r-1}\alpha_ih_i$. 

\begin{example}{\rm
Let us revisit the earlier example of $(10,5,4,8)$ assignments. It is clear that a shape vector corresponding to stretched compact assignment is permissible, namely $h_D= [25, 0, 0, 0, 20]^T$. Such an assignment is indeed possible. Divide the $10$ jobs into two sets of $5$ jobs. Assign each of these sets of jobs to $4$ servers. That results in a total of $20$ pairs sharing $4$ servers each and the rest $25$ pairs consisting of a job each from the two sets sharing no servers. This repetition assignment is a stretched compact assignment and therefore has the largest variance amongst all possible balanced $(10,5,4,8)$ assignments.  %$h_D = \begin{pmatrix} 25 \\ 0 \\ 0 \\ 0 \\ 20 \end{pmatrix}$. 
}
\end{example}

It is clear that this sort of repetition assignment where multiple servers have the same set of jobs assigned is only possible if $k$ divides $n$. In such a situation, one can subdivide the jobs into $\frac{n}{k}$ groups of $k$ jobs each. Each of these groups are repeated at $r$ servers, thus accounting for $\frac{n}{k}r = c$ servers. Thus the number of job pairs that appear together $r$ times is equal to $\frac{n}{k}{k \choose 2} = \frac{n(k-1)}{2}$. And in all these cases, these repetition assignments would correspond to a stretched compact assignment which has the largest variance amongst all balanced $(n,k,r,c)$ assignments.

%With these definitions, we now provide our key results on the least and the largest variance in the number of distinct jobs $d$ at the server.

%\begin{theorem}{\label{min_var_gen}}
 %   The least variance on the number of distinct jobs received at the server for any $x \in [1,c-2r+1]$ is attained uniquely by the proximally minimal compact assignment (if exists) amongst all balanced $(n,k,r,c)$ assignments.

  %  However, for $x>c-2r+1$, the result on least variance still holds without guarantee of uniqueness.
%\end{theorem}

%To prove this theorem, we first prove the following claim on $g(p,x)$ as as defined in Equation \eqref{g_defn}. Observe that this lemma proved some convexity results on $g(p,x)$ specific to case where $p$ is discrete.

\remove{

\begin{namedclaim}{Claim}{\label{Some claims om g(p,x)}}
	Recall the definition of $g(p,x)$ as defined in Equation \eqref{g_defn}. Then, the following can be said (for every $c-2r+1\geq x>1$):
	\begin{itemize}
		\item $\frac{g(m+k_1,x)-g(m,x))}{k_1}>\frac{g(m,x))-g(m-k_2,x)}{k_2}$ $\forall$ $k_1,k_2 \in \mathbbm{N}$.
		\item $\frac{g(m+k_1+v,x)-g(m+v,x)}{k_1}>\frac{g(m+u,x))-g(m-k_2+u,x)}{k_2}$ $\forall$ $k_1,k_2 \in \mathbbm{N}$ with $(k_1,k_2)\neq (1,1)$ and $(u,v) \in \{0,1\}^2$ with $u \neq v$.
		% \item 
		% $\frac{g(m+k_1+1,x)-g(m+1,x)}{k_1}>\frac{g(m,x)-g(m-k_2,x)}{k_2}$ $\forall$ $k_1,k_2 \in \mathbbm{N}$ with $(k_1,k_2)\neq (1,1)$.
		% \item $\frac{g(m+k_1,x)-g(m,x)}{k_1}>\frac{g(m+k_2,x)-g(m,x)}{k_2}$ $\forall$ $k_1, k_2 \in \mathbbm{N}, k_1>k_2$.
	\end{itemize}

However, the inequalities may not strict for $x > c-2r+1$ but maybe {\color{red} attained with equality }
  
\end{namedclaim}

\begin{proof}

We first prove the strict inequalities assuming $x\leq c-2r+1$
 
	\begin{align}{\label{first_ineq}}
	  \frac{g(m+k_1,x)-g(m,x)}{k_1}
	  = \frac{\sum\limits_{i=0}^{i=k_1-1}(g(m+i+1,x)-g(m+i,x))}{k_1}
	 \overset{(a)}{\geq}& \frac{k_1 (g(m+1,x)-g(m,x)}{k_1}\nonumber\\        
     \geq & g(m+1,x)-g(m,x)
     \end{align}


Now consider,
	\begin{align}{\label{second_ineq}}
	\frac{g(m+k_1+1,x)-g(m+1,x)}{k_1}
	= \frac{\sum\limits_{i=1}^{i=k_1}(g(m+i+1,x)-g(m+i,x))}{k_1}
	\overset{(d)}{\geq}& \frac{k_1 (g(m+2,x)-g(m+1,x)}{k_1}\nonumber\\        
	> & g(m+2,x)-g(m+1,x)
	\end{align}
Note $(a)$ and $(d)$ follow since since $g(m+i+1,x)-g(m+i,x) > g(m+1,x)-g(m,x)$ $\forall i \in \mathbbm{N}$ as shown in in Claim \ref{g_p_diff_lemma} where 

$$g(m,x)-g(m-1,x)= \left[{{(c-2) \choose (x-1)}}-2{{(c-r-1) \choose (x-1)}}+ {{(c-2r+m-1)\choose (x-1)}}\right]$$

strictly increases with $m$ for every $c-2r+1>x>1$. Also observe that $(a)$ and $(d)$ would be tight inequalities when $k_1>1$.

Similarly,
  \begin{align}{\label{third_ineq}}
  \frac{g(m,x)-g(m-k_2,x)}{k_2}
  = \frac{\sum\limits_{i=0}^{i=k_2-1}(g(m-i,x)-g(m-i-1,x))}{k_2}
  \overset{(b)}{\leq}& \frac{k_2 (g(m,x)-g(m-1,x)}{k_2}\nonumber\\        
  \leq & g(m,x)-g(m-1,x)
  \end{align}

Similarly,
\begin{align}{\label{fourth_ineq}}
\frac{g(m+1,x)-g(m-k_2+1,x)}{k_2}
= \frac{\sum\limits_{i=0}^{i=k_2-1}(g(m-i+1,x)-g(m-i,x))}{k_2}
\overset{(c)}{\leq}& \frac{k_2 (g(m+1,x)-g(m,x)}{k_2}\nonumber\\        
\leq & g(m+1,x)-g(m,x)
\end{align}


Note $(b)$ and $(c)$ follow since $g(m-i,x)-g(m-i-1,x) \leq g(m,x)-g(m-1,x)$ $\forall i \in \mathbbm{N}$ as shown in Claim \ref{g_p_diff_lemma} where $g(m+1,x)-g(m,x)$ strictly increases with $m$ for every $c-2r+1>x>1$. Also observe that $(b)$ and $(c)$ would be tight inequalities when $k_2>1$.

Thus we can say from Equations \eqref{first_ineq},\eqref{second_ineq},\eqref{third_ineq},\eqref{fourth_ineq} and the fact that $g(m+1)-g(m)$ strictly increases with $m$, the following equations \eqref{result_1},\eqref{result_2},\eqref{result_3}.
\begin{equation}{\label{result_1}}
\frac{g(m+k_1,x)-g(m,x)}{k_1} > \frac{g(m,x)-g(m-k_2,x)}{k_2} \forall k_1,k_2 \in \mathbbm{N}
\end{equation} 

and 

\begin{equation}{\label{result_2}}
\frac{g(m+k_1,x)-g(m,x)}{k_1} > \frac{g(m+1,x)-g(m-k_2+1,x)}{k_2} \forall k_1,k_2 \in \mathbbm{N} \text{ with } (k_1,k_2) \neq (1,1).
\end{equation} 

\begin{equation}{\label{result_3}}
\frac{g(m+k_1+1,x)-g(m+1,x)}{k_1} > \frac{g(m+1,x)-g(m-k_2+1,x)}{k_2} \forall k_1,k_2 \in \mathbbm{N} \text{ with } (k_1,k_2) \neq (1,1).
\end{equation} 


Thus the first and second inequalities in Claim \ref{Some claims om g(p,x)}are precisely the equations \eqref{result_1},\eqref{result_2} and \eqref{result_3}.





% Now consider the following for $k_1>k_2$

% \begin{align*}
% \frac{g(m+k_1,x)-g(m,x)}{k_1} \geq \frac{g(m+k_2,x)-g(m,x)}{k_2}
% \Leftrightarrow \frac{g(m+k_1,x)-g(m+k_2,x)}{k_1-k_2} \geq \frac{g(m+k_2,x)-g(m,x)}{k_2} 
% \end{align*} 
     
% Note that since $k_1>k_2$, we prove the inequality on R.H.S from Equation \eqref{result_1}. Thus, the fourth inequality in Claim \ref{Some claims om g(p,x)} holds true.


Observe that for $x> c-2r+1$, the function $g(m+1,x)-g(m,x)$ is not strictly increasing with $m$ as the last term ${{c-2r+m-1 \choose x-1}}$ maybe zero when $m$ equals $0$ or $1$ and thus the inequalities in the lemma maybe attained with equality.
\end{proof}




With this convexity result on $g(m,x)$, we now prove Theorem \ref{min_var_gen}. 


\begin{proof}
	
%Recall $y$ from the definition in Claim \ref{var_equal}. $y$ denotes the number of servers a pair of jobs chosen uniformly at random is present together. Now we know that var$(y)$ = $\sigma_{D,2}(d)$ from Claim \ref{var_equal}. Now we know from theorem \ref{mean_equality} that  $\mathbbm{E}_{D,2}[d]= 2.k - \frac{n.\sum\limits_{t=1}^{r-1} t{r \choose (t+1)} {(c-r) \choose (2-t-1)}}{{c \choose 2}} =  2k - \frac{n{r \choose 2}}{{c \choose 2}}$ whereas $\mathbbm{E}[y]= \frac{\sum\limits_{p=0}^{r}p.\mathfrak{n}^D_{p,D}}{{n \choose 2}} = \frac{c.{{k \choose 2}}}{{{n \choose 2}}}$.
%
%The number of common jobs $c$ can be written as $2k-d$ when $x=2$ servers return.
%
%Thus var$(y)$ = $\sigma_{D,2}(c)$, $\mathbbm{E}_{D,2}(c)=\mathbb{E}[y] = \frac{n.{{k \choose 2}}}{{{n \choose 2}}}$ which is fixed for a given $n,k$. Thus $l = \floor*{\frac{n.{{k \choose 2}}}{{{n \choose 2}}}} $ as $c$ takes values only $l$ or $l+1$.
%
%Note that random variable $y$ and $c$ can take only integer values, since in this case $c$ takes only 2 consecutive integer values, variance of $c$ is the least possible for a given $\mathbbm{E}_{D,2}[c]$.
%
%However this least variance can only be achieved for $y$ if random variable $y$ also takes values $l$ or $l+1$ as it also has the same expectation and variance as that of $c$.    

Recall the definition of $\mathfrak{m}^D(m)$ from Equation \eqref{m_D_defn} which denotes the number of pairs of jobs that are assigned together to exactly $m$ servers with $D$ denoting any proximally minimally compact design.

Now we know that $\mathfrak{m}^{D}(m) = 0$ only for $m\neq l,l+1$ for any proximally minimally compact $(n,k,r,c)$ assignment scheme. This would ensure that $l= \floor{\frac{c.{{k \choose 2}}}{{{n \choose 2}}}}$ as shown in Lemma \ref{lemma_on_l_proximally_minimal}.



%Now consider any other distribution $D_1$. 
%%Using the proof techniques similar to that of last part of Theorem \ref{min_var} we can say that $D$ gives least variance on number of distinct jobs for every $x$.  


Let us consider another job assignment ${D}_1$ which is a balanced $(n,k,r,c)$ assignment scheme.
 
%Since we know that $\mathfrak{n}^D_{p,D_1}$ = 0

%Recall the definition of $g(p,x)$ as defined in Claim \ref{f_defn}. %Let us denote it as $g_x(p)$ as it is only a function of $p$.

First observe that $\sum\limits_{m=0}^{r} \mathfrak{m}^D(m) = \sum\limits_{m=0}^{r} \mathfrak{m}^{D_1}(m) = {{n \choose 2}}$ which follows from Equation \eqref{proporty_m_1} and $\sum\limits_{m=0}^{r} m \times \mathfrak{m}^D(m) = \sum\limits_{m=0}^{r} m \times \mathfrak{m}^{D_1}(m)= c {{k \choose 2}}$ follows from Equation \eqref{property_m_2}.

We thus have 

\begin{equation}{\label{conditions_no_pairs}}
    \sum\limits_{m=0}^{r} \mathfrak{m}^D(m) = \sum\limits_{m=0}^{r} \mathfrak{m}^{D_1}(m) = {{n \choose 2}} \text{ and } \sum\limits_{m=0}^{r} m \times \mathfrak{m}^D(m) =\sum\limits_{m=0}^{r} m \times \mathfrak{m}^{D_1}(m)= c {{k \choose 2}}
\end{equation}

We now consider four different cases and in each of these cases, we show that the variance is the least for the assignment $D$. Also, we first consider the case where $x\leq c-2r+1$ to prove that least variance is uniquely attained by proximallyminimally compact assignments.


\begin{itemize}
	\item Case 1: $\mathfrak{m}^{D_1}(l) \geq \mathfrak{m}^{D}(l)$ but $\mathfrak{m}^{D_1}(l+1) \geq \mathfrak{m}^{D_1}(l+1)$

Note that $\mathfrak{m}^{D_1}(m) \geq \mathfrak{m}^D(m) \forall m \in [r]$ which follows since $\mathfrak{m}^D(m)=0 \forall m \neq l,l+1$. However, equation \eqref{conditions_no_pairs} would imply that $\mathfrak{m}^{D}(m)= \mathfrak{m}^{D_1}(m)$ $\forall$ $m \in [r]$ which would imply distribution $D_1$ has same variance of distinct jobs as that of distribution $D$ which follows from Equation \ref{var_sim_exp} in Theorem \ref{result_variance} as the variance $\sigma_{D,x}$ is just a function of $\mathfrak{m}^D(.)$ other than design parameters $n,k,r$ and $c$.


\item Case 2: $\mathfrak{m}^{D_1}(l) < \mathfrak{m}^{D}(l)$ but $\mathfrak{m}^{D_1}(l+1) \geq \mathfrak{m}^{D_1}(l+1)$
	
	
	
Let us denote $x_m=\mathfrak{m}^{D_1}(m)-\mathfrak{m}^{D}(m)$ $\forall m \in [0,r]$. Clearly, $x_m < 0$ only for $m=l$ as for every $m \neq l,l+1$ we have $\mathfrak{m}^D(m)=0$
	
%	Now we know that $\sum\limits_{p=0}^{r} p.\mathfrak{n}^D_{p,D}= \sum\limits_{p=0}^{r} p.\mathfrak{n}^D_{p,D_1}=n{k \choose 2}$ implying $\sum\limits_{p=0}^{r} p.x_p=0$. Similarly, we can also argue $\sum\limits_{p=0}^{r} x_p=0$.

Observe that equation \eqref{conditions_no_pairs} ensures that $\sum\limits_{m=0}^{r} x_m = \sum\limits_{m=0}^{r} m \times x_m = 0$. 
	
 
 Let us denote $\sum\limits_{m=0}^{l-1} x_m =x$ and $\sum\limits_{m=l+1}^{r} x_m =y$. Since $\sum\limits_{m=0}^{r} x_m=0$, we can say that $x_l= -(x+y)$.
	
	Thus,
 
 \begin{equation}{\label{temp1}}
    \sum\limits_{m=0}^{r} m.x_m =0 \Leftrightarrow (x+y)l = \sum\limits_{m=l+1}^{r} m\times x_m+\sum\limits_{m<l}m\times x_m \Leftrightarrow \sum\limits_{m=l+1}^{r} x_m\times (m-l) = \sum\limits_{q=0}^{l-1} x_q\times (l-q)     
 \end{equation}

	
	However, we know from Claim \ref{Some claims om g(p,x)} that  

 \begin{equation}{\label{temp2}}
     \frac{g(m,x)-g(l,x)}{m-l} > \frac{g(l,x)-g(q,x)}{l-q} \forall m>l>q
 \end{equation}
	
These equations \eqref{temp1} and \eqref{temp2} and the fact that $x_m \geq 0$ for $m\neq l, m \in [0,r]$ above would imply:
	\begin{align}{\label{temp_eqn_variance_case1}}
    \sum\limits_{m=l+1}^{r} x_m (g(m,x)-g(l,x)) > \sum\limits_{q=0}^{l-1} x_q (g(l,x)-g(q,x))
	\overset{(c)} {\Leftrightarrow} & \sum\limits_{\substack{m \neq l\\ m \in [0,r]}} x_m.g(m,x) - \sum\limits_{\substack{m \neq l\\ m \in [0,r]}} x_m g(l,x)>0\nonumber \\
	\Leftrightarrow & \sum\limits_{\substack{m \neq l\\ m \in [0,r]}} x_m.g(m,x) + x_l.g(l,x) >0\nonumber\\
	{\Leftrightarrow} & \sum\limits_{m=0}^{r} x_m g(m,x)>0\nonumber \\
	\overset{(f)}{\Leftrightarrow} & \sum\limits_{m=0}^{r} \mathfrak{m}^{D_1}(m) g(m,x) > \sum\limits_{m=0}^{r} \mathfrak{m}^{D}(m) g(m,x)
	\end{align}
	
	Note $(c)$ follows since $\sum\limits_{m =0}^{r} x_m=0$ and $(f)$ follows from the fact that $x_m= \mathfrak{m}^{D_1}(m) - \mathfrak{m}^{D}(m)$
%%	 $ which would imply $\sum\limits_{p=0}^{r} x_p.g(p,x)$.

%Since the numerator of the first term in $\sigma_{D,x}(d)$ is 
Now let us consider the numerator of the first term in $\sigma_{{D},x}(d)$ as in theorem \ref{var_sim_exp} which can be written as $2.\sum\limits_{m=0}^{r}\mathfrak{m}^{D}(m)g(m,x) + n.\left(\sum\limits_{t=1}^{r-1} t^2{r \choose (t+1)} {(c-r) \choose (x-t-1)}\right)$.

%Now we consider this expression for $D$ = $D$ and $D_1$.
Thus the inequality proven in equation \eqref{temp_eqn_variance_case1} would imply that distribution $D_1$ has higher variance of number of distinct jobs received than that of distribution $D$. 

\item Case 3: $\mathfrak{m}^{D_1}(l+1) < \mathfrak{m}^{D}(l+1)$ but $\mathfrak{m}^{D_1}(l) \geq \mathfrak{m}^{D}(l)$

Note this can be proven in a very similar way as that of Case 2. The entire proof could be done for $l+1$ instead of $l$

\item Case 4: $\mathfrak{m}^{D_1}(l+1) < \mathfrak{m}^{D}(l+1)$ and  $\mathfrak{m}^{D_1}(l) < \mathfrak{m}^{D}(l)$

Let us denote $x_m=\mathfrak{m}^{D_1}(m)-\mathfrak{m}^{D}(m)$ $\forall m \in [0,r]$. Clearly, $x_m < 0$ only for $m=l,l+1$.
	
Now equation \eqref{conditions_no_pairs} ensures that $\sum\limits_{m=0}^{r} m\times x_m=0$ and $\sum\limits_{m=0}^{r} x_m=0$.
	

Let us denote $\sum\limits_{m=0}^{l-1}x_m =\alpha_1+\alpha_2$ and $\sum\limits_{m=l+2}^{r} x_m=\beta_1+\beta_2$. Since $\sum\limits_{m=0}^{r} x_m=0$, we can say that 


\begin{equation}{\label{temp_10}}
    x_l= -(\alpha_1+\beta_1) \text{ and } x_{l+1}=-(\alpha_2+\beta_2) \text { for some }\alpha_1,\beta_1,\alpha_2,\beta_2 \in \mathbbm{N}
\end{equation}

Now define $[y_m]_{m=0}^{r}$ and $[z_m]_{m=0}^{r}$as follows below.

\begin{itemize}
    \item $y_m = x_m \times \frac{\alpha_1}{\alpha_1+\alpha_2}$ and $z_m = x_m \times \frac{\alpha_2}{\alpha_1+\alpha_2}$ if $0\leq m<l$ 
    \item $y_m=x_m\times \frac{\beta_1}{\beta_1+\beta_2}$ and $z_m=x_m\times \frac{\beta_2}{\beta_1+\beta_2}$
   for $l+1<m\leq r$
   \item $y_m= \alpha_1$ and $z_m = \alpha_2$ if $m=l$
   \item $y_m= \beta_1$ and $z_m = \beta_2$ if $m=l+1$
\end{itemize}
			

%\newline
	

   
   Thus,
   
   $\sum\limits_{m=l+2}^{r} y_m=\beta_1$ ; $\sum\limits_{m=l+2}^{r} z_m=\beta_2$; $\sum\limits_{m=0}^{l-1}y_m=\alpha_1$ ; $\sum\limits_{m=0}^{l-1}z_m=\alpha_2$;	
   	
   %Choose $y_l=-x_1$ and $z_l=-x_2$ and 	
   	
	Thus $\sum\limits_{m=0}^{r} mx_m =0$ implies the following set of conditions.
	
	\begin{align}{\label{temp3}}
      & (\alpha_1+\beta_1)l+(\alpha_2+\beta_2)(l+1) = \sum\limits_{m=l+2}^{r}m\times x_m+\sum\limits_{m=0}^{l-1}m\times x_m \nonumber\\
    & \overset{(d)}{\Leftrightarrow} \left(\sum\limits_{m=l+2}^{r} y_m + \sum\limits_{m=0}^{l-1} y_m\right)l+\left(\sum\limits_{m=l+2}^{r} z_m + \sum\limits_{m=0}^{l-1} z_m\right)(l+1) = \sum\limits_{m=l+2}^{r}m\times (y_m+z_m)+\sum\limits_{m=0}^{l-1}m\times (y_m+z_m)\nonumber\\
     & {\Leftrightarrow} \sum\limits_{m=l+2}^{r} y_m(m-l)+ \sum\limits_{m=l+2}^{r} z_m(m-l-1) = \sum\limits_{q=0}^{l-1} y_q(l-q) + \sum\limits_{q=0}^{l-1} z_q(l+1-q)
	\end{align}
	
Note $(d)$ follows since 

i) $y_m+z_m = x_m \forall m \in [0,l-1] \cup [l+2,r]$, ii) $\sum\limits_{m=l+2}^{r} y_m + \sum\limits_{q=0}^{l-1} y_q = (\alpha_1+\beta_1)$ and \\
iii) $\sum\limits_{m=l+2}^{r} z_m + \sum\limits_{q=0}^{l-1} z_q = (\alpha_2+\beta_2)$ \\
	
	Now we can say from Claim \ref{Some claims om g(p,x)} that 
	
\begin{equation}{\label{temp4}}
    \frac{g(m,x)-g(t,x)}{m-t}> \frac{g(u,x)-g(q,x)}{u-q}
	\text{ }\forall m>l+1, q< l \text{ and } t,u \in \{l,l+1\}.
 \end{equation}
	
	
Thus we can say the following from equations \eqref{temp3} and \eqref{temp4} and the fact that $x_m,y_m,z_m>0$ for $m \in [0,r]; m \neq \{l,l+1\}$.
	
	\begin{align}{\label{temp_eqn_variance_case2}}
	 & \sum\limits_{m=l+2}^{r} y_m(g(m,x)-g(l,x))+  \sum\limits_{m=l+2}^{r} z_m(g(m,x)-g(l+1,x))\\ & > \sum\limits_{q=0}^{l-1} y_q(g(l,x)-g(q,x)) + \sum\limits_{q=0}^{l-1} z_q(g(l+1,x)-g(q,x))\\
	& \overset{(e)}{\Leftrightarrow} \sum\limits_{\substack{m \neq l,l+1\\ m \in [0,r]}} (y_m+z_m) g(m,x)+ (\alpha_1+\beta_1) g(l,x) + (\alpha_2+\beta_2) g(l+1,x)>0\\
	& \overset{(g)}{\Leftrightarrow} \sum\limits_{\substack{m \neq l,l+1\\ m \in [0,r]}} x_m.g(m,x)+ x_l.g(l,x) + x_{l+1}.g(l+1,x)>0\\
	& \Leftrightarrow \sum\limits_{m=0}^{r} x_m.g(m,x)>0\\
    & \overset{(h)}{\Leftrightarrow} \sum\limits_{m=0}^{r} \mathfrak{m}^{D_1}(m) g(m,x) > \sum\limits_{m=0}^{r} \mathfrak{m}^{D}(m) g(m,x)
	\end{align}
	
Note $(e)$ follows since $\sum\limits_{m=l+2}^{r} y_m + \sum\limits_{q=0}^{l-1} y_q = (\alpha_1+\beta_1)$ and $\sum\limits_{m=l+2}^{r} z_m + \sum\limits_{q=0}^{l-1} z_q = (\alpha_2+\beta_2)$ from Equation \eqref{temp_10} and the fact $y_m+z_m=x_m \forall m \in [0,l-1] \cup [l+2,r]$. \\ $(g)$ follows from the fact that $x_l=-(\alpha_1+\beta_1)$ and $x_{l+1}=-(\alpha_2+\beta_2)$ $(h)$ follows from the fact that that $x_m=\mathfrak{m}^{D_1}(m)-\mathfrak{m}^{D}(m)$ 	
	
Now let us consider the numerator of the first term in $\sigma_{{D},x}(d)$ as in theorem \ref{var_sim_exp} which can be written as $2.\sum\limits_{m=0}^{r}\mathfrak{m}^{D}(m)g(m,x) + n.\left(\sum\limits_{t=1}^{r-1} t^2{r \choose (t+1)} {(c-r) \choose (x-t-1)}\right)$.

%Now we consider this expression for $D$ = $D$ and $D_1$.
Thus the inequality proven in the previous equation \eqref{temp_eqn_variance_case2} would imply that distribution $D_1$ has higher variance of number of distinct jobs received than that of distribution $D$.  	


Note that other than Case 1 in this proof (where we show $D_1$ is also a proximally minimally compact assignment), the distribution $D_1$ is not a proximally minimally compact assignment and we show strict optimality of proximally minimally compact assignment over any other balanced assignment for $x \leq c-2r+1$. However, if $x > c-2r+1$, the inequalities still hold but are not strict as it follows from Claim \ref{Some claims om g(p,x)}.

Combining these statements, we prove the strict optimality (attains least variance )of pairwise balanced designs for $x\leq c-2r+1$ and weak optimality for $x>c-2r+1$
	
	
\end{itemize}
 

\end{proof}	






\begin{theorem}{\label{max_var_gen}}
    The largest variance on the number of distinct jobs received at the server for any $x \in [1,c-2r+1]$ is attained uniquely by the stretched minimally compact design (if exists) amongst all balanced $(n,k,r,c)$ assignments.

    However, for $x>c-2r+1$, the result on the largest variance still holds without guarantee of uniqueness.
\end{theorem}


We also prove this theorem using the convexity property of $g(m,x)$ as shown in Claim \ref{Some claims om g(p,x)}.




%\section{Construction of $\vec{h^D}$}




% With this setup, we now study assignment schemes on when the least variance on the number of distinct jobs $d$ is attained. We specifically propose pairwise balanced designs discussed in Definition \ref{pair_job_balanced_definition} and \ref{pair_server_balanced_definition}  in Theorem \ref{min_var_gen} and \ref{min_var_gen_spec} and show that it attains the least variance amongst the class of balanced assignments. We now compare  this definition to balanced incomplete block designs (BIBD) \cite{doi:10.1111/j.1469-1809.1939.tb02219.x,10.5555-1202540} and show that it is a generalization of the same.

% \begin{nameddefinition}{Defintion}
%     (BIBD $(v,b,r,k,\lambda)$ scheme as in \cite{10.5555-1202540}) - A balanced incomplete block design (BIBD) is a pair $(V, B)$ where V is a $v$-set and B
% is a collection of $b$ $k$-sized subsets of $V$ (blocks) such that each element of $V$ is contained
% in exactly $r$ blocks and any 2-subset of V is contained in exactly $\lambda$ blocks.
% \end{nameddefinition}

% Note that this set up can be directly mapped to our setup where $V$ denotes the set of all jobs and each block in $B$ denotes a server and each server(block) in $B$ is precisely assigned those jobs corresponding to the set of elements of $V$ in that block. Also, observe that in BIBD design, we require every set of jobs to occur together in the same number of servers but our pairwise balanced schemes allow a tolerance of upto 1 as we can see in Definition \ref{pair_job_balanced_definition}.






%However, a key difference is that in our definition, we don't require the number of common jobs between any pair of servers to be exactly equal but allow a tolerance of one. In terms of $[\mathfrak{m}^D(m)]_{m=0}^{r}$, the elements of this list is non-zero at exactly two consecutive indices for the pairwise balanced designs proposed in Definition \ref{pair_job_balanced_definition}. 



%Let us denote the $n$ jobs by $\mathcal{A} = \{a_1,\ldots,a_n\}$ and $c$ servers by $\mathcal{S} = \mathcal{S}$. For any assignment ($D$) of jobs in $\mathcal{A}$ to servers in $\mathcal{S}$, we can equivalently represent it as a bipartite graph $\mathcal{G}_D$ where the nodes denote the jobs and the servers with edges existing between nodes denoting job $a_i$ and server $s_j$ if job $a_i$ is assigned to server $s_j$. %There exist edges in from node denoting job $a_i$ to node denoting server $s_j$ only when job $a_i$ is precisely assigned to job $s_j$.

%Edges exist in 



%Alternatively, for any balanced $(n,k,r,c)$ assignment (Definition \ref{definition_balanced}), we can equivalently say every row of matrix $A_D$ sums up to $r$ and every column of matrix $A_D$ sums up to $k$. %We redefine balanced $(n,k,r,c)$ assignment schemes in terms of matrix $A_D$ in {\color{red} Definition \ref{definition_balanced_alt}}.

%\begin{definition*}%{\label{definition_balanced_alt}}
%(Alternate statement of balanced $(n,k,r,c)$ assignment): Given a set of $n$ jobs and $c$ servers, we call an assignment scheme of jobs to various servers a balanced $(n,k,r,c)$ assignment if job assignment matrix $A_D$ satisfies the following properties
%\begin{itemize}
 %   \item Every row of matrix $A_D$ sums upto $r$.
%    \item Each column of matrix $A_D$ sums upto $k$.
%\end{itemize}
%Note that this assignment scheme ensures that $n \times r=k \times c$.
%\end{definition*}





%We now define another set of assignment schemes within balanced $(n,k,r,c)$ assignments. Note that this definition is quite close to the construction of balanced incomplete block designs (BIBD) \cite{doi:10.1111/j.1469-1809.1939.tb02219.x}. However, a key difference is that in our definition, we don't require the number of common jobs between any pair of servers to be exactly equal but allow a tolerance of one.

% \begin{nameddefinition}{Definition}{\label{pair_job_balanced_definition}}
%     (Pairwise balanced job $(n,k,r,c)$ assignment): Given a balanced $(n,k,r,c)$ assignment, we call it  pairwise balanced job $(n,k,r,c)$ assignment if for every pair of distinct jobs $a_i$ and $a_j$ in $\mathcal{A}$, the number of servers which are assigned both $a_i$ and $a_j$ is exactly $l$ or $l+1$ for some integer $l$.

% \end{nameddefinition}

% Using $\mathfrak{m}^D(.)$ defined in \eqref{m_D_defn}, we can define pairwise balanced job assignments below. W.L.O.G, we may assume in pairwise balanced job $(n,k,r,c)$ assignment, there always exist a pair of jobs occurring together in $l$ server and there may or may not be pairs of jobs that occur together in $l+1$ servers. 


% \begin{definition*}
%     [Definition \ref{pair_job_balanced_definition} in terms of $\mathfrak{m}^D(.)$](Pairwise balanced job $(n,k,r,c)$ assignment): Given a balanced $(n,k,r,c)$ assignment, we call it server pairwise -balanced $(n,k,r,c)$ if $\mathfrak{m}_D(m)$ is non-zero for at most 2 consecutive values of $m$ (call it $l$ and $l+1$). 
% \end{definition*}


% Thus, we can see that BIBD would also fall into the category of pairwise balanced job assignment schemes. The existence of BIBD is still not fully understood and some sufficient conditions on $n,k,r$ and $c$ under which BIBD exists are also discussed in \cite{10.5555-1202540,doi:10.1111/j.1469-1809.1939.tb02219.x}. The famous Bruck-Ryser-Chowla theorem gives some necessary condition on $n,k,c,r$ for the existence of BIBDs. 




% The following corollary proves a result on $l$ for any pairwise balanced job $(n,k,r,c)$ assignment.

% \begin{namedlemma}{Lemma}{\label{lemma_on_l_job}}
%     For any pairwise balanced job $(n,k,r,c)$ assignment, we have $l=\Bigl\lfloor\frac{c.{{k \choose 2}}}{{{n \choose 2}}}\Bigr\rfloor$

%     %\Bigl\lfloor\dfrac{1}{2}\Bigr\rfloor
% \end{namedlemma}

% \begin{proof}


% For any pairwise balanced job $(n,k,r,c)$ assignment $D$, we must have $\mathfrak{m}^D(m)$ to be zero for all $m\neq l,l+1$. Thus, we have $\mathfrak{m}^D(l+1) = {{n \choose 2}}- \mathfrak{m}^D(l)$ using eqaution \eqref{proporty_m_1} and similarly, we have $l(\mathfrak{m}^D(l)) + (l+1)({{n \choose 2}}- \mathfrak{m}^D(l)) = c{{k\choose 2}}$ using equation \eqref{property_m_2}. We thus have $l {{n \choose 2}} \leq c{{k \choose 2}}$ and $(l +1){{n \choose 2}} > c{{k \choose 2}}$ (as $\mathfrak{m}^D(l)>0$) and thus $l=\Bigl\lfloor\frac{c.{{k \choose 2}}}{{{n \choose 2}}}\Bigr\rfloor$

% \remove{
    
% Let $n_l$ be the number of pairs of jobs that are present together in exactly $l$ servers and all other pairs of jobs are contained in $l+1$ servers. Therefore, the number of pairs of jobs that are present together in exactly $l+1$ servers is given by ${{n \choose 2}}-n_l$. 


% Thus, summing up over all pairs of jobs, we can say that the total number of servers that contain pairs of distinct jobs (allowing multiple counting for a server if contains more than a pair) is given by $l\times n_l+ (l+1) \times ({{n \choose 2}}-n_l)$. However, observe that the number of pairs of jobs that are assigned to a fixed server $s_i$ is given by ${{k \choose 2}}$. Thus, summing over all such servers $\mathcal{S}$ we can obtain the same quantity to be $c \times {{k \choose 2}}$ and thus, $l\times n_l+ (l+1) \times ({{n \choose 2}}-n_l)=c \times {{k \choose 2}}$ implying, $l= \Bigl\lfloor\frac{c.{{k \choose 2}}}{{{n \choose 2}}}\Bigr\rfloor$ 


% }

% \end{proof}



% %This follows since the total number of pairs of distinct jobs that can be assigned a fixed server $s_i$ is given by ${{k \choose 2}}$ thus, the total number of pairs of jobs that are assigned to a single server (allowing multiple counting if one pair of jobs is present together in more than one server) is given by $c{{k \choose 2}}$ 





% \begin{nameddefinition}{Definition}{\label{pair_server_balanced_definition}}
%     (Pairwise balanced server $(n,k,r,c)$ assignment): Given a balanced $(n,k,r,c)$ assignment, we call it server pairwise -balanced $(n,k,r,c)$ if for every pair of distinct servers $s_i$ and $s_j$ in $\mathcal{S}$, the number of jobs assigned to both $s_i$ and $s_j$ is exactly $l$ or $l+1$ for some integer $l$.
% \end{nameddefinition}

% \begin{namedlemma}{Lemma}{\label{lemma_on_l_server}}
%     For any pairwise balanced server $(n,k,r,c)$, we must have $l=\Bigl\lfloor\frac{n.{{r \choose 2}}}{{{c \choose 2}}}\Bigr\rfloor$
% \end{namedlemma}

% This lemma can be proved in a very similar way as that of Lemma \ref{lemma_on_l_job}.

% With this, we could alternately redefine pairwise balanced server $(n,k,r,c)$ schemes as follows in terms of matrix $A_D$ as follows.

% \begin{definition*}
%     [Definition \ref{pair_job_balanced_definition} in terms of $A_D$](Pairwise balanced server $(n,k,r,c)$ assignment): Given a balanced $(n,k,r,c)$ assignment, we call it server pairwise -balanced $(n,k,r,c)$ if for every pair of distinct indices $i$ and $j$, $|\text{supp}(A_D[:,i]) \cap \text{supp}(A_D[:,j])| = l \text{ or } l+1$ for some integer $l$. 
% \end{definition*}

% \begin{definition*}
%      [Definition \ref{pair_server_balanced_definition} in terms of $A_D$](Pairwise balanced job $(n,k,r,c)$ assignment): Given a balanced $(n,k,r,c)$ assignment, we call it job pairwise -balanced $(n,k,r,c)$ if for every pair of distinct indices $i$ and $j$, $|\text{supp}(A_D[i,:]) \cap \text{supp}(A_D[j,:])| = l \text{ or } l+1$ for some integer $l$. 
% \end{definition*}






% We now describe a pairwise balanced job and server scheme in Example \ref{pairwise_dual_balanced} below. Note that the balanced design is both pairwise job and server balanced in this design. Further, in example \ref{pairwise_balanced_server}, we present an assignment scheme which is pairwise server balanced but not pairwise job balanced.

% \begin{example}{\label{pairwise_dual_balanced}}
%     We now describe a pairwise balanced server and job $(9,3,3,9)$ assignment scheme in Table \ref{pairwise_dual_balanced_assn}. Note that in this scheme, every pair of jobs appear together in exactly 1 or 0 servers, thus it is a pairwise balanced job assignment scheme. Similarly, we can also show that it is also a pairwise balanced server scheme too as every pair of servers has either one job or zero jobs common.
% \end{example}


% \begin{table}[!h]
%     \centering
% {
% 	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c| } 
% 		\hline
% 	\text{Jobs}& $s_1$ & $s_2$ & $s_3$ & $s_4$ & $s_5$ & $s_6$ & $s_7$ & $s_8$ & $s_9$\\
%     \hline
%     $a_1$ & 1 & 1 & 1 & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$ \\
%     \hline
%     $a_2$ & $\text{}$ & $\text{}$ & $\text{}$ & 1 & 1 & 1 & $\text{}$ & $\text{}$ & $\text{}$\\
%         \hline
%      $a_3$ & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$ & 1 & 1 & 1\\
%         \hline
%     $a_4$ & 1 & $\text{}$ & $\text{}$ & 1 & $\text{}$ & $\text{}$ & 1 & $\text{}$ & $\text{}$\\
%     \hline
%     $a_5$ & $\text{}$ &1 & $\text{}$ & $\text{}$ & 1 & $\text{}$ &  $\text{}$ & 1 & $\text{}$\\
%         \hline
%      $a_6$ & $\text{}$ & $\text{}$ &1  & $\text{}$ & $\text{}$ & 1 &  $\text{}$  & $\text{}$ & 1\\
%         \hline
    
%     $a_7$ & 1 & $\text{}$ & $\text{}$ & $\text{}$ & 1& $\text{}$ & $\text{}$ & $\text{}$ & 1\\
%     \hline
%     $a_8$ &$\text{}$& 1 & $\text{}$ & $\text{}$ & $\text{}$ & 1& 1& $\text{}$ & $\text{}$  \\
%         \hline
%      $a_9$ & $\text{}$ & $\text{}$ & 1 & 1& $\text{}$ & $\text{}$ & $\text{}$ & 1 & $\text{}$ \\
%         \hline
        
% 	\end{tabular}
%  }
% 	\vspace{1 em}
% 	\caption{Assignment of jobs to various servers in a pairwise balanced $(9,3,2,6)$ assignment scheme}
% 	\label{pairwise_dual_balanced_assn}
% \end{table}

% \newpage
% \begin{example}{\label{pairwise_balanced_server}}
%     We now describe a pairwise balanced server $(14,6,3,7)$ assignment but not a pairwise balanced job scheme in Table \ref{pairwise_balanced_server_assn}. Note that in this scheme, every pair of servers have exactly 2 jobs in common. However, some pairs of jobs appear together in 1 server like $(a_1,a_2)$ and some pairs of jobs appear together in 3 servers like pairs of jobs $(a_1,a_8)$ and thus it is not pairwise job balanced.
% \end{example}


% \begin{table}[!h]
%     \centering
% {
% 	\begin{tabular}{|c|c|c|c|c|c|c|c| } 
% 		\hline
% 	\text{Jobs}& $s_1$ & $s_2$ & $s_3$ & $s_4$ & $s_5$ & $s_6$ &$s_7$ \\
%     \hline
%     $a_1$ & $\text{}$ & 1 & $\text{}$ & 1 & $\text{}$ & 1 & $\text{}$ \\
%     \hline
%     $a_2$ & 1 & $\text{}$ & $\text{}$ & 1 & 1 & $\text{}$ & $\text{}$\\
%         \hline
%      $a_3$ & $\text{}$ & $\text{}$ & 1 & 1 & $\text{}$ & $\text{}$ & 1 \\
%         \hline
%     $a_4$ & 1 & 1 & 1 & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$\\
%     \hline
%     $a_5$ & $\text{}$ &1 & $\text{}$ & $\text{}$ & 1 & $\text{}$ &  1 \\
%         \hline
%      $a_6$ & 1 & $\text{}$  & $\text{}$ & $\text{}$ &  $\text{}$  & 1 & 1\\
%         \hline
    
%     $a_7$ & $\text{}$ & $\text{}$ & 1 & $\text{}$ & 1& 1 &$\text{}$ \\
%     \hline
%     $a_8$ & $\text{}$ & 1 & $\text{}$ & 1 & $\text{}$ & 1 & $\text{}$ \\
%     \hline
%     $a_9$ & 1 & $\text{}$ & $\text{}$ & 1 & 1 & $\text{}$ & $\text{}$\\
%         \hline
%      $a_{10}$ & $\text{}$ & $\text{}$ & 1 & 1 & $\text{}$ & $\text{}$ & 1 \\
%         \hline
%     $a_{11}$ & 1 & 1 & 1 & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$\\
%     \hline
%     $a_{12}$ & $\text{}$ &1 & $\text{}$ & $\text{}$ & 1 & $\text{}$ &  1 \\
%         \hline
%      $a_{13}$ & 1 & $\text{}$  & $\text{}$ & $\text{}$ &  $\text{}$  & 1 & 1\\
%         \hline
    
%     $a_{14}$ & $\text{}$ & $\text{}$ & 1 & $\text{}$ & 1 & 1 & $\text{}$  \\
%     \hline
        
% 	\end{tabular}
%  }
% 	\vspace{1 em}
% 	\caption{Assignment of jobs to various servers in a pairwise server balanced $(14,6,3,7)$ assignment scheme}
% 	\label{pairwise_balanced_server_assn}
% \end{table}








% Note that the following two theorems say that the variance on the number of distinct $d$ received at the master is the least for the pairwise balanced designs discussed in Definition \ref{pair_job_balanced_definition} and \ref{pair_server_balanced_definition}. However such designs may not always exist and it is not entirely known when such designs exist for every tuple of $(n,k,r,c)$ satisfying $n \times r = k \times c$. This is closely related to balanced incomplete block designs (BIBD) \cite{doi:10.1111/j.1469-1809.1939.tb02219.x} whose existence is not fully and clearly understood. However, a key difference for the pairwise balanced designs we consider is that it is a generalization of BIBD in which they restrict the number of jobs common to any pair of servers to be the same for every such pair of servers. 

% Recall that for the following theorems, we study the setup described in Section \ref{setup_section} where any set of $x$ servers could be the only set of servers that could communicate with the master. Recall that we further assume that every set of $x$ servers is equally likely to be the only set of servers that could communicate with the master. %Reca 





%We prove this theorem in Section \ref{proof_min_var_gen}

\begin{proof}
    Recall the definition of $\mathfrak{m}^D(m)$ from Equation \ref{m_D_defn} which denotes the number of pairs of jobs that are assigned together to exactly $m$ servers with $D$ denoting a stretched minimally compact design.

Now we know that $\mathfrak{m}^{D}(m) = 0$ only for $m\neq 0,r$.


%Now consider any other distribution $D_1$. 
%%Using the proof techniques similar to that of last part of Theorem \ref{min_var} we can say that $D$ gives least variance on number of distinct jobs for every $x$.  


Let us consider another job assignment ${D}_1$ which is a balanced $(n,k,r,c)$ assignment scheme.
 
%Since we know that $\mathfrak{n}^D_{p,D_1}$ = 0

%Recall the definition of $g(p,x)$ as defined in Claim \ref{f_defn}. %Let us denote it as $g_x(p)$ as it is only a function of $p$.

First observe that $\sum\limits_{m=0}^{r} \mathfrak{m}^D(m) = \sum\limits_{m=0}^{r} \mathfrak{m}^{D_1}(m) = {{n \choose 2}}$ which follows from Equation \eqref{proporty_m_1} and $\sum\limits_{m=0}^{r} m \times \mathfrak{m}^D(m) = \sum\limits_{m=0}^{r} m \times \mathfrak{m}^{D_1}(m)= c {{k \choose 2}}$ follows from Equation \eqref{property_m_2}.

We thus have 

\begin{equation}{\label{conditions_no_pairs_repeat}}
    \sum\limits_{m=0}^{r} \mathfrak{m}^D(m) = \sum\limits_{m=0}^{r} \mathfrak{m}^{D_1}(m) = {{n \choose 2}} \text{ and } \sum\limits_{m=0}^{r} m \times \mathfrak{m}^D(m) =\sum\limits_{m=0}^{r} m \times \mathfrak{m}^{D_1}(m)= c {{k \choose 2}}
\end{equation}

We now consider three different cases and in each of these three cases, we show that the variance is the largest for the assignment $D$. Also, we first consider the case where $x\leq c-2r+1$ to prove that the largest variance is uniquely attained by pairwise heavy imbalanced designs.


\begin{itemize}
	\item Case 1: $\mathfrak{m}^{D_1}(r) \geq \mathfrak{m}^{D}(r)$

 Note that this implies that $\sum_{m=0}^{r} m \times \mathfrak{m}^{D_1}(m) \geq \sum_{m=0}^{r} m \times \mathfrak{m}^{D}(m)$
as $\mathfrak{m}^D(m)=0\forall m \in [0,r-1]$. Thus, equation \eqref{conditions_no_pairs_repeat} implies that $\mathfrak{m}^{D_1}(m)=\mathfrak{m}^{D}(m) \forall m \in [r]$ which would imply distribution $D_1$ has same variance of distinct jobs as that of distribution $D$ which follows from Equation \eqref{var_sim_exp} in Theorem \ref{result_variance} as the variance $\sigma_{D,x}$ is just a function of $\mathfrak{m}^D(.)$ other than design parameters $n,k,r$ and $c$.

%Note that $\mathfrak{m}^{D_1}(m) \geq \mathfrak{m}^D(m) \forall m \in [r]$ which follows since $\mathfrak{m}^D(m)=0 \forall m \neq 0,r$. However, equation \eqref{conditions_no_pairs} would imply that $\mathfrak{m}^{D}(m)= \mathfrak{m}^{D_1}(m)$ $\forall$ $m \in [r]$ which would imply distribution $D_1$ has same variance of distinct jobs as that of distribution $D$ which follows from Equation \eqref{var_sim_exp} in Theorem \ref{result_variance} as the variance $\sigma_{D,x}$ is just a function of $\mathfrak{m}^D(.)$ other than design parameters $n,k,r$ and $c$.


\item Case 2: $\mathfrak{m}^{D_1}(r) < \mathfrak{m}^{D}(r)$ but $\mathfrak{m}^{D_1}(0) \geq \mathfrak{m}^{D}(0)$
	
Let us denote $x_m=\mathfrak{m}^{D_1}(m)-\mathfrak{m}^{D}(m)$ $\forall m \in [0,r]$. Clearly, $x_m < 0$ only for $m=r$ as for every $m \neq r$ we have $\mathfrak{m}^D(m)=0$.
	
%	Now we know that $\sum\limits_{p=0}^{r} p.\mathfrak{n}^D_{p,D}= \sum\limits_{p=0}^{r} p.\mathfrak{n}^D_{p,D_1}=n{k \choose 2}$ implying $\sum\limits_{p=0}^{r} p.x_p=0$. Similarly, we can also argue $\sum\limits_{p=0}^{r} x_p=0$.

Observe that equation \eqref{conditions_no_pairs} ensures that $\sum\limits_{m=0}^{r} x_m = \sum\limits_{m=0}^{r} m \times x_m = 0$. 
	
 
 Let us denote $\sum\limits_{m=0}^{r-1} x_m =x$. Since $\sum\limits_{m=0}^{r} x_m=0$, we can say that $x_r= -x$.
	
	Thus,
 
 \begin{align}{\label{temp1_repeat}}
        \sum\limits_{m=0}^{r} x_m \times g(m,x) & = \sum\limits_{m=0}^{r-1} x_m\times g(m,x) - x \times g(r,x) \nonumber \\
        & = \sum\limits_{m=0}^{r-1} x_m \times(g(m,x)-g(r,x)) \overset{(a)}{\leq} 0.
 \end{align}

Note that $(a)$ follows from the fact that $x_m>0$ for all $m \in [0,r-1]$ and the fact that $g(m,x)$ is monotonic in $m$.  
	

\item Case 3: $\mathfrak{m}^{D_1}(0) < \mathfrak{m}^{D}(0)$ and  $\mathfrak{m}^{D_1}(r) < \mathfrak{m}^{D}(r)$

Let us denote $x_m=\mathfrak{m}^{D_1}(m)-\mathfrak{m}^{D}(m)$ $\forall m \in [0,r]$. Clearly, $x_m < 0$ only for $m=0,r$.
	
Now equation \eqref{conditions_no_pairs_repeat} ensures that $\sum\limits_{m=0}^{r} m\times x_m=0$ and $\sum\limits_{m=0}^{r} x_m=0$ Observe that $x_0+x_r = - \sum\limits_{m=1}^{r-1}  x_m$
	




%Let us denote $\sum\limits_{m=0}^{l-1} x_m =\alpha_1 + \alpha_2$ and $\sum\limits_{m=l+2}^{r} x_m=\beta_1+\beta_2$. Since $\sum\limits_{m=0}^{r} x_m=0$, we can say that 

\remove{
\begin{equation}{\label{temp_10}}
    x_l= -(\alpha_1+\beta_1) \text{ and } x_{l+1}=-(\alpha_2+\beta_2) \text { for some }\alpha_1,\beta_1,\alpha_2,\beta_2 \in \mathbbm{N}
\end{equation}
}

Now define $[y_m]_{m=0}^{r}$ and $[z_m]_{m=0}^{r}$as follows below.

\begin{itemize}
    \item $y_m = x_m \times \frac{x_0}{x_0+x_r}$ and $z_m = x_m \times \frac{x_r}{x_0+x_r}$ if $0< m<r$ 
\end{itemize}
			
Also note that $y_m+z_m = x_m\forall m \in [1,r-1]$ and also  $\sum_{l=1}^{r-1} y_l = -x_0$ and $\sum_{l=1}^{r-1} z_l = -x_r$. Thus, $\sum\limits_{m=0}^{r} mx_m =0$ implies

\begin{equation}{\label{temp3_repeat}}
    \sum_{m=1}^{l-1} (r-m) z_m = \sum_{q=1}^{l-1} q \times y_q
\end{equation}



	Now we can say from Claim \ref{Some claims om g(p,x)} that 
	
\begin{equation}{\label{temp4_repeat}}
    \frac{g(r,x)-g(t,x)}{r-t}> \frac{g(t,x)-g(0,x)}{t-0}
	\text{ }\forall t \in [0,r].
 \end{equation}
	
	
Thus we can say the following from equations \eqref{temp3_repeat} and \eqref{temp4_repeat} and the fact that $x_m,y_m,z_m>0$ for $m \in [0,r];$
	
\begin{align}{\label{temp_eqn_variance_case2_repeat}}
	& \sum_{m=1}^{r-1} z_m (g(r,x)-g(m,x)) > \sum_{q=1}^{r-1} y_q (g(q,x)-g(0,x)) \nonumber\\
  \Leftrightarrow & (\sum_{m=1}^{r-1} z_m) g(r,x) - \sum_{m=1}^{r-1}( y_m+z_m) g(m,x) + (\sum_{m=0}^{r-1} y_m) g(0,x) > 0\nonumber\\
 \overset{(b)}{\Leftrightarrow} & -x_r g(r,x) - \sum_{m=1}^{r-1} x_m g(m,x) - x_0 g(0,x) > 0\nonumber\\
 {\Leftrightarrow} & \sum_{m=0}^{r} x_m g(m,r) < 0\nonumber\\
 {\Leftrightarrow} & \sum\limits_{m=0}^{r} \mathfrak{m}^{D_1}(m) g(m,x) < \sum\limits_{m=0}^{r} \mathfrak{m}^{D}(m) g(m,x)
\end{align}
	
Note $(b)$ follows from $y_m+z_m = x_m\forall m \in [1,r-1]$ and also  $\sum_{l=1}^{r-1} y_l = -x_0$ and $\sum_{l=1}^{r-1} z_l = -x_r$.


Now let us consider the numerator of the first term in $\sigma_{{D},x}(d)$ as in theorem \ref{var_sim_exp} which can be written as $2.\sum\limits_{m=0}^{r}\mathfrak{m}^{D}(m)g(m,x) + n.\left(\sum\limits_{t=1}^{r-1} t^2{r \choose (t+1)} {(c-r) \choose (x-t-1)}\right)$.

%Now we consider this expression for $D$ = $D$ and $D_1$.
Thus the inequality proven in the previous equation \eqref{temp_eqn_variance_case2} would imply that assignment scheme $D_1$ has a smaller variance of the number of distinct jobs received at the master than that of assignment scheme $D$, thus proving our desired result. 	


Note that other than Case 1 in this proof (where we show $D_1$ is also a stretched minimally compact assignment), the distribution $D_1$ is not a stretched minimally compact design and we show strict optimality of stretched minimally compact design over any other balanced assignment for $x \leq c-2r+1$. However, if $x> c-2r+1$, the inequalities still hold but are not strict as it follows from Claim \ref{Some claims om g(p,x)}.

Combining these statements, we prove the strict optimality (attains largest variance ) of stretched minimally compact assignments for $x\leq c-2r+1$ and weak optimality for $x>c-2r+1$.
	
	
\end{itemize}

\end{proof}


}

==> mean-and-variance.tex <==
\section{The Mean and the Variance}{\label{setup_section}}

We consider the number of distinct jobs $d$ received at the master when only a subset of $x$ servers manage to communicate with the master. We consider any subset of $\mathcal{S}$ with cardinality $x$ to be equally likely be the set of servers that communicates with the master.  Note that with this definition, if $\hat{S} \subseteq \mathcal{S}$ (with $|\hat{S}| = x$) is the subset of servers that communicate with the master, then we can denote the number of distinct jobs received $d=|\cup_{j \in \hat{S}}\text{supp}(A_D[:,j])|$ where $\text{supp}(v)$ denotes the indices of the non-zero entries of the vector $v$.

Now, consider the uniform distribution over all subsets of servers of cardinality $x$ which we denote by $\mathfrak{D}_{\mathcal{S},x}$ i.e. a sample from this distribution returns any subset of $\mathcal{S}$ of cardinality $x$ with probability $\frac{1}{{{|\mathcal{S}| \choose x}}}$. 

For a given assignment ${D}$ of jobs to servers, we denote the expectation of the number of distinct completed jobs received by the master when any subset of $x$ servers is able to communicate with master uniformly at random by $\mathbbm{E}_{{D},x}[d]$ and the corresponding variance by $\sigma_{{D},x}[d]$. The expectation and the variance on the number of distinct received jobs $d$ may be written as 

\begin{equation}{\label{formal_eqn_var_exp}}
    \mathbbm{E}_{D,x}[d]= \mathbbm{E}_{\hat{S} \sim \mathfrak{D}_{\mathcal{S},x}} \left[\left|\bigcup_{j \in \hat{S}}\text{supp}(A_D[:,j])\right|\right] \text{ and } \sigma_{D,x}[d]= \sigma_{\hat{S} \sim \mathfrak{D}_{\mathcal{S},x}} \left[\left|\bigcup_{j \in \hat{S}}\text{supp}(A_D[:,j])\right|\right]
\end{equation}

Note that the randomness in this setup is only in the set of servers that can  communicate with the master. The assignment scheme has no randomness associated with it.

%We analyse the number of distinct jobs $d$ when any subset of servers ($\mathcal{S}$) of cardinality $x$ is able to communicate with the master with equal probability. Recall that $\mathcal{S}$ denotes the entire set of servers in the system.

%For a given assignment ${D}$ of jobs to servers, we denote the expectation in the number of distinct completed jobs received by the master when any set of $x$ servers is able to communicate with master uniformly at random by $\mathbbm{E}_{{D},x}[d]$ and the corresponding variance by $\sigma_{{D},x}[d]$. 


Theorem~\ref{all_mean} states that the expectation on the number of distinct jobs $\mathbb{E}_{D,x}[d]$ is the same for every balanced $(n,k,r,c)$ assignment. This expectation is a function of $n,k,r,c$ and $x$ and is independent of the specific balanced assignment $D$ we choose. Throughout the remainder of this paper, $\mathfrak{n}^D_{i,\hat{S}}$ denotes the number of servers in $\hat{S}$ to which job $a_i$ is assigned under the assignment scheme $D$.  Observe that $\mathfrak{n}^D_{i,\hat{S}}$ can take any value from $0$ to $r$. 




%There would be some jobs appearing multiple number of times in the subset of servers $S$. Thus, we say job $a_i$ occurred $\mathfrak{n}^D_{i,S}$ times in subset $S$ for any $i \leq n$. Note that $\mathfrak{n}^D_{i,S}$ could possibly be zero for some values of $i$ as well. Note that $\mathbbm{1}_E$ denotes the indicator random variable corresponding to event $E$. Let us denote the distribution of jobs in servers by $\mathcal{D}$. %We denote the number of subsets of 

%We are interested in those jobs which have $\mathfrak{n}^D_{i,S}>1$ in subset $S$ and thus claim that number of distinct jobs ($d$) received from subset of workers $S$ is $(k\times x- \sum\limits_{i=1}^{n} (\mathfrak{n}^D_{i,S}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,S}>1})$ if the cardinality of $S$ is $x$. 




\begin{theorem}{\label{all_mean}}
 Consider any balanced $(n,k,r,c)$ assignment $D$. The expectation of the number of distinct completed jobs $d$ received by the master when any subset of cardinality $x$ of the set of servers $\mathcal{S}$ is able to communicate with the master with equal probability is the same for every balanced $(n,k,r,c)$ assignment $D$ and is given by 
 
 %Note that has the same expectation of distinct jobs received for every $x\leq c$ assuming $S$ can be any subset of the servers of cardinality $x$ with equal probability. Also the expectation can be computed as 
 \begin{equation}
  \mathbbm{E}_{{D},x}[d]= n\cdot\left(1-\frac{{c-r \choose x}}{{c \choose x}}\right) 
 \end{equation}
 %where $d$ denotes the number of distinct jobs received when any set of $x$ servers return and the job distribution is denoted by $\mathcal{D}$. 
 
 
 		
\end{theorem}

We present a proof sketch below. A detailed proof is presented in Appendix \ref{sec:all_mean_proof}.

% We may observe that for $x>c-r$, the expectation goes to $n$. This follows since, every job would definitely be received at the master as each job is assigned to exactly $r$ servers, hence no job can be missing from the set of jobs received at the master.



\begin{proof}[Proof Sketch]
    
	
%Let us compute the expectation of distinct jobs($d$) received.For the computation of $d$, w

%\begin{equation}{\label{n_D_defn}}
 %   \mathfrak{n}^D_{i,\hat{S}}= |(\text{sup}(A[i,:]) \cap \hat{S})|
%\end{equation}
%or maybe defined as in terms of assignment matrix $A_D$. 

The number of distinct jobs $d$ received by the master when servers in a subset $\hat{S}$ (with $|\hat{S}| = x$) is able to communicate with the master is given by 

\begin{equation}{\label{constr_d}}
    d = \left|\bigcup_{j \in \hat{S}}\text{supp}(A_D[:,j])\right|= \left(k\times x- \sum\limits_{i=1}^{n} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1}\right)
\end{equation}

%where $x$ denotes the cardinality of set $\hat{S}$. 
Note that the term $\sum\limits_{i=1}^{n} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1}$ excludes those jobs which have been received multiple times from various servers present in $\hat{S}$.
 
	
	\begin{align}{\label{expectation_simplification}}
	 \mathbb{E}_{D,x}[d]
	= \frac{\sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} (k \times x- \sum\limits_{i=1}^{n} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1})}{\sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} 1}
	  {=} & k\times x - \frac{n\sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1} }{{c \choose x}}
	\end{align}
	
	
	%$(a)$ follows on interchanging summations.
	
	Observe that for every job $a_i$ in a balanced $(n,k,r,c)$ assignment, the quantity $\sum\limits_{\hat{S} \subset \mathcal{S},|\hat{S}|=x} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1}$ is the same, i.e., this summation is independent of $i$.  We now show that the quantity  $\sum\limits_{\hat{S} \subset \mathcal{S},|\hat{S}|=x} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1}$ for any specified $x$, is the same for every balanced  $(n,k,r,c)$ distribution ${D}$. We compute this sum by counting the number of subsets $\hat{S} \subset \mathcal{S}$ of cardinality $x$ which additionally satisfies the constraint on $\mathfrak{n}^D_{i,\hat{S}}=t$ (i.e. job $a_i$ is present in exactly $t$ servers from $\hat{S}$) for every $t$ from $2$ to $r$ (as these cases deal with the job $a_i$ appearing more than once in the subset $\hat{S}$). Equation \eqref{temp_result_removal} follows from multiplying two binomial expressions \footnote{Detailed proof is presented in Appendix \ref{sec:all_mean_proof}} and considering their coefficients.
	
	
\begin{align}{\label{removal_comp_mean}}
	\sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1}
	{=} \sum\limits_{t=1}^{r-1} \sum\limits_{\substack{\hat{S} \subset \mathcal{S}; \\|\hat{S}|=x,\mathfrak{n}^D_{i,\hat{S}}=t+1}} t\nonumber 
	\overset{(a)}{=} & \sum\limits_{t=1}^{r-1} t{r \choose (t+1)} {(c-r) \choose (x-t-1)} \\
\end{align}

%We desribe the reasoning for each of the equalities in $(a),(b),(c)$ and $(d)$ below.

%\begin{itemize}
 %   \item $(a)$ follows since $\mathfrak{n}^D_{i,\hat{S}}$ can take value only from $\{0,1,2,...r\}$.
  %  \item $(b)$ follows since $t$ is a constant for the second summation.

 %   \item (c) follows from the argument below.
	
%	Note that $\sum\limits_{\substack{\hat{S} \subset \mathcal{S}; \\|\hat{S}|=x,\mathfrak{n}^D_{i,\hat{S}}=t+1}} 1$ denotes the number of subsets of servers of cardinality $x$ which have job $a_i$ occurring $(t+1)$ times.
	
%	This would be unique irrespective of distribution since job $a_i$ would occur in exactly $r$ servers. This the subsets should have $(t+1)$ servers from these $r$ servers and all the other $(x-t-1)$ servers from the remaining $(c-r)$ servers. Hence, there are ${r \choose (t+1)} {(c-r) \choose (x-t-1)}$ such subsets.


%    \item For equality in $(d)$, we use the following binomial expressions.\\
% The last equality $(a)$ comes from counting the number of subsets $\hat{S} \subset \mathcal{S}$ of cardinality $x$ that contain precisely $t+1$ servers that were assigned the job $a_i$.
% Consider the following binomial expressions	
% 	\begin{equation}{\label{binomial_1}}
% 	    ry(1+y)^{r-1} + 1 - {(1+y)^r} = \sum\limits_{t=0}^{r-1} t{{r \choose t+1}} y^{t+1}
% 	\end{equation}

%         \begin{equation}{\label{binomial_2}}
%             (1+y)^{c-r}=\sum\limits_{u=0}^{c-r} {{c-r \choose u}} y^u
%         \end{equation}
% 	%$$
 
%  %$$$$ 
% Multiplying equations \eqref{binomial_1} and \eqref{binomial_2}, one observes that $\sum\limits_{t=1}^{r-1} t{r \choose (t+1)} {(c-r) \choose (x-t-1)}$ is precisely the coefficient of $y^{x}$ in $ry(1+y)^{c-1} + {(1+y)^{c-r}} - {(1+y)^c}$. Thus,
\vspace{-2 em}
\begin{equation}{\label{temp_result_removal}}
    \sum\limits_{t=1}^{r-1} t{r \choose (t+1)} {(c-r) \choose (x-t-1)} = r \times {{c-1 \choose x-1}} + {{c-r \choose x}} - {{ c \choose x}}
\end{equation}
%equals $r \times {{c-1 \choose x-1}} + {{c-r \choose x}} - {{ c \choose x}}$. 
%\end{itemize}
	
	 %whereas 
	%Thus, we have $\mathbbm{E}_{D,x}[d]= k \times x - \frac{n\sum\limits_{t=1}^{r-1} t{r \choose (t+1)} {(c-r) \choose (x-t-1)}}{{c \choose x}}$
	
	%This would imply that the mean number of distinct elements received for a given $x$ remains the same irrespective of job distribution chosen as long as it as a balanced assignment scheme (defined in Definition \ref{definition_balanced}).
	
	
	%Note that using the idea of summation of series using coefficients of binomial expressions we can show that $\sum\limits_{t=1}^{r-1} t{r \choose (t+1)} {(c-r) \choose (x-t-1)} = r \times {{c-1 \choose x-1}} + {{c-r \choose x}} - {{ c \choose x}}$. 


Combining equations \eqref{expectation_simplification},
\eqref{removal_comp_mean} and \eqref{temp_result_removal}, we get the desired result. 

% $$\mathbbm{E}_{D,x}[d]= k \times x - \frac{n\left(r \times {{c-1 \choose x-1}} + {{c-r \choose x}} - {{c \choose x}}\right)}{{{c \choose x}}}= n\left(1-\frac{{{c-r \choose x}}}{{{c \choose x}}}\right)$$
 

\end{proof}

A few comments are in order here. Note that for $x=1$, the expectation (as expected) is precisely $k$. Observe that for $x>c-r$, the expectation goes to $n$. In other words, if the number of servers that successfully communicates with the master is greater than $(c-r)$, then the master obtains at least one copy of every job $a_i \in \mathcal{A}$. This follows since every job is assigned to exactly $r$ servers and therefore for any job to be missed out, the $r$ servers to which that specific job was  assigned, should fail to communicate with the master. Thus, if any job is missed out, then the number of servers that manage to communicate with the master $x$ can at most be $c-r$.  


We now calculate the variance for the number of distinct jobs $d$ received at the master for any balanced $(n,k,r,c)$ job assignment $D$. From the comments in the previous paragraph, it is clear that $\sigma_{D,1}[d] = 0$ for the case $x = 1$, since the master always receives precisely $k$ distinct jobs, if only one server manages to communicate with the master. Similarly, $\sigma_{D,x}[d] = 0$ for $x > c-r$, as the master would receive all the $n$ jobs if more than $c-r$ servers communicate (for the sake of completeness, we formally calculate this in Corollary \ref{corollary_variance}).

For calculating the variance on the number of distinct jobs $d$ received by the master, observe 
\begin{equation*}
 \sigma_{D,x}(d) =
	\sigma_{D,x}\left(k\times x- \sum\limits_{i} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1}\right) = \sigma_{D,x} \left(\sum\limits_{i} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1}\right)   
\end{equation*}
The above follows since $\sigma(t-X) = \sigma(X)$ where $t$ is a constant and $X$ is a random variable. We now make use of the definition $\text{var}(X) = \mathbbm{E}[X^2]- (\mathbbm{E}[X])^2$. Therefore,
\begin{align}{\label{sigma_expression1}}
	% \sigma_{D,x}(d) &=
	\sigma_{D,x} \left(\sum\limits_{i} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1}\right)
	= & \frac{\sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} {\left(\sum\limits_{i=1}^{n} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1}\right)}^2}{\sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} 1} - \left(\frac{\sum\limits_{\substack{\hat{S} \subset \mathcal{S}; |\hat{S}|=x}} {(\sum\limits_{i=1}^{n} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1})}}{\sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} 1}\right)^2\nonumber\\
	& \hspace{-2 em}\overset{(a)}{=} \frac{\sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} (\sum\limits_{i=1}^{n} \sum\limits_{j=1}^{n} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1} (\mathfrak{n}^D_{j,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{j,\hat{S}}>1})}{\sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} 1} - \left(\frac{\sum\limits_{i=1}^{n} \sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\ |\hat{S}|=x}} {((\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1})}}{{c \choose x}}\right)^2\nonumber\\
	& \overset{(b)}{=} \frac{\sum\limits_{i=1}^{n} \sum\limits_{j=1}^{n} \sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1} (\mathfrak{n}^D_{j,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{j,\hat{S}}>1}}{{c \choose x}}- \left(\frac{n\sum\limits_{t=1}^{r-1} t{r \choose (t+1)} {(c-r) \choose (x-t-1)}}{{c \choose x}}\right)^2\nonumber\\
    & \overset{(c)}{=} \frac{\sum\limits_{i=1}^{n} \sum\limits_{j=1}^{n} \sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1} (\mathfrak{n}^D_{j,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{j,\hat{S}}>1}}{{c \choose x}}- \left(\frac{n{{c-r \choose x}}}{{{c \choose x}}} + n \times\left(\frac{rx}{c}-1\right)\right)^2
\end{align}

In the above set of equations, $(a)$ follows from the identity $(\sum\limits_i b_i)^2 = \sum\limits_i \sum\limits_j b_i b_j$. The first term in $(b)$ is obtained by interchanging the order of summations, whereas the second term comes from equation \eqref{removal_comp_mean}.  Further, the second term in $(c)$ follows using the equation \eqref{temp_result_removal} given in the proof of Theorem \ref{all_mean}.

Observe that the second term in the final expression in equation~\eqref{sigma_expression1} depends only on $n,r,c$ and $x$ and is independent of the specific balanced $(n,k,r,c)$ job assignment $D$. On the other hand, the first term in equation~\eqref{sigma_expression1} depends on the particular assignment $D$. We now consider the numerator of the first term of equation~\eqref{sigma_expression1} in more detail. We can break this expression into two parts, where one part is dependent on just one index $i$ and the other part is dependent on two distinct indices $i,j$. Thus,   \begin{align}{\label{twoparts}}
	& \sum\limits_{i=1}^{n} \sum\limits_{j=1}^{n} \sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1} (\mathfrak{n}^D_{j,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{j,\hat{S}}>1}\nonumber\\
	= & 2\sum\limits_{1\leq i < j\leq n} \sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1} (\mathfrak{n}^D_{j,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{j,\hat{S}}>1}\\
	& \hspace{8 em} + \sum\limits_{1\leq i =j\leq n} \sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1} (\mathfrak{n}^D_{j,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{j,\hat{S}}>1}
\end{align}
In equation~\eqref{twoparts}, the second term can be rewritten as $\sum\limits_{1\leq i \leq n} \sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} ((\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1})^2$. For every job $a_i$, this expression calculates $\sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} ((\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1})^2$, which is independent of the choice of the job $a_i$ in any balanced $(n,k,r,c)$ assignment $D$. In fact, this second term of equation~\eqref{twoparts} is independent of the choice of $D$ and it depends only on the values of $n,c,r$ and $x$. We can compute this sum by counting the number of subsets $\hat{S} \subset \mathcal{S}$ of cardinality $x$ that additionally satisfy the constraint $\mathfrak{n}^D_{i,\hat{S}}=t$ (i.e. job $a_i$ is present in exactly $t$ servers from $\hat{S}$) for every $t$ from $2$ to $r$. Thus \begin{equation}\label{squares}
\sum\limits_{1\leq i \leq n} \sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} ((\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1})^2 = n\sum\limits_{t=1}^{r-1} t^2{r \choose (t+1)} {(c-r) \choose (x-t-1)}
\end{equation} 
Note that the number of subsets $\hat{S} \subset \mathcal{S}$ of cardinality $x$ such that a particular job $a_i$ appears $t+1$ times in $\hat{S}$ is given by ${r \choose (t+1)}{(c-r) \choose (x-t-1)}$. As $\mathfrak{n}^D_{i,\hat{S}}=t+1$ for this particular $\hat{S}$, therefore $((\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1})^2 = t^2$. This explains the final expression in equation~\eqref{squares}.  A closed form expression for the sum $\sum\limits_{t=1}^{r-1} t^2{r \choose (t+1)} {(c-r) \choose (x-t-1)}$ can be obtained by considering the following binomial expressions 
\begin{equation}{\label{binomial_corollary_4}}
    r(r-1) y^2(1+y)^{r-2} - ry(1+y)^{r-1} - 1 + {(1+y)^r} = \sum_{t=1}^{r-1} t^2 {{r \choose t+1}} y^{t+1}
\end{equation}

\begin{equation}{\label{binomial_corollary_5}}
        (1+y)^{c-r} = \sum_{v=0}^{c-r} {{c-r \choose v}} y^v
\end{equation}

Multiplying equations \eqref{binomial_corollary_4} and \eqref{binomial_corollary_5}, one obtains $\sum\limits_{t=1}^{r-1} t^2 {{r \choose t+1}}{{c-r \choose x-t-1}}$ to be the coefficient of $y^{x}$ in $r(r-1) y^2(1+y)^{c-2} - ry(1+y)^{c-1} - (1+y)^{c-r} + (1+y)^c$, thus,  

\begin{equation}{\label{temp_corollary}}
        \sum\limits_{t=1}^{r-1} t^2 {{r \choose t+1}}{{c-r \choose x-t-1}} = r(r-1) {{c-2 \choose x-2}} - r{{c-1 \choose x-1}} -{{c-r \choose x}}+ {{c \choose x}}
\end{equation}

Finally, we analyse the first term in equation~\eqref{twoparts}, viz., $\sum\limits_{1\leq i < j\leq n} \sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1} (\mathfrak{n}^D_{j,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{j,\hat{S}}>1}$. If a specific pair of jobs $a_i,a_j$ appear $(\alpha + 1)$ and $(\beta + 1)$ times respectively in some subset $\hat{S} \subset \mathcal{S}$ of cardinality $x$, then such a pair of jobs contribute $\alpha\beta$ towards this expression that we are analysing. One needs to add up such contributions from every distinct pair of jobs $(a_i,a_j)$ and every subset $\hat{S} \subset \mathcal{S}$ of cardinality $x$ to get the final value of this expression. The strategy that we adopt to compute this sum is as follows : we find $\sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1} (\mathfrak{n}^D_{j,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{j,\hat{S}}>1}$ for any given pair of distinct jobs $(a_i,a_j)$. Observe that this expression depends on how the pair of jobs $(a_i,a_j)$ are distributed amongst the $c$ servers, which in turn depends on the particular balanced $(n,k,r,c)$ job assignment $D$ that is under consideration. Now, given a particular pair of jobs $(a_i,a_j)$, how they are farmed to the servers can essentially differ only in the number of servers that are assigned both the jobs $a_i,a_j$ simultaneously. The number of servers that are simultaneously assigned both the jobs $(a_i,a_j)$ can range from $0$ to $r$. If a pair of jobs $(a_i,a_j)$ are assigned together to precisely $m$ servers (with $0 \le m \le r$), then the sum $\sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1} (\mathfrak{n}^D_{j,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{j,\hat{S}}>1}$
calculated for this particular pair of jobs is precisely equal to the corresponding sum for every other pair of jobs that are assigned together to precisely $m$ servers. We use the notation 

\begin{equation}{\label{g_defn}}
    g(m,x) = \sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1} (\mathfrak{n}^D_{j,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{j,\hat{S}}>1}
\end{equation} 
to indicate this particular sum that arises from a pair of jobs $a_i,a_j$ that are assigned together to precisely $m$ servers. We now show that the values of $g(m,x)$ depends only on $c,r,m$ and $x$. We give the expression for $g(0,x)$ in Lemma \ref{g_p_0_lemma} and give a recursion to compute $g(m,x)$ in Lemma \ref{g_p_diff_lemma}.

\begin{lemma}{\label{g_p_0_lemma}}
    For a balanced $(n,k,r,c)$ assignment, the value of $g(0,x)$ is given by 
    \begin{align}{\label{g_0_exp}}
    g(0,x) = & r^2 {{c-2 \choose x-2}} - 2r {{c-1 \choose x-1}} + {{c \choose x}} - 2{{c-r \choose x}} + 2 r{{c-r-1 \choose x-1}} + {c-2r \choose x}
\end{align}
\end{lemma}


\begin{lemma}{\label{g_p_diff_lemma}}
For a balanced $(n,k,r,c)$ assignment, the values for $g(m,x)$ are related in the following fashion 
\begin{equation}{\label{g_p_diff}}
    g(m+1,x) - g(m,x) = {c-2 \choose x-1} - 2{c-r-1 \choose x-1} + {c-2r+m \choose x-1}
\end{equation}
\end{lemma}


We prove these Lemmas in Appendix \ref{sec:g_p_0_lemma_proof} and \ref{sec:g_p_diff_lemma_proof} respectively using a careful application of techniques from combinatorics. %The proof of Lemma \ref{g_p_0_lemma} follows by considering a pair of jobs which never appears together in a server and by doing a careful counting using techniques from combinatorics. %Lemma \ref{g_p_diff_lemma} is proven by considering two distinct pairs of jobs that appear together in $m$ and $m+1$ servers respectively.

Note that all the expressions for $g(m,x)$ depends on the values of $c,r,m$ and $x$ and is therefore independent of which balanced $(n,k,r,c)$ assignment $D$ we choose. Observe further that the expression for $g(m+1,x)-g(m,x)$ is an increasing function of $m$ when $x$ is fixed. This is clear from the fact that only the last term in \eqref{g_p_diff} depends on $m$. Of course, if $x \le c - 2r$, then we can further conclude that $g(m+1,x)-g(m,x)$ is a strictly increasing function of $m$.

We now define $\mathfrak{m}^D(m)$ as the number of distinct pairs of jobs $(a_i,a_j)$ with $1 \le i < j \le n$ that are assigned together to precisely $m$ servers in the balanced $(n,k,r,c)$ assignment $D$. One can formally define this number for a specific balanced $(n,k,r,c)$ assignment $D$ using the assignment matrix $A_D$ as \begin{equation}{\label{m_D_defn}}
    \mathfrak{m}^D(m) = \sum_{\substack{(i_1,i_2)\\ 1\leq i_1<i_2 \leq n }} \mathbbm{1}_{\sum_{j=1}^{c} A_D[i_1,j]A_D[i_2,j]=m} 
\end{equation}

Given a balanced $(n,k,r,c)$ assignment $D$, the numbers $\mathfrak{m}^D(m)$ have some additional properties

% \begin{multicols}{2}
%    \begin{equation}{\label{proporty_m_1}}
%          \sum_{m=0}^r \mathfrak{m}^D(m) = {n \choose 2}
%     \end{equation}
%     \begin{equation}{\label{property_m_2}}
%         \sum_{m=0}^r m\mathfrak{m}^D(m) = c{k \choose 2}
%     \end{equation}
% \end{multicols}

\noindent\begin{minipage}{0.49\linewidth}
    \begin{equation}
     \sum_{m=0}^r \mathfrak{m}^D(m) = {n \choose 2}
    \label{proporty_m_1}
    \end{equation}
\end{minipage}
\hfill
\begin{minipage}{0.48\linewidth}
    \begin{equation}
    \sum_{m=0}^r m\mathfrak{m}^D(m) = c{k \choose 2}
    \label{property_m_2}
    \end{equation}
\end{minipage}



%\end{itemize}

\vspace{1 em}

Equation \eqref{proporty_m_1} follows from the fact that there are a total of $n$ jobs and thus the total number of job pairs is given by ${{n \choose 2}}$. Equation \eqref{property_m_2} follows from the fact that the number of pairs of jobs that are assigned together to a fixed server $s_i$ is given by ${{k \choose 2}}$. Summing over all the servers in $\mathcal{S}$ gives us the RHS in \eqref{property_m_2}. Note that we count each pair of jobs as many times as they appear together in a server and thus we say $\sum_{m=0}^r m\mathfrak{m}^D(m) = c{k \choose 2}$.



%However, observe that the number of pairs of jobs that are assigned to a fixed server $s_i$ is given by ${{k \choose 2}}$. Thus, summing over all such servers $\mathcal{S}$ we can obtain the same quantity to be $c \times {{k \choose 2}}$


Observe that the first term of equation~\eqref{twoparts} that we are evaluating can now be rewritten as \begin{equation}
 \sum\limits_{1\leq i < j\leq n} \sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1} (\mathfrak{n}^D_{j,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{j,\hat{S}}>1} = \sum_{m = 0}^r \mathfrak{m}^D(m)g(m,x)   
\end{equation}
Putting all of the discussion together, we therefore conclude the following regarding evaluation of variance $\sigma_{D,x}(d)$ : 


\begin{theorem}{\label{result_variance}}

Consider any assignment $D$ amongst balanced $(n,k,r,c)$ assignments. The variance on the number of distinct jobs $d$ $(\sigma_{D,x}(d))$ received by the master when any subset of servers $\mathcal{S}$ of cardinality $x>1$ is able to communicate to the master with equal probability, is equal to
  
  \begin{equation}{\label{var_sim_exp}}
\sigma_{{D},x}(d)= \frac{2\sum\limits_{m=0}^{r}\mathfrak{m}^D(m)g(m,x) + T_2(n,r,c,x)}{{c \choose x}}- \left(T_1(n,r,c,x)\right)^2\\
\end{equation}  
 
{where} $T_1(n,r,c,x) = \frac{n{{c-r \choose x}}}{{{c \choose x}}} + n \times(\frac{rx}{c}-1)$ and 
\begin{align}
    T_2(n,r,c,x) = & n\sum\limits_{t=1}^{r-1} t^2{r \choose (t+1)} {(c-r) \choose (x-t-1)}\\
    = & n\left(r(r-1) {{c-2 \choose x-2}} - r{{c-1 \choose x-1}} -{{c-r \choose x}}+ {{c \choose x}}\right)
\end{align}

%$$ $$


% \remove{
% and $g(.) : \{0,1,\ldots,r\}\rightarrow \mathbbm{N}\cup \{0\}$ satisfying equations \eqref{g_p_diff} and \eqref{g_p_start}.

%     \begin{equation}{\label{g_p_diff}}
%         g(p+1)-g(p)= \left[{{(c-2) \choose (x-1)}}-2{{(c-r-1) \choose (x-1)}}+ {{(c-2r+p-1)\choose (x-1)}}\right]
%     \end{equation}
%     \item 
%     \begin{align}{\label{g_p_start}}
%         g(0)= & \sum\limits_{i=2}^{r+1}\sum\limits_{j=2}^{r+1} (i-1).(j-1).{(c-2r) \choose (x-i-j)}.{r \choose i}.{r\choose j}\nonumber\\
%         & = r^2 {{c-2 \choose x-2}} - 2r {{c-1 \choose x-1}} + {{c \choose x}} - 2{{c-r \choose x}} + 2 r{{c-r-1 \choose x-1}}
%     \end{align}
    
%  }   
\end{theorem}

Thus, we have shown that while the mean of the number of received jobs $d$ is the same for all balanced $(n,k,r,c)$ assignments, the variance of $d$ is dependent on the frequency distribution of job pairs assigned to the same server.  



==> preliminary.tex <==
\section{Preliminaries and Notation}
{\label{setting_section}}

%We consider a setup where a master has $n$ jobs to compute and has $c$ servers to perform the computations. We further assume a noisy scenario where only a fraction of these servers are able to communicate back to the master. %Therefore, for increasing reliability, redundancies are introduced in the setup by assigning each job to multiple servers. In this paper, we examine the expectation and variance on the number of distinct completed jobs that the master receives from the servers that were able to communicate, for various assignment schemes. In particular, we study assignment schemes that achieve certain desired variances on the number of received distinct jobs.

%\section{Notations and symbols} {\label{setting_section}}

%Given a set of $n$ jobs(tasks) and $c$ servers, we would like to study the assignemnt $k$ jobs to each server with no two same jobs in any server along with each job appearing in exactly $r$ distinct servers. This would imply that $n \times r = k \times c$. 

Given a set of $n$ jobs and $c$ servers, we study various assignments of jobs to different servers by the master server. More formally, let us denote the $n$ jobs by $\mathcal{A} = \{a_1,\ldots,a_n\}$ and $c$ servers by $\mathcal{S} = \{s_1,s_2,\ldots,s_c\}$. Any assignment ($D$) of jobs in $\mathcal{A}$ to servers in $\mathcal{S}$, can be  equivalently represented by a bipartite graph $\mathcal{G}_D$ where the nodes denote the jobs and the servers. The edges of the graph exist between nodes representing job $a_i$ and server $s_j$ if job $a_i$ is assigned to server $s_j$. Alternately, for a job assignment ${D}$, we can define an assignment matrix $A_{{D}} \in \{0,1\}^{n \times c}$ as given below.

\begin{nameddefinition}{Definition}
(Construction of $A_D$): Given an assignment of jobs in $\mathcal{A}$ to servers in $\mathcal{S}$, we define matrix $A_D \in \{0,1\}^{n \times c}$ as follows.
: \begin{align}{\label{A_defn}}
    A_{{D}}[i,j] & = 1 \text{ if job $a_i$ is assigned to server $s_j$}\nonumber \\
                & = 0 \text{ otherwise}
\end{align}
\end{nameddefinition}

Observe that the matrix $A_{D}$ represents the adjacency matrix for the bipartite graph $\mathcal{G}_D$. 



%Note that by balanced assignments, we consider assignments where each server is assigned the same number of jobs and each job is assigned to the same number of servers. We state it formally as the two conditions given below. 

We specifically study balanced assignment schemes where each server is assigned the same number of jobs and each job is assigned to the same number of servers. More formally, we define this as follows.


%More formally, we state it as two conditions below.

\begin{nameddefinition}{Definition}{\label{definition_balanced}}
(Balanced $(n,k,r,c)$ assignment): Given a set of $n$ jobs and $c$ servers, we call an assignment scheme of jobs a balanced $(n,k,r,c)$ assignment if the following conditions are satisfied.
\begin{itemize}
    \item Each server is assigned precisely $k$ distinct jobs to compute.
    \item Each job is assigned to precisely $r$ distinct servers.
\end{itemize}
Note that this assignment scheme ensures that $n \times r=k \times c$.
\end{nameddefinition}

We can equivalently define it in terms of matrix $A_D$ as follows.

\begin{definition*}
    (Balanced $(n,k,r,c)$ assignment in terms of $A_D$): Given $n$ jobs and $c$ servers, we call the assignment scheme $D$ of jobs to servers a balanced $(n,k,r,c)$ assignment if each row of $A_D$ sums up to $r$ and each column sums up to $k$.
\end{definition*}

Let us look at an example of a balanced $(9,3,2,6)$ assignment scheme. 



% \begin{tabular}{|c|c|c|}
%   \hline
%   \multicolumn{1}{|c}{\raisebox{-1ex}{\rotatebox{45}{Column 1}}} & Header 1 & Header 2 \\
%   \hline
%   Row 1 & Content 1 & Content 2 \\
%   \hline
%   Row 2 & Content 3 & Content 4 \\
%   \hline
% \end{tabular}



\begin{example}{\rm
We describe a balanced assignment scheme with 9 jobs $\{a_1,a_2,\ldots,a_9\}$ and 6 servers $\{s_1,s_2,\ldots,s_6\}$ in Table \ref{balanced_assn}. Note that each job is assigned to precisely $2$ servers and each server has exactly 3 jobs to compute. The assignment scheme is motivated from a cyclic assignment scheme.
}\end{example}


%\rule{0pt}{20pt}\rotatebox{-10}{\makebox[10pt][l]
\begin{table}[!h]
    \begin{center}
{
	\begin{tabular}{|c|c|c|c| c|c|c|c| } 
		\hline
	{{\diagbox[width = 5 em]{Jobs}{Servers}}}& $s_1$ & $s_2$ & $s_3$ & $s_4$ & $s_5$ & $s_6$ \\
    \hline
    $a_1$ & 1 & 1 & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$ \\
    \hline
    $a_2$ & $\text{}$ & 1 & 1 & $\text{}$ & $\text{}$ & $\text{}$\\
        \hline
     $a_3$ & $\text{}$ & $\text{}$ & 1 & 1 & $\text{}$ & $\text{}$\\
        \hline
    
    $a_4$ & $\text{}$ & $\text{}$ & $\text{}$ & 1 & 1 & $\text{}$\\
    \hline
    $a_5$ & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$ & 1 & 1\\
        \hline
     $a_6$ & 1& $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$ & 1 \\
        \hline
    
    $a_7$ & 1 & 1 & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$\\
    \hline
    $a_8$ & $\text{}$ & $\text{}$ & 1 & 1 & $\text{}$ & $\text{}$ \\
        \hline
     $a_9$ & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$ & 1 & 1 \\
        \hline
        
	\end{tabular}
 }
 \end{center}
	\vspace{1 em}
	\caption{Assignment of jobs to various servers in a balanced $(9,3,2,6)$ assignment scheme}
	\label{balanced_assn}
\end{table}


==> removedpart.tex <==
\remove{
We now consider the case where $x>c-r$, and show that the variance as stated in Theorem \ref{result_variance} goes to 0. As each of the $n$ jobs would be received by the master since every job is present in exactly $r$ servers and at most $r-1$ servers fail to communicate with the master, the number of jobs received is always $n$ and hence the variance should be zero.%This should follows as each of the $n$ jobs would be received by the master as every job is present in exactly $r$ servers, thus the number of jobs received is always $n$, hence zero variance.

\begin{namedcorollary}{Corollary}{\label{corollary_variance}}
    The variance $\sigma_{D,x}(d)=0$ for every $x>c-r$ follows from Equation \eqref{var_sim_exp} in Theorem \ref{result_variance}.
\end{namedcorollary}


The proof of this corollary requires some algebraic computation and is described in Section~\ref{proof_corollary_variance}.




We now discuss the proof of Theorem \ref{result_variance} and to prove this theorem, we first state and prove the following Claim \ref{f_diff}.

\begin{namedclaim}{Claim}{\label{f_diff}}
Define $\mathfrak{n}^D_{i,S}$ as the number of times job $a_i$ occurs amnogst the servers in $S$ as in the proof of Theorem \ref{min_var_gen} (Equation \eqref{n_D_defn}). For any pair of jobs $(a_i,a_j)$ occurring together in exactly $m$ servers, we can say that \\

$$f(i,j)= \sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1} (\mathfrak{n}^D_{j,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{j,\hat{S}}>1} = g(m)$$ where $g(.)$ is defined in Theorem \ref{result_variance}.

\remove{
\begin{itemize}
    \item $g(p+1)-g(p)= \left[{{(c-2) \choose (x-1)}}-2{{(c-r-1) \choose (x-1)}}+ {{(c-2r+m-1)\choose (x-1)}}\right]$
    \item $g(0)= \sum\limits_{i=2}^{r+1}\sum\limits_{j=2}^{r+1} (i-1).(j-1).{(c-2r) \choose (x-i-j)}.{r \choose i}.{r\choose j}$
\end{itemize}

}

%Note that $f(i,j)$ 

\end{namedclaim}


\begin{proof}
%We first argue that the function $f(i,j)$ is just a function of $m,n,k,r$ and $c$ but not a function of precisely which $m$ servers are assigned both jobs $a_{i}$ and $a_{j}$. Let us alternately denote $\mathfrak{n}^{D}_{i,j,\hat{S}}$ as the number of servers in $\hat{S}$ which are assigned both jobs $a_{i}$ and $a_{j}$.

Consider any pair of jobs $(a_i,a_j)$ occurring together in exactly $m$ servers. Now, the number of subsets $\hat{S}$ with cardinality $x$ satisfying $\mathfrak{n}^D_{i,j,\hat{S}}=t_{com}$, $\mathfrak{n}^D_{i,\hat{S}}=t_1$ and $\mathfrak{n}^D_{j,\hat{S}}=t_2$ would be a function of $m,t_1,t_2,t_{com}$ and $n,k,r,c$. This follows since we have to select $t_{com}$ servers from a collection of $m$ servers (that contain both $a_{i}$ and $a_{j}$), $t_{1}-t_{com}$ servers from a collection of $r-m$ servers (ones that contain $a_{i}$ but not $a_{j}$), $t_{2}-t_{com}$ servers from a collection of $r-m$ servers (ones that contain $a_{j}$ but not $a_{i}$) and similarly, $c-t_1-t_2+t_{com}$ servers from the remaining $c-r+m$ servers that contain neither job.

Summing over all possible values of $t_1,t_2$ and $t_{com}$ gives us the desired expression of $f(i,j)$ which is a function of $m,n,k,r$ and $c$ but not a function of precisely which $m$ servers are assigned both jobs $a_{i}$ and $a_{j}$. Thus we may write $f(i,j)$ as some function of $m$.



%Note that this follows since these conditions ensure that number of server in which job $a_{i}$ is present but not job $a_{j}$ is given by $m-t_$
 

 
Now consider $f(u,v) = \sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} (\mathfrak{n}^D_{{u},\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{{u},\hat{S}}>1} (\mathfrak{n}^D_{{v},\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{{v},\hat{S}}>1}$ for any pair of jobs $(a_u,a_v)$ occurring together in exactly $m-1$ servers.
		
		
		Let us try to compute the difference between the functions $f(i,j)$ and $f(u,v)$. Let us consider the two pairs of jobs call it $P_1=(a_i,a_j)$ and $P_2=(a_u,a_v)$. As argued above, since the precise set of servers that are assigned both the jobs $a_{i}$ and $a_{j}$ does not factor in the calculations. W.L.O.G, we may assume that servers $s_{1},...s_{{m-1}}$ are shared by both the pairs $P_1$ and $P_2$. Server $s_{{m}}$ is shared by only the pair $P_1= (a_{i},a_{j})$, however only contains $a_{u}$ from pair $P_1$, and server $s_{m+1}$ contains only $a_{v}$ from pair $P_2$ but none of the elements in the other pair $P_1$.
		
		Let $s_{k_1},s_{k_2},...s_{k_{r-m}}$ denote the servers containing only one element each from pairs $P_1$ and $P_2$, say $a_{i}$ (from $P_1$) and $a_{u}$ (from $P_2$), however, $s_{l_1},s_{l_2},...s_{l_{r-m}}$ denote the servers containing only one element each from pairs $P_1$ and $P_2$ say, $a_{j}$ (from $P_1$) and $a_{v}$(from $P_2$). This is because job $a_{i}$ occurs without $a_{j}$ in $(r-m)$ such servers and similarly job $a_{u}$ occurs without $a_{v}$ in $(r-m+1)$ such servers which we have satisfied above. Let us denote the remaining servers by $R$ i.e. $R=\mathcal{S} \setminus \{s_{k_1},s_{k_2},\ldots,s_{k_{r-m}},s_{l_1},s_{l_2},...s_{l_{r-m}},s_1,s_2,\ldots,s_{m+1}\}$ of cardinality $c-2r+m-1$.
		
		Now let us compare the difference between two functions $f(i,j)$ and $f(u,v)$ for each subset $\hat{S}$ of cardinality $x$. We define $\mathfrak{g}(\hat{S})$ in Equation \eqref{diff_equation} such that $f(i,j)-f(u,v)= \sum\limits_{\substack{\hat{S}\subseteq\mathcal{S}\\ |\hat{S}|=x}} h(\hat{S})$.
    
		
		\begin{equation}{\label{diff_equation}}
		h(\hat{S})= (\mathfrak{n}^D_{{i},\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{{i},\hat{S}}>1} (\mathfrak{n}^D_{{j},\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{{j},\hat{S}}>1}- (\mathfrak{n}^D_{{u},\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{{u},\hat{S}}>1} (\mathfrak{n}^D_{{v},\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{{v},\hat{S}}>1}
		\end{equation}
		for all subsets $\hat{S}$ of cardinality $x$.
		
		\begin{enumerate}
			\item If the set $\hat{S}$ neither contains $s_m$ or $s_{m+1}$, then we can say that Equation \eqref{diff_equation} goes to zero.
			\item If the set $\hat{S}$ contains both $s_m$ and $s_{m+1}$, then also we can say that Equation \eqref{diff_equation} goes to 0.
		\end{enumerate}. 

        Thus we now consider the sets $\hat{S}=S\cup \{s_m\},S\cup \{s_{m+1}\}$ and consider the their sum w.r.t the function $h(.)$ for every set $S\subseteq \mathcal{S}\setminus \{s_m,s_{m+1}\}$ i.e. 

        \begin{equation}{\label{diff_equation2}}
          \tilde{h}(S) = h(S\cup \{s_m\}) + h(S\cup \{s_{m+1}\})  
        \end{equation}
    
        %$$$$
    
        
		
		Now consider a subset $S$ where $S\subseteq \mathcal{S}\setminus \{s_m,s_{m+1}\}$ with, $(\alpha+1)$ occurrences of $a_{u}$ and $a_{i}$ in the subset of servers $S$ (i.e. $\mathfrak{n}^D_{u,S}=\mathfrak{n}^D_{i,S}= \alpha+1$) and $(\beta+1)$ occurrences of $a_{v}$ and $a_{j}$ in the subset of servers $S$ (i.e. $\mathfrak{n}^D_{v,S}=\mathfrak{n}^D_{j,S}= \beta+1$) for some $\alpha, \beta \geq 0$. For this set $S$, we compute $\tilde{g}(S)$ as defined in Equation \eqref{diff_equation2}. 
		
	Look at the set $\hat{S}=S \cup \{s_m\}$. For this set, $h(S \cup \{s_{m}\})$, Equation \eqref{diff_equation} goes to $(\alpha+1)(\beta+1)- (\alpha+1)\beta$. Similarly, for the set $h(S \cup \{s_{m+1}\})$, Equation \eqref{diff_equation} goes to $\alpha\beta - \alpha(\beta+1)$. Summing these up we obtain $\tilde{h}(S)=1$ as defined in Equation \eqref{diff_equation2}.
		
	We can also show that if set $S$ contains zero occurrences of $a_{u}$ and $a_{i}$ or zero occurrences of $a_{v}$ and $a_{j}$, $\tilde{g}(S)$ in Equation \eqref{diff_equation2} goes to 0 as both terms $h(S \cup \{s_m\})=h(S \cup \{s_{m+1}\})=0$, however there are $2{{(c-r-1) \choose (x-1)}}- {{(c-2r+m-1)\choose (x-1)}}$ such subsets $S$. This follows from the fact that such a case occurs only when ${S}$ is a subset of  $\{s_{k_1},s_{k_2},...,s_{k_{r-m}}\} \cup R$ or $\{s_{l_1},s_{l_2},...,s_{l_{r-m}}\} \cup R$ and there are $2{{(c-r-1) \choose (x-1)}} - {{(c-2r+m-1)\choose (x-1)}}$ precisely such subsets. However the total number of subsets of $\mathcal{S} \setminus \{s_m,s_{m+1}\}$ of cardinality $x-1$ is given by ${{(c-2) \choose (x-1)}}$. 	
		
		Hence, the function $f(i,j)-f(u,v)$ goes to $\left[{{(c-2) \choose (x-1)}}-2{{(c-r-1) \choose (x-1)}}+ {{(c-2r+m-1)\choose (x-1)}}\right]$ by excluding these cases when $S$ is a subset of $\{s_{k_1},s_{k_2},...,s_{k_{r-m}}\} \cup R$ or $\{s_{l_1},s_{l_2},...,s_{l_{r-m}}\} \cup R$.


 Since $f(i,j)$ equals $g(p)$ and $f(u,v)$ equals $g(p-1)$, we prove 

\begin{equation}{\label{g_p_diff_claim}}
    g(p+1) - g(p) = \left[{{(c-2) \choose (x-1)}}-2{{(c-r-1) \choose (x-1)}}+ {{(c-2r+p-1)\choose (x-1)}}\right]
\end{equation}

 


 Let us now compute $g(0)$. For this let us choose a pair of jobs $(a_{i_1}, a_{i_2})$ which occur together in 0 servers. Thus, we may compute $\sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} (\mathfrak{n}^D_{i_1,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i_1,\hat{S}}>1} (\mathfrak{n}^D_{i_2,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i_2,\hat{S}}>1}$. 


 Now, observe that job $a_{i_1}$ is present in exactly $r$
servers and job $a_{i_2}$ is present in another set of $r$ servers with no overlap between these sets. Thus, the number of ways a set of servers $\hat{S}$ of cardinality $x$ can be chosen satisfying $\mathfrak{n}^D_{i,\hat{S}}=i$ and $\mathfrak{n}^D_{i,\hat{S}}=j$ is given by ${{c-2r\choose x-i-j}}{{r \choose i}}{{r \choose j}}$. Thus, we can observe 


\begin{equation}{\label{g_0_claim}}
    g(0)= \sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} (\mathfrak{n}^D_{i_1,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i_1,\hat{S}}>1} (\mathfrak{n}^D_{i_2,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i_2,\hat{S}}>1} = \sum_{i=2}^{r+1}\sum_{j=2}^{r+1} (i-1)(j-1){{c-2r\choose x-i-j}}{{r \choose i}}{{r \choose j}}
\end{equation}
%$$$$.

We now give a closed-form expression for $g(0)$ below. 
\remove{
Let us now compute $g(0)$ using the expression in Equation \eqref{g_0_claim}. Observe that
 
\begin{equation}{\label{binomial_corollary_1}}
        ry(1+y)^{r-1} + 1 - (1+y)^r = \sum_{t=1}^{r} (t-1) {{r \choose t}} y^t
\end{equation}

\begin{equation}{\label{binomial_corollary_2}}
        ry(1+y)^{r-1} + 1 - (1+y)^r = \sum_{u=1}^{r} (u-1) {{r \choose u}} y^u
\end{equation}

\begin{equation}{\label{binomial_corollary_3}}
        (1+y)^{c-2r} = \sum_{v=0}^{c-2r} {{c-2r \choose v}} y^v
\end{equation}

Multiplying these three expressions \eqref{binomial_corollary_1}, \eqref{binomial_corollary_2} and \eqref{binomial_corollary_3}, we get that $\sum_{i=2}^{r+1}\sum_{j=2}^{r+1} (i-1)(j-1) {{c-2r \choose x-i-j}}{{r \choose i}}{{r \choose j}}$ is the coefficient of $y^x$ in $\left(r(1+y)^{r-1} + 1 - (1+y)^r\right)^2(1+y)^{c-2r}$. %Note that since $x>c-r$, we obtain 


\begin{align}{\label{g_0_exp}}
    & \sum_{i=2}^{r+1}\sum_{j=2}^{r+1} (i-1)(j-1) {{c-2r \choose x-i-j}}{{r \choose i}}{{r\choose j}}\nonumber\\ 
    = &r^2 {{c-2 \choose x-2}} - 2r {{c-1 \choose x-1}} + {{c \choose x}} - 2{{c-r \choose x}} + 2 r{{c-r-1 \choose x-1}}
\end{align}
}


Coupled with results in equations \eqref{g_0_claim} and \eqref{g_p_diff_claim} and \eqref{g_0_exp}, we prove Claim \ref{f_diff}.
 

  
  
  
  %We subtract from ${{(c-2) \choose (x-1)}}$ as it denotes the total number of possible subsets $S\subseteq \mathcal{S} \setminus \{s_m,s_{m+1}\}$ of cardinality $x-1$.
\end{proof}

We now prove Theorem \ref{result_variance} using Claim \ref{f_diff}.

% where $\mathfrak{n}^D_{i,S}$ denotes the number of servers in set $S$ which have been assigned the job $a_i$ under the assignment scheme $D$.


 
 %Also under the constraint $n=c$, we obtain $\mathbbm{E}_{{D},x}[d]=n.\left(1 - \frac{{{n-x \choose r }}}{{{n \choose r}}}\right)$


%We first state our main theorem below on attaining the least variance on the number of different jobs under the setup.

\begin{proof}

    Let us compute the expectation of distinct jobs($d$) received. For the computation of $d$, we denote by $\mathfrak{n}^D_{i,\hat{S}}$ denoting the number of servers in $\hat{S}$ to which job $a_i$ is assigned to under the assignment scheme $D$ or maybe defined as $\mathfrak{n}^D_{i,\hat{S}}= |(\text{sup}(A[i,:]) \cap \hat{S})|$ in terms of assignment matrix $A_D$ similar to the proof of Theorem \ref{min_var_gen}. Observe that $\mathfrak{n}^D_{i,\hat{S}}$ can take any value from $0$ to $r$.

Now, observe that the number of distinct jobs $d$ received at the master when any  servers in set $S$ are able to communicate with the master is given by 


\begin{equation}{\label{constr_d}}
    d = \left|\bigcup_{j \in \hat{S}}\text{supp}(A_D[:,j])\right|= (k\times x- \sum\limits_{i=1}^{n} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1})
\end{equation}

where $x$ denotes the cardinality of set $\hat{S}$. Note that the term $\sum\limits_{i=1}^{n} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1}$ excludes those jobs which have been received multiple times from various servers in $\hat{S}$.



    In the next set of equations, we give an expression for the variance on the number of distinct jobs and apply its definition i.e. $\text{var}(X) = \mathbbm{E}[X^2]- (\mathbbm{E}[X])^2$ and observe that in our set-up every subset of servers with cardinality $x$ is equally likely to be the only set of servers communicating with the master. 
	
	
	
	\begin{align}{\label{sigma_expression}}
	\sigma_{D,x}(d) &=
	\sigma_{D,x}(k\times x- \sum\limits_{i} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1})\nonumber\\
	& \overset{(d)}{=} \sigma_{D,x} \left(\sum\limits_{i} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1}\right)\nonumber\\
	% & = \mathbb{E}_{D,x}[d^2]- {(\mathbb{E}_{D,x}[d])}^2\\
	% & = \frac{\sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} {(k\times x- \sum\limits_{i} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1})}^2}{\sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} 1} - \left(\frac{\sum\limits_{\substack{\hat{S} \subset \mathcal{S}; |\hat{S}|=x}} {(k\times x- \sum\limits_{i} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1})}}{\sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} 1}\right)^2\\
	& = \frac{\sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} {\left(\sum\limits_{i=1}^{n} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1}\right)}^2}{\sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} 1} - \left(\frac{\sum\limits_{\substack{\hat{S} \subset \mathcal{S}; |\hat{S}|=x}} {(\sum\limits_{i=1}^{n} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1})}}{\sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} 1}\right)^2\nonumber\\
	& \overset{(e)}{=} \frac{\sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} (\sum\limits_{i=1}^{n} \sum\limits_{j=1}^{n} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1} (\mathfrak{n}^D_{j,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{j,\hat{S}}>1})}{\sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} 1} - \left(\frac{\sum\limits_{i=1}^{n} \sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\ |\hat{S}|=x}} {((\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1})}}{{c \choose x}}\right)^2\nonumber\\
	& \overset{(f)}{=} \frac{\sum\limits_{i=1}^{n} \sum\limits_{j=1}^{n} \sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1} (\mathfrak{n}^D_{j,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{j,\hat{S}}>1}}{{c \choose x}}- \left(\frac{n\sum\limits_{t=1}^{r-1} t{r \choose (t+1)} {(c-r) \choose (x-t-1)}}{{c \choose x}}\right)^2\\
    & \overset{(i)}{=} \frac{\sum\limits_{i=1}^{n} \sum\limits_{j=1}^{n} \sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1} (\mathfrak{n}^D_{j,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{j,\hat{S}}>1}}{{c \choose x}}- \left(\frac{n{{c-r \choose x}}}{{{c \choose x}}} + n \times\left(\frac{rx}{c}-1\right)\right)^2
\end{align}

%\frac{n{{c-r \choose x}}}{{{c \choose x}}} + n \times(\frac{rx}{c}-1)
	
Let us attempt to compute variance of the number of distinct jobs.
	
$(d)$ follows since $\sigma(c-X) = \sigma(X)$ where $c$ is a constant and $X$ is the random variable. 

The first term in $(e)$ follows since $(\sum\limits_i b_i)^2 = \sum\limits_i \sum\limits_j b_i b_j$. The first term in $(f)$ follows from interchange of summations whereas the second term follows from $(c)$ in previous equation \eqref{removal_comp_mean}. Note the second term in $(i)$ follows using the Equation \eqref{temp_result_removal} in the proof of Theorem \ref{result_mean}.

Now, consider the numerator of the first term of equation \eqref{sigma_expression} which we discuss below. 

\begin{align}{\label{f_i_j_exp}}
	& \sum\limits_{i=1}^{n} \sum\limits_{j=1}^{n} \sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1} (\mathfrak{n}^D_{j,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{j,\hat{S}}>1}\nonumber\\
	= & 2\sum\limits_{1\leq i < j\leq n} \sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1} (\mathfrak{n}^D_{j,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{j,\hat{S}}>1}
	+ & \sum\limits_{1\leq i =j\leq n} \sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1} (\mathfrak{n}^D_{j,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{j,\hat{S}}>1}\nonumber\\
	\overset{(g)}{=} &  2.\sum\limits_{p=0}^{r} \mathfrak{m}^{D}(p) g(p) + \sum\limits_{1\leq i \leq n} \sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} ((\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1})^2\nonumber\\
	\overset{(h)}{=} &  2\sum\limits_{p=0}^{r} \mathfrak{m}^{D}(p)g(p) + n\sum\limits_{t=1}^{r-1} t^2{r \choose (t+1)} {(c-r) \choose (x-t-1)}
\end{align}
	
%	Note the first term in $(a)$ follows since $f(i,j)= \sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1} (\mathfrak{n}^D_{j,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{j,\hat{S}}>1}$ and recall that $\mathfrak{m}^D(p)$ is the precisely the number of pairs of jobs such that they are present together in exactly $m$ servers. The second term in $(b)$ is computed using a very similar technique as used in theorem \ref{mean_equality} for computation of $\sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} \left(\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1}\right)^2$ in Equation \eqref{removal_comp_mean}.    

Note that $(g)$ follows from Claim \ref{f_diff} where we show that $\sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}}(\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1} (\mathfrak{n}^D_{j,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{j,\hat{S}}>1}$ is given by the function $g(.)$ defined in Theorem \ref{result_variance}. The second term in $(h)$ follows from a similar argument used in the proof of Theorem \ref{result_mean} in Equation \eqref{removal_comp_mean}.


Now, we compute the term ($\sum\limits_{t=1}^{r-1} t^2 {{r \choose t+1}}{{c-r \choose x-t-1}}$) from Equation \eqref{f_i_j_exp}.

%Observe that 
%\begin{equation}{\label{binomial_corollary_4}}
 %   r(r-1) y^2(1+y)^{r-2} - ry(1+y)^{r-1} - 1 + {(1+y)^r} = \sum_{t=0}^{r} t^2 {{r \choose t+1}} y^{t+1}
%\end{equation}

%\begin{equation}{\label{binomial_corollary_5}}
%        (1+y)^{c-r} = \sum_{v=0}^{c-r} {{c-r \choose v}} y^v
%\end{equation}

%Multiplying equations \eqref{binomial_corollary_4} and \eqref{binomial_corollary_5}, we obtain $\sum\limits_{t=1}^{r-1} t^2 {{r \choose t+1}}{{c-r \choose x-t-1}}$ to be the coefficient of $y^{x}$ in $r(r-1) y^2(1+y)^{c-2} - ry(1+y)^{c-1} - (1+y)^{c-r} - (1+y)^c$, thus,  

%\begin{equation}{\label{temp_corollary}}
%        \sum\limits_{t=1}^{r-1} t^2 {{r \choose t+1}}{{c-r \choose x-t-1}} = r(r-1) {{c-2 \choose x-2}} - r{{c-1 \choose x-1}} -{{c-r \choose x}}+ {{c \choose x}}
%\end{equation}

Thus, equations \eqref{temp_corollary}, \eqref{f_i_j_exp} and \eqref{sigma_expression} prove Theorem \ref{result_variance}.


%$$f(i,j) = $$


\end{proof}

}

==> server-jobs-equal.tex <==
\section{Assignment equivalence when number of servers equals number of jobs}\label{job_no_server_no_identical_section}


%Recall that we defined the $\mathfrak{m}^D(m)$ w.r.t pairs of jobs. However, since the jobs and the servers may be treated interchangeably, we can also describe the entire framework w.r.t pairs of servers and count the number of pairs of servers that have exactly $m$ jobs in common.

So far, we have been viewing the $(n,k,r,c)$ balanced assignment as a task of assigning jobs to servers. Equivalently, one can also view the same balanced assignment as assigning servers to jobs. Since every job is assigned to $r$ distinct servers, there is a total of ${r \choose 2}$ server pairs that can be associated to each job. Like the shape vector $h_D$ that was built from information about frequency of job-pairs at the servers in a given assignment, one may build an equivalent shape vector based on frequency of server-pairs that are associated to the jobs. Thus every server-pair can possibly be associated to $m$ jobs, where $0 \le m \le k$. Thus, the shape vector corresponding to server assignment viewpoint would be a vector in $\mathbb{N}^{k+1}$. One may now define compact balanced $(n,k,r,c)$ server assignments as those balanced assignments that have server shape vector having at most two nonzero entries. We may view proximally compact balanced $(n,k,r,c)$ server assignment, through an analogous definition.  
%We now define a pairwise job-balanced assignment scheme which would be identical to proximally minimal compact assignment as described in Definition \ref{proximally_minimal_compact}. Observe that it is the same definition restated in a slightly different way.

%\begin{nameddefinition}{Definition}{\label{pair_job_balanced_definition}}
 %   (Pairwise balanced job $(n,k,r,c)$ assignment): Given a balanced $(n,k,r,c)$ assignment, we call it  pairwise balanced $(n,k,r,c)$ job assignment if for every pair of distinct jobs $a_i$ and $a_j$ in $\mathcal{A}$, the number of servers which are assigned both $a_i$ and $a_j$ is exactly $\ell$ or $\ell+1$ for some integer $\ell$.
%\end{nameddefinition}


%Recall that we defined $\mathfrak{m}^D(m)$ w.r.t pairs of jobs. However, since the jobs and the servers may be treated interchangeably, we can also describe the entire framework w.r.t pairs of servers and count the number of pairs of servers that have exactly $m$ jobs in common.


%We could therefore define a pairwise server-balanced assignment scheme. Observe that this definition interchanges the roles played by the jobs and the servers.

\begin{nameddefinition}{Definition}{\label{pair_server_balanced_definition}}
    Given a balanced $(n,k,r,c)$ assignment, we call it  proximally compact  $(n,k,r,c)$ server assignment if for every pair of distinct servers $s_i$ and $s_j$ in $\mathcal{S}$, the number of jobs assigned to both $s_i$ and $s_j$ simultaneously is exactly $\ell$ or $\ell+1$ for some integer $\ell$.
\end{nameddefinition}

\begin{namedlemma}{Lemma}{\label{lemma_on_l_server}}
    For any proximally compact $(n,k,r,c)$ server assignment, we must have $\ell=\Bigl\lfloor\frac{n.{{r \choose 2}}}{{{c \choose 2}}}\Bigr\rfloor$
\end{namedlemma}

This lemma can be proved in a very similar way as that of Lemma \ref{lemma_on_l_proximally_minimal}.

We may observe that in general, proximally compact server assignment schemes may not be proximally compact job assignment schemes. We demonstrate that with an Example \ref{pairwise_balanced_server} below.


\begin{example}{\label{pairwise_balanced_server}}{\rm
    We now describe a proximally compact $(14,6,3,7)$ server assignment which is not a proximally compact job assignment in Table \ref{pairwise_balanced_server_assn}. Note that in this scheme, every pair of servers have exactly $2$ jobs in common and therefore proximally compact server assignment. However, some pairs of jobs appear together in one server like $(a_1,a_2)$, some pairs of jobs appear together in $2$ servers like pairs of jobs $(a_1,a_8)$ and some pairs of jobs like $(a_3,a_{10})$ appear together in 3 servers and thus it is not proximally compact job assignment. %However, it should be noted that it continues to be a compact job assignment, as only two entries of the job shape vector $h_D$ are nonzero. 
    }
\end{example}


\begin{table}[!h]
    \centering
{
	\begin{tabular}{|c|c|c|c|c|c|c|c| } 
		\hline
	{{\diagbox[width = 5 em]{Jobs}{Servers}}}& $s_1$ & $s_2$ & $s_3$ & $s_4$ & $s_5$ & $s_6$ &$s_7$ \\
    \hline
    $a_1$ & $\text{}$ & 1 & $\text{}$ & 1 & $\text{}$ & 1 & $\text{}$ \\
    \hline
    $a_2$ & 1 & $\text{}$ & $\text{}$ & 1 & 1 & $\text{}$ & $\text{}$\\
        \hline
     $a_3$ & $\text{}$ & $\text{}$ & 1 & 1 & $\text{}$ & $\text{}$ & 1 \\
        \hline
    $a_4$ & 1 & 1 & 1 & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$\\
    \hline
    $a_5$ & $\text{}$ &1 & $\text{}$ & $\text{}$ & 1 & $\text{}$ &  1 \\
        \hline
     $a_6$ & 1 & $\text{}$  & $\text{}$ & $\text{}$ &  $\text{}$  & 1 & 1\\
        \hline
    
    $a_7$ & $\text{}$ & $\text{}$ & 1 & $\text{}$ & 1& 1 &$\text{}$ \\
    \hline
    $a_8$ & 1 & $\text{}$ & $\text{}$ & 1 & $\text{}$ & 1 & $\text{}$ \\
    \hline
    $a_9$ & $\text{}$ & 1 & $\text{}$ & 1 & 1 & $\text{}$ & $\text{}$\\
        \hline
     $a_{10}$ & $\text{}$ & $\text{}$ & 1 & 1 & $\text{}$ & $\text{}$ & 1 \\
        \hline
    $a_{11}$ & 1 & 1 & 1 & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$\\
    \hline
    $a_{12}$ &1 & $\text{}$ & $\text{}$ & $\text{}$ & 1 & $\text{}$ &  1 \\
        \hline
     $a_{13}$ & $\text{}$ & 1  & $\text{}$ & $\text{}$ &  $\text{}$  & 1 & 1\\
        \hline
    
    $a_{14}$ & $\text{}$ & $\text{}$ & 1 & $\text{}$ & 1 & 1 & $\text{}$  \\
    \hline
        
	\end{tabular}
 }
	\vspace{1 em}
	\caption{Assignment of jobs to various servers in a proximally compact $(14,6,3,7)$ server assignment scheme}
	\label{pairwise_balanced_server_assn}
\end{table}


However, when $n=c$ our subsequent result shows that proximally compact server assignment schemes and proximally compact job assignment schemes are equivalent.



\begin{namedtheorem}{Theorem}{\label{job_server_pairs_identical}}
Amongst balanced $(n,k,k,n)$ assignments, every proximally compact $(n,k,k,n)$ job assignment is also a proximally compact server assignment and vice-versa.  
\end{namedtheorem}

To prove this theorem, we first prove Lemma~\ref{var_equal}.

We define a random variable $Y^D$ as follows for balanced $(n,k,r,c)$ assignment $D$ as the number of servers in which a pair of jobs chosen uniformly at random occur together. Formally, we can say that 

\begin{equation}{\label{y_d_defn}}
    \mathbb{P}[Y^D = p] = \frac{\mathfrak{m}^D(p)}{{{n \choose 2}}} \text{for any integer $p \in [0,r]$}
\end{equation}

Observe that this is a valid distribution as $\sum\limits_{p=0}^{r} \mathfrak{m}^D(p) = {{n \choose 2}}$ in Equation \eqref{proporty_m_1}.




\begin{lemma}{\label{var_equal}}
	For any balanced $(n,k,r,c)$ assignment $D$, the variance of $Y^D$ is linearly proportional to the variance of distinct jobs $d$ received at master when any 2 servers chosen uniformly at random return i.e. are able to communicate their results to the master. We can also state it as follows.
	
	\begin{equation}\label{last_lem}
	\sigma_{D,2}(d) = \frac{{{n \choose 2}}\sigma(Y^D) + \frac{\left(c{k \choose 2} \right)^2}{{n \choose 2}} + n\left({r \choose 2}\right) - c\left({k \choose 2}\right)}{{c \choose 2}} - \left(\frac{n{r \choose 2} }{{c \choose 2}}\right)^2
	\end{equation}

 Further for $n=c$, we can say that $\sigma(Y^D)= \sigma_{D,2}(d)$
\end{lemma}

\begin{proof}
Observe that $g(0,x) = \sum\limits_{i=2}^{r+1}\sum\limits_{j=2}^{r+1} (i-1)(j-1){(c-2r) \choose (x-i-j)}{r \choose i}{r\choose j}$ from equation~\eqref{g_0_exp} and therefore $g(0,2) = 0$. Further, using equation~\eqref{g_p_diff}, we have $g(m+1,2)-g(m,2) = (c-2) -2(c-r-1)+ (c-2r+m) = m$. Therefore, $g(m,2)= 1+2+\cdots + (m-1) = \frac{m(m-1)}{2}$.

Consider the numerator of first term in $\sigma_{D,x}(d)$ in equation~\eqref{var_sim_exp} which was shown to be $2\sum\limits_{m=0}^{r}\mathfrak{m}^{D}(m)g(m,x) + n\left(\sum\limits_{t=1}^{r-1} t^2{r \choose (t+1)} {(c-r) \choose (x-t-1)}\right)$. Note that here we consider $x=2$ as we are considering the case when only two servers communicate back to the master. So for $x=2$,
	
	%Thus the first term in numerator of $\sigma_{D,2}(d)$ becomes $2\sum\limits_{m=0}^{r}g(m,x) + n.\left(\sum\limits_{t=1}^{r-1} t^2{r \choose (t+1)} {(c-r) \choose (1-t)}\right)$.
	
	%Now, observe that $g(0,x) = \sum\limits_{i=2}^{r+1}\sum\limits_{j=2}^{r+1} (i-1).(j-1).{(c-2r) \choose (x-i-j)}.{r \choose i}.{r\choose j}$ from Equation \eqref{g_0_exp}. For $x=2$, we can show that it goes to 0 as $g(m,2)-g(m-1,2)$ reduces to $\left[(n-2) -2(n-k-1)+ (n-2k+m-1) \right] = m-1$ from Equation \eqref{g_p_diff} in Theorem \ref{result_variance}. Thus we can argue that $g(m,2)= 1+2+\ldots + m-1 = \frac{m(m-1)}{2}$.
	
     %Consider $n.\left(\sum\limits_{t=1}^{k-1} t^2{r \choose (t+1)} {(c-r) \choose (1-t)}\right)$ = $n.\left({r \choose 2}\right)$.
	
	%Thus for $x=2$, 
	
	\begin{align*}
	2\sum\limits_{m=0}^{r}\mathfrak{m}^{D}(m)g(m,2) + n\left(\sum\limits_{t=1}^{k-1} t^2{r \choose (t+1)} {(c-r) \choose (2-t-1)}\right)
	= & \sum\limits_{m=0}^{r} \mathfrak{m}^{D}(m)m(m-1) + n{r \choose 2}\\
	\overset{(a)}{=} & \sum\limits_{m=0}^{r} m^2 \mathfrak{m}^{D}(m) + n{r \choose 2} - c{k \choose 2}
	\end{align*}
	
	$(a)$ follows since $\sum\limits_{m=0}^{r}m\mathfrak{m}^{D}(m)= c{k \choose 2}$ in Equation \eqref{property_m_2}.
	
	Therefore,  
	\begin{align}{\label{sigma_Exp_x_2}}
	\sigma_{D,2}(d)
	%= & \frac{2.\sum\limits_{m=0}^{r}\mathfrak{m}^{D}(m)g(m,2) + n\left(\sum\limits_{t=1}^{k-1} t^2{k \choose (t+1)} {(n-k) \choose (1-t)}\right)}{{c \choose 2}} - \left(\frac{n\sum\limits_{t=1}^{r-1} t{r \choose (t+1)} {(c-r) \choose (1-t)}}{{c \choose 2}}\right)^2\nonumber\\ 
	= & \frac{\sum\limits_{m=0}^{r} m^2 \mathfrak{m}^{D}(m) + n{r \choose 2} - c{k \choose 2}}{{c \choose 2}} - \left(\frac{n{r \choose 2} }{{c \choose 2}}\right)^2
	\end{align} 


Observe $\mathbbm{E}[Y^D]= \frac{\sum_{m=0}^{r} m\mathfrak{m}^D(m)}{{{n \choose 2}}} = \frac{c{{k \choose 2}}}{{{n \choose 2}}}$ as $\sum\limits_{m=0}^{r}m\mathfrak{m}^{D}(m)= c{k \choose 2}$ by equation~\eqref{property_m_2} and using the definition of $Y^D$ in Equation \eqref{y_d_defn}.

 \begin{align}{\label{var_y_exp}}
      \sigma(Y^D)
     = & \mathbbm{E}[(Y^D)^2] - (\mathbbm{E}[Y^D])^2\nonumber\\
     = & \frac{1}{{n \choose 2}} \sum_{m=0}^{r}m^2 \mathfrak{m}^D(m) - \left(\frac{c{{k \choose 2}}}{{{n \choose 2}}}\right)^2
 \end{align}
	
	%%$(b)$ follows since $\sum\limits_{p=0}p.\mathfrak{n}^D_{p,D}= n.{k \choose 2}$.  
	
Thus, using equations \eqref{var_y_exp} and \eqref{sigma_Exp_x_2}, we obtain the expression \eqref{last_lem} in the statement of the lemma. Further, when $n=c$, then $r=k$ and the two equations \eqref{var_y_exp} and \eqref{sigma_Exp_x_2} become equal.
	%Now we know that $\text{var}_D(y) = \frac{\sum\limits_{p=0}^{r}p^2.\mathfrak{n}^D_{p,D} }{{n \choose 2}} - \left(\frac{c{k \choose 2} }{{n \choose 2}}\right)^2$
	%We also know from theorem \ref{mean_equality} that  $\mathbbm{E}_{D,2}[d]= 2.k - \frac{n.\sum\limits_{t=1}^{r-1} t{r \choose (t+1)} {(c-r) \choose (2-t-1)}}{{c \choose 2}} =  2k - \frac{n{r \choose 2}}{{c \choose 2}}$ whereas $\mathbbm{E}[y]= \frac{\sum\limits_{p=0}^{r}p.\mathfrak{n}^D_{p,D}}{{n \choose 2}} = \frac{c.{{k \choose 2}}}{{{n \choose 2}}}$.
\end{proof}

%We now prove a lemma showing that the set of pairwise balanced job assignments is identical to the set of pairwise balanced server assignments when the number of jobs and the servers are identical.

We now prove Theorem \ref{job_server_pairs_identical}.


\begin{proof}

    Consider the set of balanced $(n,k,k,n)$ assignment schemes. Now recall $Y^D$ denoted the number of servers where a pair of jobs chosen uniformly at random occurs together and for $n=c$ and $k=r$, we have 
    \begin{equation}{\label{equality_var_local}}
        \sigma_{D,2}(d)=\sigma(Y^D).
    \end{equation}
     
    
    Further $\mathbb{E}[Y^D]=\frac{n{{k \choose 2}}}{{{n \choose 2}}}$. %which follows since every server has exactly ${{k \choose 2}}$ pairs of jobs since each server is balanced (and is assigned $k$ jobs) and we have exactly $n$ servers. However, we have exactly ${{n \choose 2}}$ total number of pairs of jobs hence this equality of expectation on $y$ holds true. 
    Also, observe from Theorem \ref{all_mean} (under $x=2,n=c$ and $k=r$ ) that
    \begin{equation}{\label{equality_mean_local}}
        \mathbb{E}_{D,2}[d] = n\left(1-\frac{(n-k)(n-k-1)}{n(n-1)}\right)=\left(2k-n\frac{k(k-1)}{n(n-1)}\right) = \mathbb{E}_{D}[2k-Y^D]
    \end{equation}
    %. Thus, $\mathbb{E}_{D,2}[2k-d]=$.
    
    
    
    
    We first show that every proximally compact $(n,k,k,n)$ job assignment is also a proximally compact server assignment scheme.

    Suppose not and consider a balanced assignment scheme $D$ which is not a proximally compact server assignment but is a proximally compact job assignment. Now let us consider the scenario where $x=2$ (exactly 2 randomly chosen servers) are able to communicate with the master. Now if $D$ is not a proximally compact server assignment, then $d$ (the number of distinct jobs received) can take at least two  distinct integral values which are non-consecutive, hence $2k-d$ also has a support of at least $2$ distinct non-consecutive integral values. However the random variable $Y^D$ has a support of at most 2 over two consecutive indices (since it is a proximally compact job assignment). Now observe that random $2k-d$ and $Y^D$ have the same expectation (shown above in Equation \eqref{equality_mean_local}). Therefore the variance of $2k-d$ is clearly more than that of $Y^D$ which contradicts equation \eqref{equality_var_local}.


    Now we consider the reverse situation where a balanced assignment scheme is a proximally compact server assignment but not proximally compact job assignment. Again consider the scenario where $x=2$ (exactly 2 randomly chosen servers) are able to communicate with the master. The number of distinct jobs received at the master $d$ can take at most 2 consecutive values (as it is a proximally compact server assignment) and therefore the random variable $2k-d$ has a support of at most 2 over two consecutive indices. Suppose the assignment scheme is not proximally compact job assignment, $Y^D$ has a support of at least 2 elements which are non consecutive. As the random variables $Y^D$ and $2k-d$ have the same expectation according to \eqref{equality_mean_local}, hence the variance of $Y^D$ has to be clearly larger than that $2k-d$ which is turn contradicts equation~\eqref{equality_var_local}.

    Thus, the set of proximally compact job assignments is identical to the set of proximally compact server assignments.
\end{proof}


Thus, Theorem \ref{job_server_pairs_identical} ensures that when the number of servers equals the number of jobs, proximally compact server assignment and proximally compact job assignments minimise the variance of the number of distinct jobs received at the server as shown in Theorem \ref{job_server_pairs_identical}.



==> some-constr-descr.tex <==
\remove{
\subsection{Construction using vector spaces for some $K \neq 1$ }
%Let us discuss such a construction. Choose a finite field vector space of dimension $N$, Let us denote each job as the subspaces of this vector space of dimensionality $K$. Also we denote each server as a subspace of dimensionality $N-K$ ($N-K>K$). Now only those jobs are present in a  server such that the vector-space corresponding to a job is the  subspace of the vector-space denoting the corresponding server. 	

%Note that the number of jobs and server is same since number of subspaces of dimensionality $N-K$ is same as the number of subspaces of dimensionality $K$. Also by geometry we can show that each sub-space of dimensionality $K$ has a fixed number of sub-spaces of dimensionality $N-K$. Thus both the conditions in \ref{setting_condition} are satisfied.

We construct a distribution as described in \ref{sub_space_constr} for some $K\neq 1$ and show that it may not have the least variance for every $x$

%We would like to show that such distributions need not have the least variance.

Let us consider an example $N=6, K=2$ and a binary finite field.

So in this case $n$ becomes the number of ways to select 2 dimensionsal sub-spaces from a 6-dimensional subspace i.e., $\frac{(2^6-1)(2^6-2)}{(2^2-1)(2-1)}=31\times 21=651$.

We also show that $k$ is number of 2-dimensional spaces of a 4-dimensional subspace i.e. $35$.


Consider any 2 pair of jobs. There could be 2 possibilities.

\begin{enumerate}
	\item The vector spaces denoting each job intersect at a sub-space of dimensionality 0.
	
	In this case, the union of the two sub-spaces form a 4-dimensional sub-space and there could exactly be one server containing both of them.
	
	However the number of pairs of such servers can be shown to be 31*21*280.
	
	We argue this by choosing a two-dimensional subspace and calculating how many sub-spaces have 0 dimensional intersection which can be shown to be $q^{2^2} \bracenom{2}{2} \bracenom{4}{2}= 560$
	(reference- dissertion Trauttman) where $\bracenom{n}{k}$ denotes the number of subspaces of dimensionality $k$ in a vector space of dimension $n$. Note $q=2$ since we consider a binary field.
	
	Thus the total number of such pairs are $31*21*560/2 = 31*21*280$.
	
	\item The vector spaces denoting each job intersect in a sub-space of dimensionality 1.
	
	In this case, the union of two sub-sapces form a 3 dimensional sub-space which can be a sub-space of 7 four-dimensional sub-spaces. Also there exist 31*21*45 such pairs with the  dimensionality of the intersection subspace to be 1.
	
	We argue this by choosing a two-dimensional subspace and calculating how many sub-spaces have 1 dimensional intersection which can be shown to be $q^{1^2} \bracenom{2}{1} \bracenom{4}{1}= 90$
	(reference- dissertion Trauttman) where $\bracenom{n}{k}$ denotes the number of subspaces of dimensionality $k$ in a vector space of dimension $n$. Note $q=2$ since we consider a binary field.
	
	Thus the total number of such pairs are $31*21*90/2 = 31*21*45$.
	 
	
\end{enumerate}


Let us denote this distribution by $\mathcal{D}_1$. Thus $\mathfrak{n}^D_{1,\mathcal{D}_1}= 31*21*280$ and $\mathfrak{n}^D_{7,\mathcal{D}_1}= 31*21*45$ Also $\mathfrak{n}^D_{t,\mathcal{D}_1} = 0$  for all $t \neq 1,7$.


Recall from the proof of Theorem 3 that $f(i,j)-f(u,v) = \left[{{(n-2) \choose (x-1)}}-2{{(n-k-1) \choose (x-1)}}+ {{(n-2k+m-1)\choose (x-1)}}\right]$ where job $a_{i}$ and job $a_{j}$ denote a pair of jobs which occur together in exactly $m$ servers.
 
Also recall that $f(i,j) = \sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} (\mathfrak{n}^D_{{i},\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{{i},\hat{S}}>1} (\mathfrak{n}^D_{{j},\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{{j},\hat{S}}>1}$ which is a sub-expression in the variance of $d$. 


Now let us denote $p(m) = f(i,j)-f(u,v)= \left[{{(n-2) \choose (x-1)}}-2{{(n-k-1) \choose (x-1)}}+ {{(n-2k+m-1)\choose (x-1)}}\right]$.

Note that $p(m+1)-p(m) = {{(n-2k+m)\choose (x-1)}}- {{(n-2k+m-1)\choose (x-1)}}= {{(n-2k+m-1)\choose (x-2)}}$ which also increases with $m$.


Let us now construct a new distribution $\mathcal{D}_2$.

Choose a basis vector of this vector space and denote it as $\{b_1,b_2,b_3,b_4,b_5,b_6\}$.

We choose a server $s_1$ with basis vectors as $\{b_1,b_2,b_3,b_4\}$ and job $a_1$ with basis vectors as $\{b_1,b_2\}$. Choose server $s_2$ with basis vectors as $\{b_3,b_4,b_5,b_6\}$ and job $a_2$ with basis vectors $\{b_5,b_6\}$. Also denote the job $a_3$ with basis vectors $\{b_3,b_4\}$.

Thus job $a_1$ would only belong in server $s_1$ and job $a_2$ would only belong in server $s_2$. Also job $a_3$ would belong in both the servers. No other job would belong in both the servers since all the basis vectors $\{b_1,b_2,b_3,b_4,b_5,b_6\}$ are linearly independent. Also job $a_1$ would have zero dimensional intersection with every job in $s_2$, similarly job $a_2$ would have zero dimensional intersection with every job in $s_1$.


Now we exchange job $a_1$ in server $s_1$ with job $a_2$ in server $s_2$.

We now compute the number of jobs in $s_1$ with which $a_1$ has intersection of dimensionality 1 which can be computed to be $q^{1^2} \bracenom{2}{1} \bracenom{2}{1}= 18$ where $\bracenom{n}{k}$ denotes the number of subspaces of dimensionality $k$ in a vector space of dimension $n$. (from Trautmann dissertion that I read initially). We denote these jobs by the set $R_{1,s_1}$. Note $q=2$ as we use a binary field. 

Similarly the number of jobs in $s_1$ with which $a_1$ has intersection of dimensionality 0 can be computed to be $q^{2^2} \bracenom{2}{0} \bracenom{2}{0}= 16$. Note that job $a_3$ would also be part of this set. After removing $a_3$ from this set of jobs, we  denote it by set $R_{0,s_1}$.

Similarly we also define sets $R_{0,s_2}$ and $R_{1,s_2}$ when we use the servers $s_2$ and job $a_2$.

Now consider a pair of jobs with one job in $R_{1,s_1}$ and job $a_1$. The common servers for these jobs would reduce from 7 to 6 after the exchange. As we saw above there would be 18 such pairs. Now consider a pair of jobs with one job in $R_{0,s_1}$ and job $a_1$. The common servers for these jobs would reduce from 1 to 0 post exchange and there are 15 such pairs. Now consider a pair with one job in $R_{1,s_2} \cup R_{0,s_2}$ and the other job $a_1$. The common servers for these jobs would increase from 1 to 2 post exchange and there are 33 such pairs. However note that common servers for the pair $(a_1,a_3)$ would remain the same.

Exactly same argument can be made w.r.t job $a_2$.

Thus, $\mathfrak{n}^D_{1,\mathcal{D}_2}=31\times 21\times 280 - (15+33)\times 2$ and $\mathfrak{n}^D_{2,\mathcal{D}_2} = 33\times 2$, $\mathfrak{n}^D_{6,\mathcal{D}_2}= 18\times 2$, $\mathfrak{n}^D_{7,\mathcal{D}_2}= 31\times 21\times 45-18\times 2$, $\mathfrak{n}^D_{0,\mathcal{D}_2}= 15\times 2$ and $\mathfrak{n}^D_{t,\mathcal{D}_2}=0$ for all $t\neq 0,1,2,6,7$.


\remove{
Choose two jobs $b$ and $c$ such that the vector spaces denoting them intersect with dimensionality 0.

Choose the server $s_1$ such that it has only zero dimensional overlap with job $c$, server $s_2$ such that it has only zero dimensional overlap with job $b$. Thus server $s_1$ has job $b$ and server $s_2$ has job $c$.

Now let us exchange job $a_1$ from server $s_1$ and job $a_2$ from server $s_2$.

Now job $b$ would have exactly one job in server $s_1$ with intersection dimensionality 0 and intersection with all other jobs in the same server would have dimensionality 1 ($33$ such jobs).

Thus if we move $b$ to server $s_2$, there would be 33 pairs for which, the number of common servers would reduce from 7 to 6 with whom $b$ was paired earlier. 

Let us denote the job with whom $b$ has intersection of zero dimension be $a$ in server $s_1$. Now $a$ must be present in $s_2$ as well, thus the pair $(b,a)$ would continue to have same number of common servers.

Except job $a$, none of the jobs in $s_2$ would have been in server $s_1$.

Thus there would be 33 pairs for which number of common servers would increase from 1 to 2 on moving from server $s_1$ to $s_2$.

Similar argument could be made considering pairs with $c$ as well. We can also say that job $a$ would have zero dimensional intersection with job $c$ as well.

Thus $\mathfrak{n}^D_{1,\mathcal{D}_2}=31\times 21\times 280 - 33\times 2$ and $\mathfrak{n}^D_{2,\mathcal{D}_2} = 33\times 2$, $\mathfrak{n}^D_{6,\mathcal{D}_2}= 33\times 2$, $\mathfrak{n}^D_{7,\mathcal{D}_2}= 31\times 21\times 45-33\times 2$ and $\mathfrak{n}^D_{t,\mathcal{D}_2}=0$ for all $t\neq 1,2,6,7$

Now we know from previous theorem, $f(i_t,j_t)- f(i_{t-1},j_{t-1})$ is increasing in $t$.
}

\remove{
Also we can 

Thus $f(i_7,j_7)-f(i_6,j_6) > f(i_2,j_2)-(i_1,j_1)$, hence $f(i_7,j_7)+f(i_1,j_1)> f(i_2,j_2)+f(i_6,j_6)$.
}
Now,

\begin{align*}
 & \sum\limits_{p=0}^{r}\mathfrak{n}^D_{p,\mathcal{D}_1}g(p,x) - \sum\limits_{p=0}^{r}\mathfrak{n}^D_{p,\mathcal{D}_2}g(p,x)\\=
& \sum\limits_{p=0}^{r} g(p,x) (\mathfrak{n}^D_{p,\mathcal{D}_1} - \mathfrak{n}^D_{p,\mathcal{D}_2})\\
 = &  (15+33)\times 2 f(i_1,j_1) + 18\times 2 f(i_7,j_7) -33\times 2 f(i_2,j_2) - 18\times 2 f(i_6,j_6) - 15 \times 2 f(i_0,j_0)\\
= & (15\times 2)  (f(i_1,j_1)-f(i_0,j_0)) + 18 \times 2 (f(i_7,j_7)- f(i_6,j_6)) - 33 \times 2 (f(i_2,j_2)-f(i_1,j_1))\\
\overset{(a)}{=} & 30p(1) + 36 p(7) - 66p(2)\\
= & 36 (p(7)-p(2)) - 30(p(2)-p(1)) \overset{(b)}{>}  0   
\end{align*}
  
  
Note that $(a)$ follows from the definition of $p(m) = f(i,j)- f(u,v)$. $(b)$ follows since we prove $p(m+1)-p(m)$ to be increasing in $m$, thus $p(7)-p(6)> p(2)-p(1)$ implying $p(7)- p(2)>p(2)-p(1)$ coupled with the fact that $p(m)$ is non negative. 

Recall from the proof of theorem 3 that the numerator in the first term of variance can be written as
\begin{align*}
& \sum\limits_{i} \sum\limits_{j} \sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1} (\mathfrak{n}^D_{j,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{j,\hat{S}}>1}\\
=& 2.\sum\limits_{p=0}^{r}\mathfrak{n}^D_{p,\mathcal{D}}g(p,x) + \sum\limits_i \sum\limits_{\substack{\hat{S} \subset \mathcal{S};\\|\hat{S}|=x}} ((\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1})^2\\
=& 2.\sum\limits_{p=0}^{r}\mathfrak{n}^D_{p,\mathcal{D}}g(p,x) + n\sum\limits_{t=1}^{k-1} t^2{k \choose (t+1)} {(n-k) \choose (x-t-1)}
\end{align*}



Thus we show variance depends exclusively on $\sum\limits_{p=0}^{r}\mathfrak{n}^D_{p,\mathcal{D}}g(p,x)$ which implies that assignment $\mathcal{D}_2$ has smaller variance than the assignment ${D}_1$. 

Thus, the distribution as per geometry need not have the least variance.   
}
\remove{
\begin{claim}{\label{min_var_gen}}
	Consider a distribution for a given $n,k$ satisfying the conditions in \ref{setting_condition} such that any of the following conditions hold true.
	\begin{itemize}
		\item Every pair of servers have $l_1$ or $l_1+1$ number of common jobs for some positive integer $l_1$.
		\item Every pair of jobs are present together in exactly $l_2$ or $l_2+1$ servers.
	\end{itemize} 
\end{claim}
}

\remove{

\section{Higher order moments of the distinct jobs}

We now consider some other constructions based on $t$-designs as defined in \cite{tdesign} which is a generalisation of balanced incomplete block designs. Note that $t-(v,p,\lambda)$ design is defined as follows. This is an ordered pair $(A,B)$, where $\hat{S}$ is a set of cardinality $v$, and $B$ is a family of $p$-subsets (called
blocks) of $A$ with the property that each $t$-subset of $A$ is contained in precisely $\lambda$ blocks of $B$.


Let us state a key property of $t$-design as proven in \cite{tdesign}.

\begin{lemma}{\label{lower_t_design}}
	Consider any $t$-design as described above. Note that every $t$-design is also a $i-(v,p,\lambda_i)$ design with $\lambda_i\times {p-i \choose t-i}=\lambda\times {v-i \choose t-i}$ for $\forall i \leq t$.
\end{lemma}

As per the definition in the above lemma, $\lambda_0=|B|$

Assignment scheme: Now we propose an assignment of jobs and servers based on above mentioned design. Note that each job is denoted by a distinct element in $\hat{S}$ and each server is denoted by a distinct element in $B$. %Note that a server corresponding to every element in $\hat{S}$ ($p$-subset) is assigned those jobs corresponding 
Consider all elements of $\hat{S}$ belonging in every element of $B$($p$-subset). We now assign all jobs corresponding to all such elements of $\hat{S}$ to the server denoting the element of $B$($p$-subset). Thus, each server is assigned $p$ jobs which is denoted by $k$ in our setting, $v$ is denoted by $n$ and $|B|$ being denoted by $c$ in our setting.

Hence, every $i$-subset of jobs is assigned together to exactly $\lambda_i=\lambda\frac{{n-i\choose t-i}}{{k-i \choose t-i}}$ servers $\forall i \leq t$ in the above setting.

Recall the notation used in {S}ec~\ref{notation} where we denote the jobs as $\{a_1,a_2,...,a_n\}$ and the servers as $\{s_1,s_2,...,s_n\}$. Let us try to analyse the number of distinct jobs $(d)$ when any subset of servers ($\hat{S}$) return.

Recall that $\mathfrak{n}^D_{i,\hat{S}}$ denotes the number of times job $a_i$ occurred in subset $\hat{S}$ for any $i \leq n$. Note that $\mathfrak{n}^D_{i,\hat{S}}$ could possibly be zero for some values of $i$ as well. Note that $\mathbbm{1}_E$ denotes the indicator random variable corresponding to event $E$. Let us denote the distribution of jobs in servers by $D$. %We denote the number of subsets of 

We are interested in those jobs which have $\mathfrak{n}^D_{i,\hat{S}}>1$ in subset $\hat{S}$ and thus claim that no of distinct jobs ($d$) received from subset $\hat{S}$ is $(k\times x- \sum\limits_{i} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1})$ if the cardinality of $\hat{S}$ is $x$.


\begin{theorem}
	Consider an assignment scheme of jobs and servers as per the one described above based on $t$-design for a given $n,k,r$ and $c$. All such distributions would have the same $t^{th}$ moment on the number of distinct jobs received when any set of $x$ servers return their jobs uniformly at random.
\end{theorem}      


\begin{proof}
	
	Let us calculate the $t^{th}$ moment of number of distinct jobs $d$ received.
	\begin{align*}
	\mathbb{E}_{D,x}[d^t]
	= & \frac{\sum\limits_{\substack{\hat{S} \subset \{s_1,s_2,...,s_n\};\\|\hat{S}|=x}} (k\times x- \sum\limits_{i} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1})^t}{\sum\limits_{\substack{\hat{S} \subset \{s_1,s_2,...,s_n\};\\|\hat{S}|=x}} 1}\\
	= & \frac{\sum\limits_{\substack{\hat{S} \subset \{s_1,s_2,...,s_n\};\\|\hat{S}|=x}} \left(\sum\limits_{l=0}^{t}\left({{t \choose l}}(-1)^l.(k\times x)^{t-l}(\sum\limits_{i} (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1})^{l}\right)\right)}{{n \choose x}}\\
	\overset{(a)}{=} & \frac{\sum\limits_{l=0}^{t} (k\times x)^{t-l}(-1)^l \sum\limits_{\substack{\hat{S} \subset \{s_1,s_2,...,s_n\};\\|\hat{S}|=x}} \left(\sum\limits_i  (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1}\right)^l }{{n \choose x}}
	\end{align*}
	
	Now consider for any $l \leq t$.
	
	\begin{align*}
	& \sum\limits_{\substack{\hat{S} \subset \{s_1,s_2,...,s_n\};\\|\hat{S}|=x}} \left(\sum\limits_i (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1}\right)^l\\
	= & \sum\limits_{\substack{\hat{S} \subset \{s_1,s_2,...,s_n\};\\|\hat{S}|=x}} \sum\limits_{i_1,i_2,...,i_l}  (\mathfrak{n}^D_{i_1,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i_1,\hat{S}}>1} (\mathfrak{n}^D_{i_2,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i_2,\hat{S}}>1}...(\mathfrak{n}^D_{i_l,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i_l,\hat{S}}>1}
	\end{align*}
	
	Now consider the $l$ elements in $(i_1,i_2,...,i_l)$, with $q$ distinct element and $t_u$ of each type $\forall u \in [q]$ and the distinct elements are $e_1,e_2,...,e_q$ with $e_1<e_2<...<e_q$ and thus, $\sum\limits_{u=1}^{q}t_u=l$. Note that for every set $\{e_1,e_2,...,e_q\}$ and $\{t_1,t_2,...,t_q\}$, there would exist $\frac{l!}{\prod_{u=1}^{q}(t_u)!}$ distinct $l$ corresponding elements $(i_1,i_2,...,i_l)$.
	
	Hence, the above expression can be written as.
	
	\begin{align*}
	& \sum\limits_{\substack{\hat{S} \subset \{s_1,s_2,...,s_n\};\\|\hat{S}|=x}} \sum\limits_{\substack{t_1,t_2,...,t_q;\\ \sum\limits_{u=1}^{q}t_u=l}} \sum\limits_{e_1>e_2>...>e_q} (\mathfrak{n}^D_{e_1,\hat{S}}-1)^{t_1} \mathbbm{1}_{\mathfrak{n}^D_{e_1,\hat{S}}>1} (\mathfrak{n}^D_{i_2,\hat{S}}-1)^{t_2} \mathbbm{1}_{\mathfrak{n}^D_{e_2,\hat{S}}>1}...(\mathfrak{n}^D_{i_q,\hat{S}}-1)^{t_q} \mathbbm{1}_{\mathfrak{n}^D_{i_q,\hat{S}}>1}\\
	= & \sum\limits_{q=1}^{l}\sum\limits_{f_1,f_2,...,f_q=1}^{k} \sum\limits_{\substack{t_1,t_2,...,t_q;\\t_1+t_2+...+t_q=l}} \sum\limits_{\substack{\hat{S} \subset \{s_1,s_2,...,s_n\} ; |\hat{S}|=x;\\ \mathfrak{n}^D_{e_1,\hat{S}}=f_1+1;\mathfrak{n}^D_{e_2,\hat{S}}=f_2+1;...;\mathfrak{n}^D_{e_q,\hat{S}}=f_q+1}} f_1^{t_1} f_2^{t_2}... f_q^{t_q}\\
	= & \sum\limits_{q=1}^{l}\sum\limits_{f_1,f_2,...,f_q=1}^{k} \sum\limits_{\substack{t_1,t_2,...,t_q;\\t_1+t_2+...+t_q=l}}  f_1^{t_1} f_2^{t_2}... f_q^{t_q} \sum\limits_{\substack{\hat{S} \subset \{s_1,s_2,...,s_n\} ; |\hat{S}|=x;\\ \mathfrak{n}^D_{e_1,\hat{S}}=f_1+1;\mathfrak{n}^D_{e_2,\hat{S}}=f_2+1;...;\mathfrak{n}^D_{e_q,\hat{S}}=f_q+1}} 1
	\end{align*}
	
	We now argue that for an assignment as per $t$-design the above sum can be uniquely computed for every $l$. We argue this by showing for every sub-set $\{e_1,e_2,..e_q\}$ the number of subsets $\hat{S}$ with cardinality $x$ satisfying $\mathfrak{n}^D_{e_1,\hat{S}}=f_1+1;\mathfrak{n}^D_{e_2,\hat{S}}=f_2+1;...;\mathfrak{n}^D_{e_q,\hat{S}}=f_q+1$ can be uniquely determined. This can be argued as we know that every $l$ subset of jobs occur together in $\lambda_l$ servers which follows as a consequence of Lemma ~\ref{lower_t_design}. Thus, we know precisely in how man servers job $a_{e_1}$ occurs without any of $a_{e_2},...a_{e_t}$ or in how many $a_{e_1}$ and $a_{e_2}$ occur together without any of $a_{e_3},...a_{e_t}$. In general we precisely know in how many servers jobs $\{a_{e_j}|j \in T\}$ occur together without any of jobs in $\{a_{e_j}|j \notin T\}$ for every $T$ with cardinality at most $t$.
	
	%Note that every $q$-subset $(e_1,e_2,...,e_q)$  
\end{proof}

The following statement is an hypothesis which we fail to prove. 


In the subsequent lemma, we now compute the $(t+1)^{th}$ moment of the number of distinct jobs.

\begin{theorem}
	Consider an assignment scheme of jobs and servers as per the one described above based on $t$-design for a given $n,k,r$ and $c$. No other assignment of jobs to servers based on $t$-design would have a higher $(t+1)^{th}$ moment of the number of distinct jobs received when any $x$ servers return uniformly at random than the one based on a $(t+1)$-design for $t>2$.
	
	%All such distributions would have the same $t^{th}$ moment on the number of distinct jobs received when any set of $x$ servers return their jobs uniformly at random.
\end{theorem} 


For the case of $t=2$, we know that the opposite is true i.e. a design based on BIBD has the
least second moment. We can show for $t=3$ that precisely that the above hypothesis holds, however giving a general statement remains an important question.
}

\remove{
	It is important to note that every $(t+1)$-design is a $t$-design too as shown in \ref{lower_t_design}.
	
	\begin{proof}
		Recall from the proof of previous theorem that 
		
		
		\begin{align*}
		& \mathbb{E}_{\mathcal{D},x}[d^{t+1}]\\
		\overset{(a)}{=} & \frac{\sum\limits_{l=0}^{t+1} (k\times x)^{t-l}(-1)^l \sum\limits_{\substack{\hat{S} \subset \{s_1,s_2,...,s_n\};\\|\hat{S}|=x}} \left(\sum\limits_i  (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1}\right)^l }{{n \choose x}}\\
		= & \frac{\sum\limits_{l=0}^{t} (k\times x)^{t+1-l}(-1)^l \sum\limits_{\substack{\hat{S} \subset \{s_1,s_2,...,s_n\};\\|\hat{S}|=x}} \left(\sum\limits_i  (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1}\right)^l }{{n \choose x}} + (-1)^{t+1} \frac{\sum\limits_{\substack{\hat{S} \subset \{s_1,s_2,...,s_n\};\\|\hat{S}|=x}} \left(\sum\limits_i  (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1}\right)^{t+1} }{{n \choose x}} 
		\end{align*}
		
		
		Note that we have shown in the proof of previous theorem that first term can be uniquely determined for every $t$-design as $\sum\limits_{\substack{\hat{S} \subset \{s_1,s_2,...,s_n\};\\|\hat{S}|=x}} \left(\sum\limits_i (\mathfrak{n}^D_{i,\hat{S}}-1) \mathbbm{1}_{\mathfrak{n}^D_{i,\hat{S}}>1}\right)^l$ was shown to be same for every $t$-design. 	
	\end{proof} 
}




==> test-conclusion.tex <==
\section{Conclusion}
In this work, we study the mean and the variance of the number of distinct jobs received at server under various assignment schemes and show that assignment schemes based on the repetition coding and block designs attain the largest and least variance respectively. However, it is not always known whether such designs always exist and famous Bruck-Ryser-Chowla theorem in \cite{sprott1955} gives some necessary conditions on $n,k,r$. In future works, it would be interesting to see if small modifications to designs are still close to ``extremal'' variance in case they do not exist. Another direction of work could be to extend these ideas to analyse the $t^{th}$ moment beyond the second moment that we study and investigate if constructions based on $t$-designs can attain extremal results. 


%Even in cases where $n,k,r$ may lead to a  $\lambda$ which is a positive integer,  it is not known whether a BIBD always exists. However, multiple constructions of BIBD for various parameters have been described in \cite{doi:10.1111/j.1469-1809.1939.tb02219.x} using various techniques, like vector sub-spaces over finite fields etc. The famous Bruck-Ryser-Chowla theorem in \cite{sprott1955} gives some necessary conditions on $n,k,r$ that guarantees the existence of a BIBD.

==> test-intro.tex <==
\section{Introduction}

A distributed computing framework where the computation is done on multiple machines has been widely used for large-scale computations in \cite{Azurecitation, AWScitation, GoogleCloudcitation}. This framework allows us to utilize the computation resources and memory of multiple machines often referred to as workers. Under a common and simple implementation of distributed computing, the master server divides the computation tasks to multiple child servers (workers). After each worker finishes its computation, it shares its results with the master server.  The master aggregates the results received from different workers to finish its task.


However, in real noisy communication frameworks, a subset of servers (workers) can be arbitrarily slow (often referred to as the stragglers) compared to the rest of the workers. Lately, there has been work to mitigate the issue of stragglers by introducing redundancies \cite{JMLR:v20:18-148, DBLP:journals/corr/abs-1906-10664,10.1145/3055281}. Coding theoretic techniques have often been used to introduce redundancies for straggler mitigation described extensively in \cite{li2020coded} and used to split the data and assign different data parts to different servers. Distributed coding framework has been used in gradient computation \cite{pmlr-v70-tandon17a}, matrix-matrix multiplication \cite{lee2017speeding, yu2017polynomial}, polynomial computation \cite{yu2019lagrange} and convolution coding\cite{8006960} using techniques from coding theory namely MDS codes\cite{lee2017speeding,ferdinand2018hierarchical}, LDPC codes\cite{maity2019robust} and rateless codes\cite{mallick2020rateless}. The master server aggregates the computations transmitted by the non-straggling workers to compute the desired result.




However, as happens typically in most modern cloud computing systems like Amazon EC2,  some servers can operate with a significantly high throughput \cite{10.5555/2482626.2482645,6681620,6973767}. Statistical knowledge of communication and computation latency of each server can be used to design better assignment schemes and allocate the tasks more efficiently as studied in\cite{8885332,9014006,10.1145/3323679.3326528}. 

On a side note, there may be several scenarios where it may not be possible to split a computing task to multiple sub-parts, and job cloning is often used for straggler mitigation in such scenarios as studied in \cite{chen2014queueing,ananthanarayanan2013effective,joshi2015queues,10.1145/3055281,4154088}. This is also popular in cloud computing \cite{10.1145/3055281,10.1145/2847220.2847223,10.1145/2637364.2592042} where one task is assigned to multiple servers to combat the stragglers to obtain a low compute time. 


In this paper, we broadly study this problem of job assignment of multiple cloned jobs to multiple servers treating each server with identical communication latency where each server has a significant probability of straggling. These assignment schemes may be particularly useful in framework where there is high noise in the communication channel between the child servers and master server.



\section{Related work}

Block designs have been widely used in experiment design \cite{bose1939partially,addelman1969generalized,shieh2004effectiveness} where experiment designs are grouped into blocks and random treatments are applied to each block. Recently block designs and its variants have been used to construct LDPC codes \cite{ammar2004construction}, gradient coding \cite{kadhe2019gradient,sakorikar2021variants} and error correcting codes \cite{smith1968application}. The most common amongst these are 2-designs or as often called balanced incomplete block designs (BIBDs), which are designs where every pair of points occur together in the same number of blocks \cite{bose1939partially,10.5555-1202540}. It has been shown that 2-designs (if exist) uniquely attain A-, D- and E optimality for experiment design \cite{10.1214/aos/1176343002,4e05890a-5af4-3aa4-948b-f44a2cc9151f}, which was further generalized in \cite{7c66992f-2b5b-3d69-be0f-fe6ad7e70150}. However, our framework is different where we study variance on the number of distinct tasks received at the the master and show that repetition coding and a generalization of BIBDs can be utilized to attain the largest and the least variance respectively.

%Our work demonstrates that .




In another direction, assignment policies of tasks to different servers under a distributed server system have been studied, check \cite{semchedine2011task} for a survey on the same. Typically tasks arrive to a distributed server system stochastically in real time and this system typically distributes the tasks to various servers to minimise the response time as studied in \cite{colajanni1998analysis,harchol2000task,harchol1999choosing}. Recent observations show that the distribution of tasks follows a heavy-tailed distribution \cite{650143,workoladcharacterisation,crovella1998heavy,williams2005web}, and designing assignment policies suited for load balancing across servers becomes difficult. 
In many cases, it may not be possible to recover the entire result but only partially recover the result as studied in coding theory \cite{DBLP:journals/corr/BalajiK15,KORHONEN2009229}. This setup has also been studied in distributed computing setups where the aim is not to recover the exact result but an approximation of the result suffices. This setup has been studied for matrix computation \cite{ozfatura2021coded} and for gradient coding \cite{sarmasarkar2022gradient,10.1145/3366700}. Our problem follows a similar setup where the master only aims to recover a high fraction of the jobs as it may be difficult for the server to recover all tasks in a noisy environment where a substantial fraction of servers may straggle. 

\section{Our contributions}
In this paper, we study a setup where a master aims to compute $n$ jobs and has $c$ identical servers to do the computations. In our model, the arrival and assignment of tasks are not in real-time but instead, the set of tasks (jobs) to be computed and the set of servers is given apriori. Jobs are appropriately replicated and can be viewed as a way to mitigate the issue of slow (straggling) workers. We study a homogeneous setup treating all the servers as having identical computing and stochastic properties, that is, balanced schemes with each server being assigned $k$ jobs and each job being assigned to $r$ servers. We further assume that each server is equally likely to straggle. We consider a 
setup where a non-straggling worker can successfully transmit all tasks to the master as studied in \cite{pmlr-v70-tandon17a,10.1145/3055281,8849684}. We aim to design coding schemes where the master aims to maximise the number of computed distinct jobs that are received. Towards this aim, we study the mean and variance of the number of distinct jobs received in Section \ref{setup_section}. %Optimizing for the second moment viz, the variance may be useful for communication in a noisy setup where a large or a significant fraction of servers may fail to communicate or straggle. 


Our contributions can be described as follows.

a) We first show that when any set of $x$ servers is equally likely to straggle, then for every balanced assignment, the expected number of completed jobs that the master receives is the same (Theorem \ref{all_mean}) and study the variance of the number of jobs received within the class of balanced assignment schemes. 

b) Typically, assignment schemes with the largest variance may be useful for systems where we aim to increase the likelihood of the master receiving a large number (or all) of jobs (heavier mass at distribution tails), and schemes with the least variance may be useful for systems where one aims to reduce the likelihood of the master receiving a small number of jobs (lighter mass at the distribution tails). This follows since every balanced assignment scheme has the same expectation on the jobs received.

c) We show that certain special balanced assignments (called proximally compact and stretched compact designs) when they exist, are guaranteed to attain the least variance and largest variance respectively  (Theorem \ref{min_var} and Theorem \ref{max_var} in Section \ref{extreme_var_section}). 

d) We show how our results generalise to the case where $x$ is sampled from a distribution. This would imply that results on least variance and largest variance would continue to hold when each worker is independently and equally likely to straggle with probability $p$ (Theorems  \ref{all_mean_sampled}, \ref{max_var_sampled} and \ref{min_var_sampled} in Section \ref{sec_randomness_return_servers}).

e) Finally, we show that when the number of jobs equals the number of servers, proximally compact job assignments and server assignments (replacing the roles of jobs and servers) are identical and both of them attain the least variance in Theorem \ref{job_server_pairs_identical} in Appendix \ref{job_no_server_no_identical_section}.

%We thus broadly study the idea of partial recovery in this job assignment setup.











==> timepass.tex <==
\section{Construction of $\vec{h^D}$}




With this setup, we now study assignment schemes on when the least variance on the number of distinct jobs $d$ is attained. We specifically propose pairwise balanced designs discussed in Definition \ref{pair_job_balanced_definition} and \ref{pair_server_balanced_definition}  in Theorem \ref{min_var_gen} and \ref{min_var_gen_spec} and show that it attains the least variance amongst the class of balanced assignments. We now compare  this definition to balanced incomplete block designs (BIBD) \cite{doi:10.1111/j.1469-1809.1939.tb02219.x,10.5555-1202540} and show that it is a generalization of the same.

\begin{nameddefinition}{Defintion}
    (BIBD $(v,b,r,k,\lambda)$ scheme as in \cite{10.5555-1202540}) - A balanced incomplete block design (BIBD) is a pair $(V, B)$ where V is a $v$-set and B
is a collection of $b$ $k$-sized subsets of $V$ (blocks) such that each element of $V$ is contained
in exactly $r$ blocks and any 2-subset of V is contained in exactly $\lambda$ blocks.
\end{nameddefinition}

Note that this set up can be directly mapped to our setup where $V$ denotes the set of all jobs and each block in $B$ denotes a server and each server(block) in $B$ is precisely assigned those jobs corresponding to the set of elements of $V$ in that block. Also, observe that in BIBD design, we require every set of jobs to occur together in the same number of servers but our pairwise balanced schemes allow a tolerance of upto 1 as we can see in Definition \ref{pair_job_balanced_definition}.


\begin{nameddefinition}{Definition}{\label{pair_job_balanced_definition}}
    (Pairwise balanced job $(n,k,r,c)$ assignment): Given a balanced $(n,k,r,c)$ assignment, we call it  pairwise balanced job $(n,k,r,c)$ assignment if for every pair of distinct jobs $a_i$ and $a_j$ in $\mathcal{A}$, the number of servers which are assigned both $a_i$ and $a_j$ is exactly $l$ or $l+1$ for some integer $l$.

\end{nameddefinition}

Using $\mathfrak{m}^D(.)$ defined in \eqref{m_D_defn}, we can define pairwise balanced job assignments below. W.L.O.G, we may assume in pairwise balanced job $(n,k,r,c)$ assignment, there always exist a pair of jobs occurring together in $l$ server and there may or may not be pairs of jobs that occur together in $l+1$ servers. 


\begin{definition*}
    [Definition \ref{pair_job_balanced_definition} in terms of $\mathfrak{m}^D(.)$](Pairwise balanced job $(n,k,r,c)$ assignment): Given a balanced $(n,k,r,c)$ assignment, we call it server pairwise -balanced $(n,k,r,c)$ if $\mathfrak{m}_D(m)$ is non-zero for at most 2 consecutive values of $m$ (call it $l$ and $l+1$). 
\end{definition*}


Thus, we can see that BIBD would also fall into the category of pairwise balanced job assignment schemes. The existence of BIBD is still not fully understood and some sufficient conditions on $n,k,r$ and $c$ under which BIBD exists are also discussed in \cite{10.5555-1202540,doi:10.1111/j.1469-1809.1939.tb02219.x}. The famous Bruck-Ryser-Chowla theorem gives some necessary condition on $n,k,c,r$ for the existence of BIBDs. 




The following corollary proves a result on $l$ for any pairwise balanced job $(n,k,r,c)$ assignment.

\begin{namedlemma}{Lemma}{\label{lemma_on_l_job}}
    For any pairwise balanced job $(n,k,r,c)$ assignment, we have $l=\Bigl\lfloor\frac{c.{{k \choose 2}}}{{{n \choose 2}}}\Bigr\rfloor$

    %\Bigl\lfloor\dfrac{1}{2}\Bigr\rfloor
\end{namedlemma}

\begin{proof}


For any pairwise balanced job $(n,k,r,c)$ assignment $D$, we must have $\mathfrak{m}^D(m)$ to be zero for all $m\neq l,l+1$. Thus, we have $\mathfrak{m}^D(l+1) = {{n \choose 2}}- \mathfrak{m}^D(l)$ using eqaution \eqref{proporty_m_1} and similarly, we have $l(\mathfrak{m}^D(l)) + (l+1)({{n \choose 2}}- \mathfrak{m}^D(l)) = c{{k\choose 2}}$ using equation \eqref{property_m_2}. We thus have $l {{n \choose 2}} \leq c{{k \choose 2}}$ and $(l +1){{n \choose 2}} > c{{k \choose 2}}$ (as $\mathfrak{m}^D(l)>0$) and thus $l=\Bigl\lfloor\frac{c.{{k \choose 2}}}{{{n \choose 2}}}\Bigr\rfloor$

\remove{
    
Let $n_l$ be the number of pairs of jobs that are present together in exactly $l$ servers and all other pairs of jobs are contained in $l+1$ servers. Therefore, the number of pairs of jobs that are present together in exactly $l+1$ servers is given by ${{n \choose 2}}-n_l$. 


Thus, summing up over all pairs of jobs, we can say that the total number of servers that contain pairs of distinct jobs (allowing multiple counting for a server if contains more than a pair) is given by $l\times n_l+ (l+1) \times ({{n \choose 2}}-n_l)$. However, observe that the number of pairs of jobs that are assigned to a fixed server $s_i$ is given by ${{k \choose 2}}$. Thus, summing over all such servers $\mathcal{S}$ we can obtain the same quantity to be $c \times {{k \choose 2}}$ and thus, $l\times n_l+ (l+1) \times ({{n \choose 2}}-n_l)=c \times {{k \choose 2}}$ implying, $l= \Bigl\lfloor\frac{c.{{k \choose 2}}}{{{n \choose 2}}}\Bigr\rfloor$ 


}

\end{proof}



%This follows since the total number of pairs of distinct jobs that can be assigned a fixed server $s_i$ is given by ${{k \choose 2}}$ thus, the total number of pairs of jobs that are assigned to a single server (allowing multiple counting if one pair of jobs is present together in more than one server) is given by $c{{k \choose 2}}$ 





\begin{nameddefinition}{Definition}{\label{pair_server_balanced_definition}}
    (Pairwise balanced server $(n,k,r,c)$ assignment): Given a balanced $(n,k,r,c)$ assignment, we call it server pairwise -balanced $(n,k,r,c)$ if for every pair of distinct servers $s_i$ and $s_j$ in $\mathcal{S}$, the number of jobs assigned to both $s_i$ and $s_j$ is exactly $l$ or $l+1$ for some integer $l$.
\end{nameddefinition}

\begin{namedlemma}{Lemma}{\label{lemma_on_l_server}}
    For any pairwise balanced server $(n,k,r,c)$, we must have $l=\Bigl\lfloor\frac{n.{{r \choose 2}}}{{{c \choose 2}}}\Bigr\rfloor$
\end{namedlemma}

This lemma can be proved in a very similar way as that of Lemma \ref{lemma_on_l_job}.

With this, we could alternately redefine pairwise balanced server $(n,k,r,c)$ schemes as follows in terms of matrix $A_D$ as follows.

\begin{definition*}
    [Definition \ref{pair_job_balanced_definition} in terms of $A_D$](Pairwise balanced server $(n,k,r,c)$ assignment): Given a balanced $(n,k,r,c)$ assignment, we call it server pairwise -balanced $(n,k,r,c)$ if for every pair of distinct indices $i$ and $j$, $|\text{supp}(A_D[:,i]) \cap \text{supp}(A_D[:,j])| = l \text{ or } l+1$ for some integer $l$. 
\end{definition*}

\begin{definition*}
     [Definition \ref{pair_server_balanced_definition} in terms of $A_D$](Pairwise balanced job $(n,k,r,c)$ assignment): Given a balanced $(n,k,r,c)$ assignment, we call it job pairwise -balanced $(n,k,r,c)$ if for every pair of distinct indices $i$ and $j$, $|\text{supp}(A_D[i,:]) \cap \text{supp}(A_D[j,:])| = l \text{ or } l+1$ for some integer $l$. 
\end{definition*}






We now describe a pairwise balanced job and server scheme in Example \ref{pairwise_dual_balanced} below. Note that the balanced design is both pairwise job and server balanced in this design. Further, in example \ref{pairwise_balanced_server}, we present an assignment scheme which is pairwise server balanced but not pairwise job balanced.

\begin{example}{\label{pairwise_dual_balanced}}
    We now describe a pairwise balanced server and job $(9,3,3,9)$ assignment scheme in Table \ref{pairwise_dual_balanced_assn}. Note that in this scheme, every pair of jobs appear together in exactly 1 or 0 servers, thus it is a pairwise balanced job assignment scheme. Similarly, we can also show that it is also a pairwise balanced server scheme too as every pair of servers has either one job or zero jobs common.
\end{example}


\begin{table}[!h]
    \centering
{
	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c| } 
		\hline
	\text{Jobs}& $s_1$ & $s_2$ & $s_3$ & $s_4$ & $s_5$ & $s_6$ & $s_7$ & $s_8$ & $s_9$\\
    \hline
    $a_1$ & 1 & 1 & 1 & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$ \\
    \hline
    $a_2$ & $\text{}$ & $\text{}$ & $\text{}$ & 1 & 1 & 1 & $\text{}$ & $\text{}$ & $\text{}$\\
        \hline
     $a_3$ & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$ & 1 & 1 & 1\\
        \hline
    $a_4$ & 1 & $\text{}$ & $\text{}$ & 1 & $\text{}$ & $\text{}$ & 1 & $\text{}$ & $\text{}$\\
    \hline
    $a_5$ & $\text{}$ &1 & $\text{}$ & $\text{}$ & 1 & $\text{}$ &  $\text{}$ & 1 & $\text{}$\\
        \hline
     $a_6$ & $\text{}$ & $\text{}$ &1  & $\text{}$ & $\text{}$ & 1 &  $\text{}$  & $\text{}$ & 1\\
        \hline
    
    $a_7$ & 1 & $\text{}$ & $\text{}$ & $\text{}$ & 1& $\text{}$ & $\text{}$ & $\text{}$ & 1\\
    \hline
    $a_8$ &$\text{}$& 1 & $\text{}$ & $\text{}$ & $\text{}$ & 1& 1& $\text{}$ & $\text{}$  \\
        \hline
     $a_9$ & $\text{}$ & $\text{}$ & 1 & 1& $\text{}$ & $\text{}$ & $\text{}$ & 1 & $\text{}$ \\
        \hline
        
	\end{tabular}
 }
	\vspace{1 em}
	\caption{Assignment of jobs to various servers in a pairwise balanced $(9,3,2,6)$ assignment scheme}
	\label{pairwise_dual_balanced_assn}
\end{table}

\newpage
\begin{example}{\label{pairwise_balanced_server}}
    We now describe a pairwise balanced server $(14,6,3,7)$ assignment but not a pairwise balanced job scheme in Table \ref{pairwise_balanced_server_assn}. Note that in this scheme, every pair of servers have exactly 2 jobs in common. However, some pairs of jobs appear together in 1 server like $(a_1,a_2)$ and some pairs of jobs appear together in 3 servers like pairs of jobs $(a_1,a_8)$ and thus it is not pairwise job balanced.
\end{example}


\begin{table}[!h]
    \centering
{
	\begin{tabular}{|c|c|c|c|c|c|c|c| } 
		\hline
	\text{Jobs}& $s_1$ & $s_2$ & $s_3$ & $s_4$ & $s_5$ & $s_6$ &$s_7$ \\
    \hline
    $a_1$ & $\text{}$ & 1 & $\text{}$ & 1 & $\text{}$ & 1 & $\text{}$ \\
    \hline
    $a_2$ & 1 & $\text{}$ & $\text{}$ & 1 & 1 & $\text{}$ & $\text{}$\\
        \hline
     $a_3$ & $\text{}$ & $\text{}$ & 1 & 1 & $\text{}$ & $\text{}$ & 1 \\
        \hline
    $a_4$ & 1 & 1 & 1 & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$\\
    \hline
    $a_5$ & $\text{}$ &1 & $\text{}$ & $\text{}$ & 1 & $\text{}$ &  1 \\
        \hline
     $a_6$ & 1 & $\text{}$  & $\text{}$ & $\text{}$ &  $\text{}$  & 1 & 1\\
        \hline
    
    $a_7$ & $\text{}$ & $\text{}$ & 1 & $\text{}$ & 1& 1 &$\text{}$ \\
    \hline
    $a_8$ & $\text{}$ & 1 & $\text{}$ & 1 & $\text{}$ & 1 & $\text{}$ \\
    \hline
    $a_9$ & 1 & $\text{}$ & $\text{}$ & 1 & 1 & $\text{}$ & $\text{}$\\
        \hline
     $a_{10}$ & $\text{}$ & $\text{}$ & 1 & 1 & $\text{}$ & $\text{}$ & 1 \\
        \hline
    $a_{11}$ & 1 & 1 & 1 & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$\\
    \hline
    $a_{12}$ & $\text{}$ &1 & $\text{}$ & $\text{}$ & 1 & $\text{}$ &  1 \\
        \hline
     $a_{13}$ & 1 & $\text{}$  & $\text{}$ & $\text{}$ &  $\text{}$  & 1 & 1\\
        \hline
    
    $a_{14}$ & $\text{}$ & $\text{}$ & 1 & $\text{}$ & 1 & 1 & $\text{}$  \\
    \hline
        
	\end{tabular}
 }
	\vspace{1 em}
	\caption{Assignment of jobs to various servers in a pairwise server balanced $(14,6,3,7)$ assignment scheme}
	\label{pairwise_balanced_server_assn}
\end{table}








Note that the following two theorems say that the variance on the number of distinct $d$ received at the master is the least for the pairwise balanced designs discussed in Definition \ref{pair_job_balanced_definition} and \ref{pair_server_balanced_definition}. However such designs may not always exist and it is not entirely known when such designs exist for every tuple of $(n,k,r,c)$ satisfying $n \times r = k \times c$. This is closely related to balanced incomplete block designs (BIBD) \cite{doi:10.1111/j.1469-1809.1939.tb02219.x} whose existence is not fully and clearly understood. However, a key difference for the pairwise balanced designs we consider is that it is a generalization of BIBD in which they restrict the number of jobs common to any pair of servers to be the same for every such pair of servers. 

Recall that for the following theorems, we study the setup described in Section \ref{setup_section} where any set of $x$ servers could be the only set of servers that could communicate with the master. Recall that we further assume that every set of $x$ servers is equally likely to be the only set of servers that could communicate with the master. %Reca 


Also under a special constraint $n=c$, the above theorem can also be stated as follows and we can say that the same result holds true for pairwise server balanced $(n,k,r,c)$ scheme too.

\begin{theorem}{\label{min_var_gen_spec}}
The least variance of the number of distinct jobs received at the master for any $x \in [1,c-2r+1]$ \remove{when any subset of servers $\mathcal{S}$ of cardinality $x>1$ is able to communicate with the master (denoted by $\sigma_{D,x}(d)$) with equal probability} is attained uniquely by both the pairwise balanced server $(n,k,k,n)$ assignment schemes and pairwise balanced job $(n,k,k,n)$ assignment schemes (if it exists) amongst all balanced $(n,k,k,n)$ assignments. 

However, for $x>c-2r+1$, the result on least variance still holds but the uniqueness is not guaranteed.
\end{theorem}	

We prove this theorem in Section \ref{proof_min_var_gen_spec}.


\section{Results on the largest variance on the number of distinct jobs $d$}

With this setup, we now study assignment schemes on when the largest variance in the number of distinct jobs $d$ is attained. We specifically define pairwise heavy imbalanced job $(n,k,r,c)$ assignment discussed in Definition \ref{pair_job_imbalanced_definition} and show that in Theorem \ref{max_var_gen} that these schemes attain the largest variance amongst the class of balanced assignment schemes. 

%We now define another set of imbalanced pairwise job assignment schemes where for every pair of distinct jobs $a_i$ and $a_j$ in $\mathcal{A}$, the number of servers that are assigned both of them is either $r$ or 0 and in Theorem \ref{fd} we show that these assignment schemes attain the largest variance on the number of distinct jobs.

\begin{nameddefinition}{Definition}{\label{pair_job_imbalanced_definition}}
    (Pairwise heavy imbalanced job $(n,k,r,c)$ assignment): Given a balanced $(n,k,r,c)$ assignment, we call it pairwise imbalanced job $(n,k,r,c)$ assignment if for every pair of distinct jobs $a_i$ and $a_j$ in $\mathcal{A}$, the number of servers which are assigned both $a_i$ and $a_j$ is exactly 0 or $r$.
\end{nameddefinition}

\begin{definition*}
     [Definition \ref{pair_job_imbalanced_definition} in terms of $A_D$](Pairwise heavy imbalanced job $(n,k,r,c)$ assignment): Given a balanced $(n,k,r,c)$ assignment, we call it job pairwise heavy-imbalanced job $(n,k,r,c)$ assignment if for every pair of distinct indices $i$ and $j$, $|\text{supp}(A_D[i,:]) \cap \text{supp}(A_D[j,:])| = 0 \text{ or } r$. 
\end{definition*}


\begin{lemma}
    A pairwise heavy imbalanced job $(n,k,r,c)$ assignment can exist only when either $n$ or $k-1$ is even. 
\end{lemma}

\begin{proof}
    Observe from \eqref{property_m_2} that $\sum_{m=0}^{r} \mathfrak{m}^D(m) = c{{k \choose 2}}$. Suppose neither $n$ nor $k-1$ is even, thus implying that $n(k-1)$ is not divisible by 2. However, for a pairwise heavy imbalanced job $(n,k,r,c)$ assignment scheme $D$, $\mathfrak{m}^D(m)$ is non-zero only for $m \neq 0,r$ and thus, $\mathfrak{m}^D(r)= \frac{c{{k \choose 2}}}{r}=\frac{n(k-1)}{2}$. Thus, $n(k-1)$ being odd would imply a fractional value for $\mathfrak{m}^D(r)$ which is clearly not possible.
\end{proof}


\begin{example}{\label{pairwise_imbalanced_job}}
    We now describe a pairwise heavy imbalanced job $(9,3,2,6)$ assignment scheme in Table \ref{pairwise_imbalanced_job_assn}. Note that in this scheme, every pair of jobs appear together in exactly $2$ or 0 servers, thus it is a pairwise heavy imbalanced job assignment scheme. 
\end{example}


\begin{table}[!h]
    \centering
{
	\begin{tabular}{|c|c|c|c|c|c|c| } 
		\hline
	\text{Jobs}& $s_1$ & $s_2$ & $s_3$ & $s_4$ & $s_5$ & $s_6$\\
    \hline
    $a_1$ & 1 & 1 & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$ \\
    \hline
    $a_2$ & 1 & 1 & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$\\
        \hline
     $a_3$ & 1 & 1 & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$\\
        \hline
    $a_4$ & $\text{}$ & $\text{}$ & 1 & 1 & $\text{}$ & $\text{}$\\
    \hline
    $a_5$ & $\text{}$ & $\text{}$ & 1 & 1 & $\text{}$ & $\text{}$\\
        \hline
     $a_6$ & $\text{}$ & $\text{}$ & 1 & 1 & $\text{}$ & $\text{}$\\
        \hline
    
    $a_7$ & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$ & 1 & 1 \\
    \hline
    $a_8$ & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$ & 1 & 1 \\
        \hline
     $a_9$ & $\text{}$ & $\text{}$ & $\text{}$ & $\text{}$  & 1 & 1 \\
        \hline
        
	\end{tabular}
 }
	\vspace{1 em}
	\caption{Assignment of jobs to various servers in a pairwise heavy imbalanced $(9,3,2,6)$ assignment scheme}
	\label{pairwise_imbalanced_job_assn}
\end{table}


Recall that for the following theorems, we study the setup described in Section \ref{setup_section} where any set of $x$ servers could be the only set of servers that could communicate with the master. Recall that we further assume that every set of $x$ servers is equally likely to be the only set of servers that could communicate with the master. %Reca 


\begin{namedtheorem}{Theorem}{\label{max_var_gen}}
The largest variance of the number of distinct jobs $d$ received at the master for any $x \in [2,c-2r+1]$ \remove{ when any subset of servers ($\mathcal{S}$) with cardinality $c-2r+1\leq x>1$ is able to communicate with the master $($denoted by $\sigma_{D,x}(d))$ with equal probability} is attained uniquely by the pairwise heavy imbalanced job $(n,k,r,c)$ assignment schemes (if it exists) amongst all balanced $(n,k,r,c)$ assignments. 

However, for $x>c-2r+1$, the result on largest variance still holds but the uniqueness is not guaranteed.

\end{namedtheorem}

We prove this theorem in Section \ref{proof_max_var_gen}

%have been used to introduce redundancies and assignments of data parts to different servers. In coded distributed computing, the input data is often split into multiple parts and assigned to various servers to speed up the computations. 




%Cloning of jobs to mitigate straggling workers have been studied in \cite{chen2014queueing,ananthanarayanan2013effective,joshi2015queues,10.1145/3055281,4154088}. 
%Our work follows a similar setup of job cloning to tackle straggler mitigation.   


%Redundancy techniques for cloud computing have been studied in \cite{10.1145/3055281} where one task is assigned to multiple servers to combat the stragglers to obtain a low compute time. 

%Cloning of jobs to mitigate straggling workers have been studied in \cite{chen2014queueing,ananthanarayanan2013effective,joshi2015queues,10.1145/3055281,4154088}.

%However in our model, the arrival and assignment of tasks is not in real time but the set of tasks(jobs) to be computed and the set of servers is given apriori. Jobs are appropriately replicated to mitigate the issue of slow(straggling) workers.

%\section{Redundancy in distributed computing}

%In coded distributed computing, the input data is often split into multiple parts and assigned to various servers to speed up the computations. Statistical knowledge of communication and computation latency of each server can be used to design better assignment schemes
%and allocate the tasks more efficiently as studied in \cite{8885332,9014006,10.1145/3323679.3326528}. %However, we study a homogeneous setup treating all the servers with identical computing and stochastic properties.

%Techniques from coding theory namely MDS codes\cite{lee2017speeding,ferdinand2018hierarchical}, LDPC codes\cite{maity2019robust} and rateless codes\cite{mallick2020rateless} have been used to introduce redundancies and assignments of data parts to different servers. The master server aggregates the computations transmitted by the non-straggling workers to compute the desired result. %In our work, we discuss the design and construction of a coding scheme.

%\section{Idea of partial recovery}
%We study a partial recovery setup where the aim of the master is not to recover the set of all tasks(jobs) but a partial fraction of that suffices.

%Block designs has been widely used in experiment design \cite{bose1939partially,addelman1969generalized,shieh2004effectiveness} where experiment designs are grouped into blocks and random treatments are applied to each block. Recently block designs and its variants have been used to construct LDPC codes \cite{ammar2004construction}, gradient coding \cite{kadhe2019gradient,sakorikar2021variants} and error correcting codes \cite{smith1968application}. 

%Redundancy techniques for cloud computing have been studied in \cite{10.1145/3055281} where one task is assigned to multiple servers to combat the stragglers to obtain a low compute time.

%\section{Contributions of this paper}

%We also propose the construction of stretched compact design based on a repetition coding scheme and show that proximally compact design schemes could be treated as a generalization of balanced incomplete block designs \cite{doi:10.1111/j.1469-1809.1939.tb02219.x,sprott1955} in Section \ref{min_compact_section} and \ref{max_compact_section}.
%\section{Related Work in block designs and redundancies}

%Block designs has been widely used in experiment design \cite{bose1939partially,addelman1969generalized,shieh2004effectiveness} where experiment designs are grouped into blocks and random treatments are applied to each block. Recently block designs and its variants have been used to construct LDPC codes \cite{ammar2004construction}, gradient coding \cite{kadhe2019gradient,sakorikar2021variants} and error correcting codes \cite{smith1968application}. 

%Redundancy techniques for cloud computing have been studied in \cite{10.1145/3055281} where one task is assigned to multiple servers to combat the stragglers to obtain a low compute time.

%Different assignment policies were compared to get a low compute time and 



